Training Lightweight Gaze Models without Target Gaze Annotation: What Makes a Good Teacher?

Model-generated labels offer a scalable route to training lightweight vision models, but what makes a model a good teacher, and can we tell before training a student? We study this in gaze target estimation, where interactive robots need models that are both accurate and efficient. In a controlled comparison of eleven supervision conditions, we vary only the source of gaze-point labels, keeping the student, training protocol and 361k training samples fixed, across three video datasets, two student sizes and three seeds; every student is evaluated against human annotation. Three findings emerge. First, imperfect model-generated labels can replace human annotation: Gaze-LLE, never trained on the target datasets' gaze annotation, trains students that match annotation-trained ones on ViT-Tiny and are significantly more accurate on ViT-Small (average distance error 0.187 vs 0.196), and the ViT-Tiny student runs 32$\times$ faster than its teacher on a laptop CPU. Second, apparent competence can conceal unreliable supervision: given another person's face centre in the prompt, InternVL3 and Qwen3-VL return it on 93.4% and 81.1% of test samples, and a copy-the-coordinate baseline matches InternVL3's labels and students. Without that coordinate, both models fall far behind the specialist. Third, good teachers can be identified before training: validation label error ranks student test error (Spearman's $\rho = 0.91$), and ten annotated clips single out the two specialist teachers in 95% of draws. These findings give practical principles for assessing supervision, exposing shortcuts and selecting teachers for lightweight models.

==> generated/numbers.tex <==
\makeatletter
\providecommand{\R}[1]{\ifcsname pn@#1\endcsname\csname pn@#1\endcsname\else\textbf{\color{red}??\detokenize{#1}}\fi}
\providecommand{\pend}{{\color{gray}\footnotesize pend.}}
\expandafter\def\csname pn@pop.train.vat\endcsname{103{,}877}
\expandafter\def\csname pn@copy.train.vat\endcsname{95.8\%}
\expandafter\def\csname pn@pop.train.childplay\endcsname{151{,}415}
\expandafter\def\csname pn@copy.train.childplay\endcsname{82.3\%}
\expandafter\def\csname pn@pop.train.vacation\endcsname{105{,}753}
\expandafter\def\csname pn@copy.train.vacation\endcsname{95.8\%}
\expandafter\def\csname pn@pop.train.all\endcsname{361{,}045}
\expandafter\def\csname pn@copy.train.all\endcsname{89.6\%}
\expandafter\def\csname pn@copy.train.prompted\endcsname{336{,}533}
\expandafter\def\csname pn@lab.train.vat.centre.all\endcsname{0.275}
\expandafter\def\csname pn@lab.train.vat.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.centre.all\endcsname{0.257}
\expandafter\def\csname pn@lab.train.childplay.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.centre.all\endcsname{0.300}
\expandafter\def\csname pn@lab.train.vacation.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.centre.all\endcsname{0.275}
\expandafter\def\csname pn@lab.train.all.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.centre.social\endcsname{0.267}
\expandafter\def\csname pn@lab.train.vat.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.centre.social\endcsname{0.262}
\expandafter\def\csname pn@lab.train.childplay.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.centre.social\endcsname{0.306}
\expandafter\def\csname pn@lab.train.vacation.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.centre.social\endcsname{0.281}
\expandafter\def\csname pn@lab.train.all.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.centre.object\endcsname{0.288}
\expandafter\def\csname pn@lab.train.vat.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.centre.object\endcsname{0.255}
\expandafter\def\csname pn@lab.train.childplay.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.centre.object\endcsname{0.292}
\expandafter\def\csname pn@lab.train.vacation.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.centre.object\endcsname{0.270}
\expandafter\def\csname pn@lab.train.all.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.copyb.all\endcsname{0.245}
\expandafter\def\csname pn@lab.train.vat.copyb.all.gtshare\endcsname{4\%}
\expandafter\def\csname pn@lab.train.vat.copyb.all.gtshare1\endcsname{4.3\%}
\expandafter\def\csname pn@lab.train.childplay.copyb.all\endcsname{0.362}
\expandafter\def\csname pn@lab.train.childplay.copyb.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.copyb.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.copyb.all\endcsname{0.262}
\expandafter\def\csname pn@lab.train.vacation.copyb.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.copyb.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.copyb.all\endcsname{0.303}
\expandafter\def\csname pn@lab.train.all.copyb.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.train.all.copyb.all.gtshare1\endcsname{1.0\%}
\expandafter\def\csname pn@lab.train.vat.copyb.social\endcsname{0.144}
\expandafter\def\csname pn@lab.train.vat.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.copyb.social\endcsname{0.105}
\expandafter\def\csname pn@lab.train.childplay.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.copyb.social\endcsname{0.055}
\expandafter\def\csname pn@lab.train.vacation.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.copyb.social\endcsname{0.098}
\expandafter\def\csname pn@lab.train.all.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.copyb.object\endcsname{0.387}
\expandafter\def\csname pn@lab.train.vat.copyb.object.gtshare\endcsname{10\%}
\expandafter\def\csname pn@lab.train.vat.copyb.object.gtshare1\endcsname{10.5\%}
\expandafter\def\csname pn@lab.train.childplay.copyb.object\endcsname{0.449}
\expandafter\def\csname pn@lab.train.childplay.copyb.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.copyb.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.copyb.object\endcsname{0.513}
\expandafter\def\csname pn@lab.train.vacation.copyb.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.copyb.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.copyb.object\endcsname{0.454}
\expandafter\def\csname pn@lab.train.all.copyb.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.train.all.copyb.object.gtshare1\endcsname{1.8\%}
\expandafter\def\csname pn@lab.train.vat.mtgs.all\endcsname{0.074}
\expandafter\def\csname pn@lab.train.vat.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.mtgs.all\endcsname{0.076}
\expandafter\def\csname pn@lab.train.childplay.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.mtgs.all\endcsname{0.100}
\expandafter\def\csname pn@lab.train.vacation.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.mtgs.all\endcsname{0.083}
\expandafter\def\csname pn@lab.train.all.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.mtgs.social\endcsname{0.047}
\expandafter\def\csname pn@lab.train.vat.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.mtgs.social\endcsname{0.073}
\expandafter\def\csname pn@lab.train.childplay.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.mtgs.social\endcsname{0.079}
\expandafter\def\csname pn@lab.train.vacation.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.mtgs.social\endcsname{0.067}
\expandafter\def\csname pn@lab.train.all.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.mtgs.object\endcsname{0.114}
\expandafter\def\csname pn@lab.train.vat.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.mtgs.object\endcsname{0.077}
\expandafter\def\csname pn@lab.train.childplay.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.mtgs.object\endcsname{0.126}
\expandafter\def\csname pn@lab.train.vacation.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.mtgs.object\endcsname{0.096}
\expandafter\def\csname pn@lab.train.all.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.ovd_old.all\endcsname{0.206}
\expandafter\def\csname pn@lab.train.vat.ovd_old.all.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.train.vat.ovd_old.all.gtshare1\endcsname{2.3\%}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.all\endcsname{0.233}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.all.gtshare1\endcsname{1.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.all\endcsname{0.145}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.all.gtshare1\endcsname{1.1\%}
\expandafter\def\csname pn@lab.train.all.ovd_old.all\endcsname{0.199}
\expandafter\def\csname pn@lab.train.all.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.train.all.ovd_old.all.gtshare1\endcsname{1.3\%}
\expandafter\def\csname pn@lab.train.vat.ovd_old.social\endcsname{0.157}
\expandafter\def\csname pn@lab.train.vat.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.social\endcsname{0.143}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.social\endcsname{0.066}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.ovd_old.social\endcsname{0.117}
\expandafter\def\csname pn@lab.train.all.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.ovd_old.object\endcsname{0.275}
\expandafter\def\csname pn@lab.train.vat.ovd_old.object.gtshare\endcsname{6\%}
\expandafter\def\csname pn@lab.train.vat.ovd_old.object.gtshare1\endcsname{5.6\%}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.object\endcsname{0.263}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.object.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.train.childplay.ovd_old.object.gtshare1\endcsname{1.3\%}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.object\endcsname{0.240}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.train.vacation.ovd_old.object.gtshare1\endcsname{2.4\%}
\expandafter\def\csname pn@lab.train.all.ovd_old.object\endcsname{0.260}
\expandafter\def\csname pn@lab.train.all.ovd_old.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.train.all.ovd_old.object.gtshare1\endcsname{2.3\%}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.all\endcsname{0.293}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.all\endcsname{0.278}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.all\endcsname{0.306}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.all\endcsname{0.290}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.object\endcsname{0.294}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.object\endcsname{0.267}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.object\endcsname{0.245}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.object\endcsname{0.266}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.all\endcsname{0.217}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.all.gtshare\endcsname{26\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.all.gtshare1\endcsname{26.4\%}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.all\endcsname{0.184}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.all.gtshare\endcsname{36\%}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.all.gtshare1\endcsname{36.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.all\endcsname{0.257}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.all.gtshare\endcsname{21\%}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.all.gtshare1\endcsname{20.8\%}
\expandafter\def\csname pn@lab.train.all.ovdgate55.all\endcsname{0.215}
\expandafter\def\csname pn@lab.train.all.ovdgate55.all.gtshare\endcsname{29\%}
\expandafter\def\csname pn@lab.train.all.ovdgate55.all.gtshare1\endcsname{28.9\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.ovdgate55.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.object\endcsname{0.109}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.object.gtshare\endcsname{64\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate55.object.gtshare1\endcsname{63.6\%}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.object\endcsname{0.142}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.object.gtshare\endcsname{48\%}
\expandafter\def\csname pn@lab.train.childplay.ovdgate55.object.gtshare1\endcsname{48.1\%}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.object\endcsname{0.134}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.object.gtshare\endcsname{46\%}
\expandafter\def\csname pn@lab.train.vacation.ovdgate55.object.gtshare1\endcsname{46.2\%}
\expandafter\def\csname pn@lab.train.all.ovdgate55.object\endcsname{0.135}
\expandafter\def\csname pn@lab.train.all.ovdgate55.object.gtshare\endcsname{50\%}
\expandafter\def\csname pn@lab.train.all.ovdgate55.object.gtshare1\endcsname{50.3\%}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.all\endcsname{0.215}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.all.gtshare\endcsname{26\%}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.all.gtshare1\endcsname{26.4\%}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.all\endcsname{0.177}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.all.gtshare\endcsname{38\%}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.all.gtshare1\endcsname{37.6\%}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.all\endcsname{0.254}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.all.gtshare\endcsname{21\%}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.all.gtshare1\endcsname{21.2\%}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.all\endcsname{0.210}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.all.gtshare\endcsname{30\%}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.all.gtshare1\endcsname{29.8\%}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.object\endcsname{0.105}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.object.gtshare\endcsname{64\%}
\expandafter\def\csname pn@lab.train.vat.ovdmixrand.object.gtshare1\endcsname{63.7\%}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.object\endcsname{0.132}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.object.gtshare\endcsname{50\%}
\expandafter\def\csname pn@lab.train.childplay.ovdmixrand.object.gtshare1\endcsname{50.2\%}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.object\endcsname{0.129}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.object.gtshare\endcsname{47\%}
\expandafter\def\csname pn@lab.train.vacation.ovdmixrand.object.gtshare1\endcsname{46.9\%}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.object\endcsname{0.127}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.object.gtshare\endcsname{52\%}
\expandafter\def\csname pn@lab.train.all.ovdmixrand.object.gtshare1\endcsname{51.7\%}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.all\endcsname{0.250}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.all.gtshare\endcsname{4\%}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.all.gtshare1\endcsname{4.3\%}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.all\endcsname{0.360}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.all\endcsname{0.267}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.all\endcsname{0.305}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.all.gtshare1\endcsname{1.0\%}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.social\endcsname{0.154}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.social\endcsname{0.136}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.social\endcsname{0.065}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.social\endcsname{0.113}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.object\endcsname{0.386}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.object.gtshare\endcsname{10\%}
\expandafter\def\csname pn@lab.train.vat.vlmleak_old.object.gtshare1\endcsname{10.5\%}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.object\endcsname{0.435}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmleak_old.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.object\endcsname{0.513}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmleak_old.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.object\endcsname{0.446}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.train.all.vlmleak_old.object.gtshare1\endcsname{1.8\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.all\endcsname{0.313}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.all\endcsname{0.320}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.all\endcsname{0.382}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.all\endcsname{0.338}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.object\endcsname{0.343}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.object\endcsname{0.323}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.object\endcsname{0.414}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.object\endcsname{0.349}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.all\endcsname{0.297}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.all.gtshare\endcsname{4\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.all.gtshare1\endcsname{4.3\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.all\endcsname{0.320}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.all\endcsname{0.382}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.all\endcsname{0.334}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.all.gtshare1\endcsname{1.0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.object\endcsname{0.304}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.object.gtshare\endcsname{10\%}
\expandafter\def\csname pn@lab.train.vat.vlmnoleakgtsolo.object.gtshare1\endcsname{10.5\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.object\endcsname{0.323}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.childplay.vlmnoleakgtsolo.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.object\endcsname{0.414}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vacation.vlmnoleakgtsolo.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.object\endcsname{0.342}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.train.all.vlmnoleakgtsolo.object.gtshare1\endcsname{1.8\%}
\expandafter\def\csname pn@pop.val.vat\endcsname{3{,}864}
\expandafter\def\csname pn@copy.val.vat\endcsname{97.8\%}
\expandafter\def\csname pn@pop.val.childplay\endcsname{17{,}534}
\expandafter\def\csname pn@copy.val.childplay\endcsname{78.8\%}
\expandafter\def\csname pn@pop.val.vacation\endcsname{21{,}817}
\expandafter\def\csname pn@copy.val.vacation\endcsname{97.1\%}
\expandafter\def\csname pn@pop.val.all\endcsname{43{,}215}
\expandafter\def\csname pn@copy.val.all\endcsname{89.4\%}
\expandafter\def\csname pn@copy.val.prompted\endcsname{41{,}655}
\expandafter\def\csname pn@lab.val.vat.centre.all\endcsname{0.310}
\expandafter\def\csname pn@lab.val.vat.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.centre.all\endcsname{0.199}
\expandafter\def\csname pn@lab.val.childplay.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.centre.all\endcsname{0.311}
\expandafter\def\csname pn@lab.val.vacation.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.centre.all\endcsname{0.264}
\expandafter\def\csname pn@lab.val.all.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.centre.social\endcsname{0.298}
\expandafter\def\csname pn@lab.val.vat.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.centre.social\endcsname{0.240}
\expandafter\def\csname pn@lab.val.childplay.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.centre.social\endcsname{0.307}
\expandafter\def\csname pn@lab.val.vacation.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.centre.social\endcsname{0.295}
\expandafter\def\csname pn@lab.val.all.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.centre.object\endcsname{0.326}
\expandafter\def\csname pn@lab.val.vat.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.centre.object\endcsname{0.191}
\expandafter\def\csname pn@lab.val.childplay.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.centre.object\endcsname{0.316}
\expandafter\def\csname pn@lab.val.vacation.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.centre.object\endcsname{0.244}
\expandafter\def\csname pn@lab.val.all.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.copyb.all\endcsname{0.161}
\expandafter\def\csname pn@lab.val.vat.copyb.all.gtshare\endcsname{18\%}
\expandafter\def\csname pn@lab.val.vat.copyb.all.gtshare1\endcsname{18.4\%}
\expandafter\def\csname pn@lab.val.childplay.copyb.all\endcsname{0.345}
\expandafter\def\csname pn@lab.val.childplay.copyb.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.copyb.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.copyb.all\endcsname{0.310}
\expandafter\def\csname pn@lab.val.vacation.copyb.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.copyb.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.copyb.all\endcsname{0.314}
\expandafter\def\csname pn@lab.val.all.copyb.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.all.copyb.all.gtshare1\endcsname{1.2\%}
\expandafter\def\csname pn@lab.val.vat.copyb.social\endcsname{0.063}
\expandafter\def\csname pn@lab.val.vat.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.copyb.social\endcsname{0.132}
\expandafter\def\csname pn@lab.val.childplay.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.copyb.social\endcsname{0.143}
\expandafter\def\csname pn@lab.val.vacation.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.copyb.social\endcsname{0.133}
\expandafter\def\csname pn@lab.val.all.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.copyb.object\endcsname{0.299}
\expandafter\def\csname pn@lab.val.vat.copyb.object.gtshare\endcsname{44\%}
\expandafter\def\csname pn@lab.val.vat.copyb.object.gtshare1\endcsname{44.3\%}
\expandafter\def\csname pn@lab.val.childplay.copyb.object\endcsname{0.386}
\expandafter\def\csname pn@lab.val.childplay.copyb.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.copyb.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.copyb.object\endcsname{0.529}
\expandafter\def\csname pn@lab.val.vacation.copyb.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.copyb.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.copyb.object\endcsname{0.435}
\expandafter\def\csname pn@lab.val.all.copyb.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.val.all.copyb.object.gtshare1\endcsname{2.0\%}
\expandafter\def\csname pn@lab.val.vat.mtgs.all\endcsname{0.083}
\expandafter\def\csname pn@lab.val.vat.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.mtgs.all\endcsname{0.090}
\expandafter\def\csname pn@lab.val.childplay.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.mtgs.all\endcsname{0.091}
\expandafter\def\csname pn@lab.val.vacation.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.mtgs.all\endcsname{0.090}
\expandafter\def\csname pn@lab.val.all.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.mtgs.social\endcsname{0.055}
\expandafter\def\csname pn@lab.val.vat.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.mtgs.social\endcsname{0.114}
\expandafter\def\csname pn@lab.val.childplay.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.mtgs.social\endcsname{0.081}
\expandafter\def\csname pn@lab.val.vacation.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.mtgs.social\endcsname{0.087}
\expandafter\def\csname pn@lab.val.all.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.mtgs.object\endcsname{0.122}
\expandafter\def\csname pn@lab.val.vat.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.mtgs.object\endcsname{0.082}
\expandafter\def\csname pn@lab.val.childplay.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.mtgs.object\endcsname{0.104}
\expandafter\def\csname pn@lab.val.vacation.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.mtgs.object\endcsname{0.093}
\expandafter\def\csname pn@lab.val.all.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.ovd_old.all\endcsname{0.180}
\expandafter\def\csname pn@lab.val.vat.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.vat.ovd_old.all.gtshare1\endcsname{0.6\%}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.all\endcsname{0.190}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.all.gtshare1\endcsname{0.5\%}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.all\endcsname{0.207}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.all.gtshare1\endcsname{0.7\%}
\expandafter\def\csname pn@lab.val.all.ovd_old.all\endcsname{0.198}
\expandafter\def\csname pn@lab.val.all.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.all.ovd_old.all.gtshare1\endcsname{0.6\%}
\expandafter\def\csname pn@lab.val.vat.ovd_old.social\endcsname{0.068}
\expandafter\def\csname pn@lab.val.vat.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.social\endcsname{0.180}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.social\endcsname{0.153}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.ovd_old.social\endcsname{0.149}
\expandafter\def\csname pn@lab.val.all.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.ovd_old.object\endcsname{0.339}
\expandafter\def\csname pn@lab.val.vat.ovd_old.object.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.vat.ovd_old.object.gtshare1\endcsname{1.5\%}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.object\endcsname{0.192}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.object.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.childplay.ovd_old.object.gtshare1\endcsname{0.6\%}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.object\endcsname{0.277}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.val.vacation.ovd_old.object.gtshare1\endcsname{1.7\%}
\expandafter\def\csname pn@lab.val.all.ovd_old.object\endcsname{0.231}
\expandafter\def\csname pn@lab.val.all.ovd_old.object.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.all.ovd_old.object.gtshare1\endcsname{1.0\%}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.all\endcsname{0.345}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.all\endcsname{0.204}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.all\endcsname{0.324}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.all\endcsname{0.275}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.object\endcsname{0.344}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.object\endcsname{0.193}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.object\endcsname{0.282}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.object\endcsname{0.233}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.all\endcsname{0.254}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.all.gtshare\endcsname{25\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.all.gtshare1\endcsname{25.5\%}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.all\endcsname{0.095}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.all.gtshare\endcsname{56\%}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.all.gtshare1\endcsname{55.7\%}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.all\endcsname{0.273}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.all.gtshare\endcsname{20\%}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.all.gtshare1\endcsname{19.7\%}
\expandafter\def\csname pn@lab.val.all.ovdgate55.all\endcsname{0.197}
\expandafter\def\csname pn@lab.val.all.ovdgate55.all.gtshare\endcsname{35\%}
\expandafter\def\csname pn@lab.val.all.ovdgate55.all.gtshare1\endcsname{35.1\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.ovdgate55.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.object\endcsname{0.125}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.object.gtshare\endcsname{61\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate55.object.gtshare1\endcsname{61.5\%}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.object\endcsname{0.063}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.object.gtshare\endcsname{66\%}
\expandafter\def\csname pn@lab.val.childplay.ovdgate55.object.gtshare1\endcsname{66.4\%}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.object\endcsname{0.163}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.object.gtshare\endcsname{46\%}
\expandafter\def\csname pn@lab.val.vacation.ovdgate55.object.gtshare1\endcsname{45.7\%}
\expandafter\def\csname pn@lab.val.all.ovdgate55.object\endcsname{0.103}
\expandafter\def\csname pn@lab.val.all.ovdgate55.object.gtshare\endcsname{58\%}
\expandafter\def\csname pn@lab.val.all.ovdgate55.object.gtshare1\endcsname{58.4\%}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.all\endcsname{0.256}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.all.gtshare\endcsname{26\%}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.all.gtshare1\endcsname{26.1\%}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.all\endcsname{0.123}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.all.gtshare\endcsname{42\%}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.all.gtshare1\endcsname{41.8\%}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.all\endcsname{0.267}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.all.gtshare\endcsname{20\%}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.all.gtshare1\endcsname{20.4\%}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.all\endcsname{0.206}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.all.gtshare\endcsname{30\%}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.all.gtshare1\endcsname{29.6\%}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.object\endcsname{0.127}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.object.gtshare\endcsname{63\%}
\expandafter\def\csname pn@lab.val.vat.ovdmixrand.object.gtshare1\endcsname{63.1\%}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.object\endcsname{0.097}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.object.gtshare\endcsname{50\%}
\expandafter\def\csname pn@lab.val.childplay.ovdmixrand.object.gtshare1\endcsname{49.8\%}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.object\endcsname{0.150}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.object.gtshare\endcsname{47\%}
\expandafter\def\csname pn@lab.val.vacation.ovdmixrand.object.gtshare1\endcsname{47.1\%}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.object\endcsname{0.118}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.object.gtshare\endcsname{49\%}
\expandafter\def\csname pn@lab.val.all.ovdmixrand.object.gtshare1\endcsname{49.4\%}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.all\endcsname{0.162}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.all.gtshare\endcsname{18\%}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.all.gtshare1\endcsname{18.4\%}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.all\endcsname{0.331}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.all\endcsname{0.315}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.all\endcsname{0.311}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.all.gtshare1\endcsname{1.2\%}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.social\endcsname{0.067}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.social\endcsname{0.177}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.social\endcsname{0.152}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.social\endcsname{0.148}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.object\endcsname{0.297}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.object.gtshare\endcsname{44\%}
\expandafter\def\csname pn@lab.val.vat.vlmleak_old.object.gtshare1\endcsname{44.3\%}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.object\endcsname{0.360}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmleak_old.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.object\endcsname{0.529}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmleak_old.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.object\endcsname{0.420}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.val.all.vlmleak_old.object.gtshare1\endcsname{2.0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.all\endcsname{0.367}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.all\endcsname{0.268}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.all\endcsname{0.384}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.all\endcsname{0.334}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.object\endcsname{0.398}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.object\endcsname{0.269}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.object\endcsname{0.420}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.object\endcsname{0.331}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.all\endcsname{0.305}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.all.gtshare\endcsname{18\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.all.gtshare1\endcsname{18.4\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.all\endcsname{0.268}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.all\endcsname{0.384}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.all\endcsname{0.330}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.all.gtshare1\endcsname{1.2\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.object\endcsname{0.249}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.object.gtshare\endcsname{44\%}
\expandafter\def\csname pn@lab.val.vat.vlmnoleakgtsolo.object.gtshare1\endcsname{44.3\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.object\endcsname{0.269}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.childplay.vlmnoleakgtsolo.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.object\endcsname{0.420}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vacation.vlmnoleakgtsolo.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.object\endcsname{0.324}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.object.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.val.all.vlmnoleakgtsolo.object.gtshare1\endcsname{2.0\%}
\expandafter\def\csname pn@pop.test.vat\endcsname{26{,}250}
\expandafter\def\csname pn@copy.test.vat\endcsname{96.8\%}
\expandafter\def\csname pn@pop.test.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@copy.test.childplay\endcsname{89.8\%}
\expandafter\def\csname pn@pop.test.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@copy.test.vacation\endcsname{94.3\%}
\expandafter\def\csname pn@pop.test.all\endcsname{58{,}278}
\expandafter\def\csname pn@copy.test.all\endcsname{93.4\%}
\expandafter\def\csname pn@copy.test.prompted\endcsname{50{,}416}
\expandafter\def\csname pn@lab.test.vat.centre.all\endcsname{0.305}
\expandafter\def\csname pn@lab.test.vat.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.centre.all\endcsname{0.288}
\expandafter\def\csname pn@lab.test.childplay.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.centre.all\endcsname{0.284}
\expandafter\def\csname pn@lab.test.vacation.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.centre.all\endcsname{0.294}
\expandafter\def\csname pn@lab.test.all.centre.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.centre.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.centre.social\endcsname{0.297}
\expandafter\def\csname pn@lab.test.vat.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.centre.social\endcsname{0.240}
\expandafter\def\csname pn@lab.test.childplay.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.centre.social\endcsname{0.295}
\expandafter\def\csname pn@lab.test.vacation.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.centre.social\endcsname{0.284}
\expandafter\def\csname pn@lab.test.all.centre.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.centre.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.centre.object\endcsname{0.318}
\expandafter\def\csname pn@lab.test.vat.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.centre.object\endcsname{0.305}
\expandafter\def\csname pn@lab.test.childplay.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.centre.object\endcsname{0.270}
\expandafter\def\csname pn@lab.test.vacation.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.centre.object\endcsname{0.302}
\expandafter\def\csname pn@lab.test.all.centre.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.centre.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.copyb.all\endcsname{0.273}
\expandafter\def\csname pn@lab.test.vat.copyb.all.gtshare\endcsname{6\%}
\expandafter\def\csname pn@lab.test.vat.copyb.all.gtshare1\endcsname{6.0\%}
\expandafter\def\csname pn@lab.test.childplay.copyb.all\endcsname{0.319}
\expandafter\def\csname pn@lab.test.childplay.copyb.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.copyb.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.copyb.all\endcsname{0.244}
\expandafter\def\csname pn@lab.test.vacation.copyb.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.copyb.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.copyb.all\endcsname{0.284}
\expandafter\def\csname pn@lab.test.all.copyb.all.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.test.all.copyb.all.gtshare1\endcsname{2.3\%}
\expandafter\def\csname pn@lab.test.vat.copyb.social\endcsname{0.195}
\expandafter\def\csname pn@lab.test.vat.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.copyb.social\endcsname{0.114}
\expandafter\def\csname pn@lab.test.childplay.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.copyb.social\endcsname{0.058}
\expandafter\def\csname pn@lab.test.vacation.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.copyb.social\endcsname{0.138}
\expandafter\def\csname pn@lab.test.all.copyb.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.copyb.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.copyb.object\endcsname{0.391}
\expandafter\def\csname pn@lab.test.vat.copyb.object.gtshare\endcsname{15\%}
\expandafter\def\csname pn@lab.test.vat.copyb.object.gtshare1\endcsname{15.2\%}
\expandafter\def\csname pn@lab.test.childplay.copyb.object\endcsname{0.391}
\expandafter\def\csname pn@lab.test.childplay.copyb.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.copyb.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.copyb.object\endcsname{0.491}
\expandafter\def\csname pn@lab.test.vacation.copyb.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.copyb.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.copyb.object\endcsname{0.409}
\expandafter\def\csname pn@lab.test.all.copyb.object.gtshare\endcsname{4\%}
\expandafter\def\csname pn@lab.test.all.copyb.object.gtshare1\endcsname{4.2\%}
\expandafter\def\csname pn@lab.test.vat.mtgs.all\endcsname{0.096}
\expandafter\def\csname pn@lab.test.vat.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.mtgs.all\endcsname{0.098}
\expandafter\def\csname pn@lab.test.childplay.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.mtgs.all\endcsname{0.107}
\expandafter\def\csname pn@lab.test.vacation.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.mtgs.all\endcsname{0.099}
\expandafter\def\csname pn@lab.test.all.mtgs.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.mtgs.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.mtgs.social\endcsname{0.072}
\expandafter\def\csname pn@lab.test.vat.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.mtgs.social\endcsname{0.105}
\expandafter\def\csname pn@lab.test.childplay.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.mtgs.social\endcsname{0.076}
\expandafter\def\csname pn@lab.test.vacation.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.mtgs.social\endcsname{0.082}
\expandafter\def\csname pn@lab.test.all.mtgs.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.mtgs.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.mtgs.object\endcsname{0.133}
\expandafter\def\csname pn@lab.test.vat.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.mtgs.object\endcsname{0.094}
\expandafter\def\csname pn@lab.test.childplay.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.mtgs.object\endcsname{0.148}
\expandafter\def\csname pn@lab.test.vacation.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.mtgs.object\endcsname{0.116}
\expandafter\def\csname pn@lab.test.all.mtgs.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.mtgs.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.ovd_old.all\endcsname{0.247}
\expandafter\def\csname pn@lab.test.vat.ovd_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovd_old.all.gtshare1\endcsname{0.4\%}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.all\endcsname{0.202}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.all.gtshare1\endcsname{0.3\%}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.all\endcsname{0.153}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.all.gtshare1\endcsname{1.4\%}
\expandafter\def\csname pn@lab.test.all.ovd_old.all\endcsname{0.208}
\expandafter\def\csname pn@lab.test.all.ovd_old.all.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.test.all.ovd_old.all.gtshare1\endcsname{0.6\%}
\expandafter\def\csname pn@lab.test.vat.ovd_old.social\endcsname{0.204}
\expandafter\def\csname pn@lab.test.vat.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.social\endcsname{0.138}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.social\endcsname{0.070}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.ovd_old.social\endcsname{0.151}
\expandafter\def\csname pn@lab.test.all.ovd_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.ovd_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.ovd_old.object\endcsname{0.313}
\expandafter\def\csname pn@lab.test.vat.ovd_old.object.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.test.vat.ovd_old.object.gtshare1\endcsname{1.0\%}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.object\endcsname{0.224}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovd_old.object.gtshare1\endcsname{0.4\%}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.object\endcsname{0.262}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.object.gtshare\endcsname{3\%}
\expandafter\def\csname pn@lab.test.vacation.ovd_old.object.gtshare1\endcsname{3.2\%}
\expandafter\def\csname pn@lab.test.all.ovd_old.object\endcsname{0.256}
\expandafter\def\csname pn@lab.test.all.ovd_old.object.gtshare\endcsname{1\%}
\expandafter\def\csname pn@lab.test.all.ovd_old.object.gtshare1\endcsname{1.1\%}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.all\endcsname{0.326}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.all\endcsname{0.243}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.all\endcsname{0.310}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.all\endcsname{0.289}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.object\endcsname{0.316}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.object\endcsname{0.225}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.object\endcsname{0.271}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.object\endcsname{0.259}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.ovdalwaysdino.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.all\endcsname{0.257}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.all.gtshare\endcsname{23\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.all.gtshare1\endcsname{23.4\%}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.all\endcsname{0.165}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.all.gtshare\endcsname{38\%}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.all.gtshare1\endcsname{38.2\%}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.all\endcsname{0.263}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.all.gtshare\endcsname{20\%}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.all.gtshare1\endcsname{20.1\%}
\expandafter\def\csname pn@lab.test.all.ovdgate55.all\endcsname{0.222}
\expandafter\def\csname pn@lab.test.all.ovdgate55.all.gtshare\endcsname{28\%}
\expandafter\def\csname pn@lab.test.all.ovdgate55.all.gtshare1\endcsname{28.4\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.ovdgate55.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdgate55.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.ovdgate55.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.object\endcsname{0.143}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.object.gtshare\endcsname{59\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate55.object.gtshare1\endcsname{59.1\%}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.object\endcsname{0.120}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.object.gtshare\endcsname{52\%}
\expandafter\def\csname pn@lab.test.childplay.ovdgate55.object.gtshare1\endcsname{51.6\%}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.object\endcsname{0.161}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.object.gtshare\endcsname{47\%}
\expandafter\def\csname pn@lab.test.vacation.ovdgate55.object.gtshare1\endcsname{46.6\%}
\expandafter\def\csname pn@lab.test.all.ovdgate55.object\endcsname{0.134}
\expandafter\def\csname pn@lab.test.all.ovdgate55.object.gtshare\endcsname{53\%}
\expandafter\def\csname pn@lab.test.all.ovdgate55.object.gtshare1\endcsname{52.8\%}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.all\endcsname{0.246}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.all.gtshare\endcsname{25\%}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.all.gtshare1\endcsname{25.2\%}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.all\endcsname{0.160}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.all.gtshare\endcsname{37\%}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.all.gtshare1\endcsname{37.1\%}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.all\endcsname{0.255}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.all.gtshare\endcsname{20\%}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.all.gtshare1\endcsname{19.8\%}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.all\endcsname{0.214}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.all.gtshare\endcsname{29\%}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.all.gtshare1\endcsname{28.6\%}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.object\endcsname{0.113}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.object.gtshare\endcsname{64\%}
\expandafter\def\csname pn@lab.test.vat.ovdmixrand.object.gtshare1\endcsname{63.7\%}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.object\endcsname{0.113}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.object.gtshare\endcsname{50\%}
\expandafter\def\csname pn@lab.test.childplay.ovdmixrand.object.gtshare1\endcsname{50.1\%}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.object\endcsname{0.142}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.object.gtshare\endcsname{46\%}
\expandafter\def\csname pn@lab.test.vacation.ovdmixrand.object.gtshare1\endcsname{45.9\%}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.object\endcsname{0.118}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.object.gtshare\endcsname{53\%}
\expandafter\def\csname pn@lab.test.all.ovdmixrand.object.gtshare1\endcsname{53.1\%}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.all\endcsname{0.276}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.all.gtshare\endcsname{6\%}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.all.gtshare1\endcsname{6.0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.all\endcsname{0.325}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.all\endcsname{0.237}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.all\endcsname{0.286}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.all.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.all.gtshare1\endcsname{2.3\%}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.social\endcsname{0.202}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.social\endcsname{0.135}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.social\endcsname{0.069}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.social\endcsname{0.149}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.object\endcsname{0.390}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.object.gtshare\endcsname{15\%}
\expandafter\def\csname pn@lab.test.vat.vlmleak_old.object.gtshare1\endcsname{15.2\%}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.object\endcsname{0.391}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmleak_old.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.object\endcsname{0.458}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmleak_old.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.object\endcsname{0.403}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.object.gtshare\endcsname{4\%}
\expandafter\def\csname pn@lab.test.all.vlmleak_old.object.gtshare1\endcsname{4.2\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.all\endcsname{0.335}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.all\endcsname{0.323}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.all\endcsname{0.351}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.all\endcsname{0.334}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.object\endcsname{0.340}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.object\endcsname{0.334}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.object\endcsname{0.369}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.object\endcsname{0.342}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleak.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.all\endcsname{0.315}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.all.gtshare\endcsname{6\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.all.gtshare1\endcsname{6.0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.all\endcsname{0.323}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.all\endcsname{0.351}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.all.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.all.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.all\endcsname{0.326}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.all.gtshare\endcsname{2\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.all.gtshare1\endcsname{2.3\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.social.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.object\endcsname{0.288}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.object.gtshare\endcsname{15\%}
\expandafter\def\csname pn@lab.test.vat.vlmnoleakgtsolo.object.gtshare1\endcsname{15.2\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.object\endcsname{0.334}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.childplay.vlmnoleakgtsolo.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.object\endcsname{0.369}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.object.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vacation.vlmnoleakgtsolo.object.gtshare1\endcsname{0.0\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.object\endcsname{0.328}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.object.gtshare\endcsname{4\%}
\expandafter\def\csname pn@lab.test.all.vlmnoleakgtsolo.object.gtshare1\endcsname{4.2\%}
\expandafter\def\csname pn@gate.rate.vat\endcsname{64\%}
\expandafter\def\csname pn@matched.train.vat\endcsname{100{,}360}
\expandafter\def\csname pn@matched.share.vat\endcsname{96.6\%}
\expandafter\def\csname pn@unmatched.train.vat\endcsname{3{,}517}
\expandafter\def\csname pn@unmatched.share.vat\endcsname{3.4\%}
\expandafter\def\csname pn@gate.rate.childplay\endcsname{50\%}
\expandafter\def\csname pn@matched.train.childplay\endcsname{151{,}415}
\expandafter\def\csname pn@matched.share.childplay\endcsname{100.0\%}
\expandafter\def\csname pn@unmatched.train.childplay\endcsname{0}
\expandafter\def\csname pn@unmatched.share.childplay\endcsname{0.0\%}
\expandafter\def\csname pn@gate.rate.vacation\endcsname{47\%}
\expandafter\def\csname pn@matched.train.vacation\endcsname{105{,}753}
\expandafter\def\csname pn@matched.share.vacation\endcsname{100.0\%}
\expandafter\def\csname pn@unmatched.train.vacation\endcsname{0}
\expandafter\def\csname pn@unmatched.share.vacation\endcsname{0.0\%}
\expandafter\def\csname pn@lab.train.vat.gazelle.all\endcsname{0.100}
\expandafter\def\csname pn@lab.train.vat.gazelle.social\endcsname{0.068}
\expandafter\def\csname pn@lab.train.vat.gazelle.object\endcsname{0.145}
\expandafter\def\csname pn@lab.train.vat.gazelle.n\endcsname{80{,}988}
\expandafter\def\csname pn@lab.val.vat.gazelle.all\endcsname{0.082}
\expandafter\def\csname pn@lab.val.vat.gazelle.social\endcsname{0.047}
\expandafter\def\csname pn@lab.val.vat.gazelle.object\endcsname{0.131}
\expandafter\def\csname pn@lab.val.vat.gazelle.n\endcsname{2{,}819}
\expandafter\def\csname pn@lab.test.vat.gazelle.all\endcsname{0.106}
\expandafter\def\csname pn@lab.test.vat.gazelle.social\endcsname{0.076}
\expandafter\def\csname pn@lab.test.vat.gazelle.object\endcsname{0.152}
\expandafter\def\csname pn@lab.test.vat.gazelle.n\endcsname{19{,}563}
\expandafter\def\csname pn@lab.train.childplay.gazelle.all\endcsname{0.109}
\expandafter\def\csname pn@lab.train.childplay.gazelle.social\endcsname{0.095}
\expandafter\def\csname pn@lab.train.childplay.gazelle.object\endcsname{0.114}
\expandafter\def\csname pn@lab.train.childplay.gazelle.n\endcsname{151{,}415}
\expandafter\def\csname pn@lab.val.childplay.gazelle.all\endcsname{0.095}
\expandafter\def\csname pn@lab.val.childplay.gazelle.social\endcsname{0.141}
\expandafter\def\csname pn@lab.val.childplay.gazelle.object\endcsname{0.087}
\expandafter\def\csname pn@lab.val.childplay.gazelle.n\endcsname{17{,}534}
\expandafter\def\csname pn@lab.test.childplay.gazelle.all\endcsname{0.115}
\expandafter\def\csname pn@lab.test.childplay.gazelle.social\endcsname{0.106}
\expandafter\def\csname pn@lab.test.childplay.gazelle.object\endcsname{0.119}
\expandafter\def\csname pn@lab.test.childplay.gazelle.n\endcsname{20{,}100}
\expandafter\def\csname pn@lab.train.vacation.gazelle.all\endcsname{0.118}
\expandafter\def\csname pn@lab.train.vacation.gazelle.object\endcsname{0.132}
\expandafter\def\csname pn@lab.train.vacation.gazelle.social\endcsname{0.106}
\expandafter\def\csname pn@lab.train.vacation.gazelle.n\endcsname{105{,}753}
\expandafter\def\csname pn@lab.val.vacation.gazelle.all\endcsname{0.112}
\expandafter\def\csname pn@lab.val.vacation.gazelle.social\endcsname{0.096}
\expandafter\def\csname pn@lab.val.vacation.gazelle.object\endcsname{0.132}
\expandafter\def\csname pn@lab.val.vacation.gazelle.n\endcsname{21{,}817}
\expandafter\def\csname pn@lab.test.vacation.gazelle.all\endcsname{0.124}
\expandafter\def\csname pn@lab.test.vacation.gazelle.social\endcsname{0.116}
\expandafter\def\csname pn@lab.test.vacation.gazelle.object\endcsname{0.136}
\expandafter\def\csname pn@lab.test.vacation.gazelle.n\endcsname{11{,}928}
\expandafter\def\csname pn@lab.train.all.gazelle.all\endcsname{0.110}
\expandafter\def\csname pn@lab.train.all.gazelle.social\endcsname{0.090}
\expandafter\def\csname pn@lab.train.all.gazelle.object\endcsname{0.124}
\expandafter\def\csname pn@lab.val.all.gazelle.all\endcsname{0.103}
\expandafter\def\csname pn@lab.val.all.gazelle.social\endcsname{0.099}
\expandafter\def\csname pn@lab.val.all.gazelle.object\endcsname{0.106}
\expandafter\def\csname pn@lab.test.all.gazelle.all\endcsname{0.114}
\expandafter\def\csname pn@lab.test.all.gazelle.social\endcsname{0.094}
\expandafter\def\csname pn@lab.test.all.gazelle.object\endcsname{0.131}
\expandafter\def\csname pn@lab.train.vat.ovdgate40.all\endcsname{0.267}
\expandafter\def\csname pn@lab.train.childplay.ovdgate40.all\endcsname{0.253}
\expandafter\def\csname pn@lab.train.vacation.ovdgate40.all\endcsname{0.308}
\expandafter\def\csname pn@lab.train.all.ovdgate40.all\endcsname{0.273}
\expandafter\def\csname pn@lab.train.all.ovdgate40.all.gtshare\endcsname{9\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate40.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.childplay.ovdgate40.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.vacation.ovdgate40.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.all.ovdgate40.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdgate40.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate40.object\endcsname{0.233}
\expandafter\def\csname pn@lab.train.childplay.ovdgate40.object\endcsname{0.233}
\expandafter\def\csname pn@lab.train.vacation.ovdgate40.object\endcsname{0.249}
\expandafter\def\csname pn@lab.train.all.ovdgate40.object\endcsname{0.237}
\expandafter\def\csname pn@lab.train.all.ovdgate40.object.gtshare\endcsname{16\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate48.all\endcsname{0.238}
\expandafter\def\csname pn@lab.train.childplay.ovdgate48.all\endcsname{0.217}
\expandafter\def\csname pn@lab.train.vacation.ovdgate48.all\endcsname{0.285}
\expandafter\def\csname pn@lab.train.all.ovdgate48.all\endcsname{0.243}
\expandafter\def\csname pn@lab.train.all.ovdgate48.all.gtshare\endcsname{21\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate48.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.childplay.ovdgate48.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.vacation.ovdgate48.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.all.ovdgate48.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdgate48.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate48.object\endcsname{0.163}
\expandafter\def\csname pn@lab.train.childplay.ovdgate48.object\endcsname{0.185}
\expandafter\def\csname pn@lab.train.vacation.ovdgate48.object\endcsname{0.200}
\expandafter\def\csname pn@lab.train.all.ovdgate48.object\endcsname{0.185}
\expandafter\def\csname pn@lab.train.all.ovdgate48.object.gtshare\endcsname{36\%}
\expandafter\def\csname pn@lab.train.vat.ovdmix40.all\endcsname{0.267}
\expandafter\def\csname pn@lab.train.childplay.ovdmix40.all\endcsname{0.248}
\expandafter\def\csname pn@lab.train.vacation.ovdmix40.all\endcsname{0.306}
\expandafter\def\csname pn@lab.train.all.ovdmix40.all\endcsname{0.271}
\expandafter\def\csname pn@lab.train.all.ovdmix40.all.gtshare\endcsname{10\%}
\expandafter\def\csname pn@lab.train.vat.ovdmix40.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.childplay.ovdmix40.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.vacation.ovdmix40.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.all.ovdmix40.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdmix40.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdmix40.object\endcsname{0.232}
\expandafter\def\csname pn@lab.train.childplay.ovdmix40.object\endcsname{0.228}
\expandafter\def\csname pn@lab.train.vacation.ovdmix40.object\endcsname{0.245}
\expandafter\def\csname pn@lab.train.all.ovdmix40.object\endcsname{0.233}
\expandafter\def\csname pn@lab.train.all.ovdmix40.object.gtshare\endcsname{17\%}
\expandafter\def\csname pn@lab.train.vat.ovdmix48.all\endcsname{0.236}
\expandafter\def\csname pn@lab.train.childplay.ovdmix48.all\endcsname{0.210}
\expandafter\def\csname pn@lab.train.vacation.ovdmix48.all\endcsname{0.284}
\expandafter\def\csname pn@lab.train.all.ovdmix48.all\endcsname{0.240}
\expandafter\def\csname pn@lab.train.all.ovdmix48.all.gtshare\endcsname{21\%}
\expandafter\def\csname pn@lab.train.vat.ovdmix48.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.childplay.ovdmix48.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.vacation.ovdmix48.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.all.ovdmix48.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdmix48.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdmix48.object\endcsname{0.158}
\expandafter\def\csname pn@lab.train.childplay.ovdmix48.object\endcsname{0.177}
\expandafter\def\csname pn@lab.train.vacation.ovdmix48.object\endcsname{0.197}
\expandafter\def\csname pn@lab.train.all.ovdmix48.object\endcsname{0.179}
\expandafter\def\csname pn@lab.train.all.ovdmix48.object.gtshare\endcsname{37\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate40.all\endcsname{0.343}
\expandafter\def\csname pn@lab.val.childplay.ovdgate40.all\endcsname{0.166}
\expandafter\def\csname pn@lab.val.vacation.ovdgate40.all\endcsname{0.314}
\expandafter\def\csname pn@lab.val.all.ovdgate40.all\endcsname{0.254}
\expandafter\def\csname pn@lab.val.all.ovdgate40.all.gtshare\endcsname{12\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate40.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.childplay.ovdgate40.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.vacation.ovdgate40.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.all.ovdgate40.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdgate40.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate40.object\endcsname{0.340}
\expandafter\def\csname pn@lab.val.childplay.ovdgate40.object\endcsname{0.147}
\expandafter\def\csname pn@lab.val.vacation.ovdgate40.object\endcsname{0.258}
\expandafter\def\csname pn@lab.val.all.ovdgate40.object\endcsname{0.197}
\expandafter\def\csname pn@lab.val.all.ovdgate40.object.gtshare\endcsname{19\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate48.all\endcsname{0.312}
\expandafter\def\csname pn@lab.val.childplay.ovdgate48.all\endcsname{0.121}
\expandafter\def\csname pn@lab.val.vacation.ovdgate48.all\endcsname{0.293}
\expandafter\def\csname pn@lab.val.all.ovdgate48.all\endcsname{0.223}
\expandafter\def\csname pn@lab.val.all.ovdgate48.all.gtshare\endcsname{25\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate48.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.childplay.ovdgate48.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.vacation.ovdgate48.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.all.ovdgate48.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdgate48.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate48.object\endcsname{0.264}
\expandafter\def\csname pn@lab.val.childplay.ovdgate48.object\endcsname{0.094}
\expandafter\def\csname pn@lab.val.vacation.ovdgate48.object\endcsname{0.211}
\expandafter\def\csname pn@lab.val.all.ovdgate48.object\endcsname{0.145}
\expandafter\def\csname pn@lab.val.all.ovdgate48.object.gtshare\endcsname{42\%}
\expandafter\def\csname pn@lab.val.vat.ovdmix40.all\endcsname{0.319}
\expandafter\def\csname pn@lab.val.childplay.ovdmix40.all\endcsname{0.178}
\expandafter\def\csname pn@lab.val.vacation.ovdmix40.all\endcsname{0.312}
\expandafter\def\csname pn@lab.val.all.ovdmix40.all\endcsname{0.256}
\expandafter\def\csname pn@lab.val.all.ovdmix40.all.gtshare\endcsname{9\%}
\expandafter\def\csname pn@lab.val.vat.ovdmix40.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.childplay.ovdmix40.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.vacation.ovdmix40.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.all.ovdmix40.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdmix40.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdmix40.object\endcsname{0.282}
\expandafter\def\csname pn@lab.val.childplay.ovdmix40.object\endcsname{0.161}
\expandafter\def\csname pn@lab.val.vacation.ovdmix40.object\endcsname{0.254}
\expandafter\def\csname pn@lab.val.all.ovdmix40.object\endcsname{0.201}
\expandafter\def\csname pn@lab.val.all.ovdmix40.object.gtshare\endcsname{15\%}
\expandafter\def\csname pn@lab.val.vat.ovdmix48.all\endcsname{0.284}
\expandafter\def\csname pn@lab.val.childplay.ovdmix48.all\endcsname{0.147}
\expandafter\def\csname pn@lab.val.vacation.ovdmix48.all\endcsname{0.289}
\expandafter\def\csname pn@lab.val.all.ovdmix48.all\endcsname{0.229}
\expandafter\def\csname pn@lab.val.all.ovdmix48.all.gtshare\endcsname{21\%}
\expandafter\def\csname pn@lab.val.vat.ovdmix48.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.childplay.ovdmix48.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.vacation.ovdmix48.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.all.ovdmix48.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdmix48.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdmix48.object\endcsname{0.198}
\expandafter\def\csname pn@lab.val.childplay.ovdmix48.object\endcsname{0.125}
\expandafter\def\csname pn@lab.val.vacation.ovdmix48.object\endcsname{0.201}
\expandafter\def\csname pn@lab.val.all.ovdmix48.object\endcsname{0.156}
\expandafter\def\csname pn@lab.val.all.ovdmix48.object.gtshare\endcsname{34\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate40.all\endcsname{0.307}
\expandafter\def\csname pn@lab.test.childplay.ovdgate40.all\endcsname{0.228}
\expandafter\def\csname pn@lab.test.vacation.ovdgate40.all\endcsname{0.311}
\expandafter\def\csname pn@lab.test.all.ovdgate40.all\endcsname{0.277}
\expandafter\def\csname pn@lab.test.all.ovdgate40.all.gtshare\endcsname{9\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate40.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.childplay.ovdgate40.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.vacation.ovdgate40.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.all.ovdgate40.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdgate40.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate40.object\endcsname{0.269}
\expandafter\def\csname pn@lab.test.childplay.ovdgate40.object\endcsname{0.206}
\expandafter\def\csname pn@lab.test.vacation.ovdgate40.object\endcsname{0.276}
\expandafter\def\csname pn@lab.test.all.ovdgate40.object\endcsname{0.237}
\expandafter\def\csname pn@lab.test.all.ovdgate40.object.gtshare\endcsname{16\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate48.all\endcsname{0.281}
\expandafter\def\csname pn@lab.test.childplay.ovdgate48.all\endcsname{0.189}
\expandafter\def\csname pn@lab.test.vacation.ovdgate48.all\endcsname{0.298}
\expandafter\def\csname pn@lab.test.all.ovdgate48.all\endcsname{0.249}
\expandafter\def\csname pn@lab.test.all.ovdgate48.all.gtshare\endcsname{21\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate48.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.childplay.ovdgate48.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.vacation.ovdgate48.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.all.ovdgate48.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdgate48.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate48.object\endcsname{0.204}
\expandafter\def\csname pn@lab.test.childplay.ovdgate48.object\endcsname{0.152}
\expandafter\def\csname pn@lab.test.vacation.ovdgate48.object\endcsname{0.245}
\expandafter\def\csname pn@lab.test.all.ovdgate48.object\endcsname{0.184}
\expandafter\def\csname pn@lab.test.all.ovdgate48.object.gtshare\endcsname{38\%}
\expandafter\def\csname pn@lab.test.vat.ovdmix40.all\endcsname{0.297}
\expandafter\def\csname pn@lab.test.childplay.ovdmix40.all\endcsname{0.220}
\expandafter\def\csname pn@lab.test.vacation.ovdmix40.all\endcsname{0.321}
\expandafter\def\csname pn@lab.test.all.ovdmix40.all\endcsname{0.272}
\expandafter\def\csname pn@lab.test.all.ovdmix40.all.gtshare\endcsname{10\%}
\expandafter\def\csname pn@lab.test.vat.ovdmix40.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.childplay.ovdmix40.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.vacation.ovdmix40.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.all.ovdmix40.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdmix40.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdmix40.object\endcsname{0.243}
\expandafter\def\csname pn@lab.test.childplay.ovdmix40.object\endcsname{0.194}
\expandafter\def\csname pn@lab.test.vacation.ovdmix40.object\endcsname{0.299}
\expandafter\def\csname pn@lab.test.all.ovdmix40.object\endcsname{0.227}
\expandafter\def\csname pn@lab.test.all.ovdmix40.object.gtshare\endcsname{18\%}
\expandafter\def\csname pn@lab.test.vat.ovdmix48.all\endcsname{0.267}
\expandafter\def\csname pn@lab.test.childplay.ovdmix48.all\endcsname{0.189}
\expandafter\def\csname pn@lab.test.vacation.ovdmix48.all\endcsname{0.298}
\expandafter\def\csname pn@lab.test.all.ovdmix48.all\endcsname{0.244}
\expandafter\def\csname pn@lab.test.all.ovdmix48.all.gtshare\endcsname{21\%}
\expandafter\def\csname pn@lab.test.vat.ovdmix48.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.childplay.ovdmix48.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.vacation.ovdmix48.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.all.ovdmix48.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdmix48.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdmix48.object\endcsname{0.168}
\expandafter\def\csname pn@lab.test.childplay.ovdmix48.object\endcsname{0.152}
\expandafter\def\csname pn@lab.test.vacation.ovdmix48.object\endcsname{0.246}
\expandafter\def\csname pn@lab.test.all.ovdmix48.object\endcsname{0.174}
\expandafter\def\csname pn@lab.test.all.ovdmix48.object.gtshare\endcsname{38\%}
\expandafter\def\csname pn@gate.rate40.vat\endcsname{27\%}
\expandafter\def\csname pn@gate.rate40.childplay\endcsname{16\%}
\expandafter\def\csname pn@gate.rate40.vacation\endcsname{12\%}
\expandafter\def\csname pn@gate.rate40.all\endcsname{17\%}
\expandafter\def\csname pn@gate.rate48.vat\endcsname{52\%}
\expandafter\def\csname pn@gate.rate48.childplay\endcsname{35\%}
\expandafter\def\csname pn@gate.rate48.vacation\endcsname{31\%}
\expandafter\def\csname pn@gate.rate48.all\endcsname{37\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate100.all\endcsname{0.179}
\expandafter\def\csname pn@lab.train.childplay.ovdgate100.all\endcsname{0.081}
\expandafter\def\csname pn@lab.train.vacation.ovdgate100.all\endcsname{0.210}
\expandafter\def\csname pn@lab.train.all.ovdgate100.all\endcsname{0.145}
\expandafter\def\csname pn@lab.train.all.ovdgate100.all.gtshare\endcsname{57\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate100.social\endcsname{0.292}
\expandafter\def\csname pn@lab.train.childplay.ovdgate100.social\endcsname{0.309}
\expandafter\def\csname pn@lab.train.vacation.ovdgate100.social\endcsname{0.356}
\expandafter\def\csname pn@lab.train.all.ovdgate100.social\endcsname{0.322}
\expandafter\def\csname pn@lab.train.all.ovdgate100.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.train.vat.ovdgate100.object\endcsname{0.019}
\expandafter\def\csname pn@lab.train.childplay.ovdgate100.object\endcsname{0.004}
\expandafter\def\csname pn@lab.train.vacation.ovdgate100.object\endcsname{0.032}
\expandafter\def\csname pn@lab.train.all.ovdgate100.object\endcsname{0.014}
\expandafter\def\csname pn@lab.train.all.ovdgate100.object.gtshare\endcsname{99\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate100.all\endcsname{0.214}
\expandafter\def\csname pn@lab.val.childplay.ovdgate100.all\endcsname{0.042}
\expandafter\def\csname pn@lab.val.vacation.ovdgate100.all\endcsname{0.205}
\expandafter\def\csname pn@lab.val.all.ovdgate100.all\endcsname{0.138}
\expandafter\def\csname pn@lab.val.all.ovdgate100.all.gtshare\endcsname{60\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate100.social\endcsname{0.345}
\expandafter\def\csname pn@lab.val.childplay.ovdgate100.social\endcsname{0.262}
\expandafter\def\csname pn@lab.val.vacation.ovdgate100.social\endcsname{0.356}
\expandafter\def\csname pn@lab.val.all.ovdgate100.social\endcsname{0.339}
\expandafter\def\csname pn@lab.val.all.ovdgate100.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.val.vat.ovdgate100.object\endcsname{0.030}
\expandafter\def\csname pn@lab.val.childplay.ovdgate100.object\endcsname{0.000}
\expandafter\def\csname pn@lab.val.vacation.ovdgate100.object\endcsname{0.007}
\expandafter\def\csname pn@lab.val.all.ovdgate100.object\endcsname{0.004}
\expandafter\def\csname pn@lab.val.all.ovdgate100.object.gtshare\endcsname{100\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate100.all\endcsname{0.207}
\expandafter\def\csname pn@lab.test.childplay.ovdgate100.all\endcsname{0.079}
\expandafter\def\csname pn@lab.test.vacation.ovdgate100.all\endcsname{0.220}
\expandafter\def\csname pn@lab.test.all.ovdgate100.all\endcsname{0.160}
\expandafter\def\csname pn@lab.test.all.ovdgate100.all.gtshare\endcsname{53\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate100.social\endcsname{0.332}
\expandafter\def\csname pn@lab.test.childplay.ovdgate100.social\endcsname{0.293}
\expandafter\def\csname pn@lab.test.vacation.ovdgate100.social\endcsname{0.338}
\expandafter\def\csname pn@lab.test.all.ovdgate100.social\endcsname{0.325}
\expandafter\def\csname pn@lab.test.all.ovdgate100.social.gtshare\endcsname{0\%}
\expandafter\def\csname pn@lab.test.vat.ovdgate100.object\endcsname{0.015}
\expandafter\def\csname pn@lab.test.childplay.ovdgate100.object\endcsname{0.004}
\expandafter\def\csname pn@lab.test.vacation.ovdgate100.object\endcsname{0.065}
\expandafter\def\csname pn@lab.test.all.ovdgate100.object\endcsname{0.019}
\expandafter\def\csname pn@lab.test.all.ovdgate100.object.gtshare\endcsname{99\%}
\expandafter\def\csname pn@gate.rate100.vat\endcsname{100\%}
\expandafter\def\csname pn@gate.rate100.childplay\endcsname{100\%}
\expandafter\def\csname pn@gate.rate100.vacation\endcsname{100\%}
\expandafter\def\csname pn@gate.rate100.all\endcsname{100\%}
\expandafter\def\csname pn@gate.rate55.all\endcsname{52\%}
\expandafter\def\csname pn@gate.rate55.vat\endcsname{64\%}
\expandafter\def\csname pn@gate.rate55.childplay\endcsname{50\%}
\expandafter\def\csname pn@gate.rate55.vacation\endcsname{47\%}
\expandafter\def\csname pn@lab.gap.vat.mtgs\endcsname{0.022}
\expandafter\def\csname pn@lab.gap.childplay.mtgs\endcsname{0.022}
\expandafter\def\csname pn@lab.gap.vacation.mtgs\endcsname{0.007}
\expandafter\def\csname pn@lab.gap.all.mtgs\endcsname{0.016}
\expandafter\def\csname pn@lab.gap.vat.gazelle\endcsname{0.006}
\expandafter\def\csname pn@lab.gap.childplay.gazelle\endcsname{0.006}
\expandafter\def\csname pn@lab.gap.vacation.gazelle\endcsname{0.007}
\expandafter\def\csname pn@lab.gap.all.gazelle\endcsname{0.004}
\expandafter\def\csname pn@lab.gap.vat.centre\endcsname{0.030}
\expandafter\def\csname pn@lab.gap.childplay.centre\endcsname{0.032}
\expandafter\def\csname pn@lab.gap.vacation.centre\endcsname{-0.016}
\expandafter\def\csname pn@lab.gap.all.centre\endcsname{0.019}
\expandafter\def\csname pn@lab.gap.vat.vlmleak_old\endcsname{0.026}
\expandafter\def\csname pn@lab.gap.childplay.vlmleak_old\endcsname{-0.035}
\expandafter\def\csname pn@lab.gap.vacation.vlmleak_old\endcsname{-0.030}
\expandafter\def\csname pn@lab.gap.all.vlmleak_old\endcsname{-0.019}
\expandafter\def\csname pn@lab.gap.vat.vlmnoleak\endcsname{0.022}
\expandafter\def\csname pn@lab.gap.childplay.vlmnoleak\endcsname{0.003}
\expandafter\def\csname pn@lab.gap.vacation.vlmnoleak\endcsname{-0.031}
\expandafter\def\csname pn@lab.gap.all.vlmnoleak\endcsname{-0.004}
\expandafter\def\csname pn@lab.gap.vat.ovdalwaysdino\endcsname{0.033}
\expandafter\def\csname pn@lab.gap.childplay.ovdalwaysdino\endcsname{-0.035}
\expandafter\def\csname pn@lab.gap.vacation.ovdalwaysdino\endcsname{0.003}
\expandafter\def\csname pn@lab.gap.all.ovdalwaysdino\endcsname{-0.001}
\expandafter\def\csname pn@st.tiny.gt.pooled\endcsname{0.208}
\expandafter\def\csname pn@st.tiny.gt.pooled4\endcsname{0.2079}
\expandafter\def\csname pn@st.tiny.gt.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.gt.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.gt.pck05\endcsname{0.055}
\expandafter\def\csname pn@st.tiny.gt.pck10\endcsname{0.201}
\expandafter\def\csname pn@st.tiny.gt.vat\endcsname{0.215}
\expandafter\def\csname pn@st.tiny.gt.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.gt.childplay\endcsname{0.192}
\expandafter\def\csname pn@st.tiny.gt.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.gt.vacation\endcsname{0.223}
\expandafter\def\csname pn@st.tiny.gt.vacation.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gt.social\endcsname{0.178}
\expandafter\def\csname pn@st.tiny.gt.social.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.gt.object\endcsname{0.233}
\expandafter\def\csname pn@st.tiny.gt.object.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gt.collapse.min\endcsname{0.76}
\expandafter\def\csname pn@st.tiny.gt.collapse.max\endcsname{0.83}
\expandafter\def\csname pn@st.tiny.gt.collapse.mean\endcsname{0.80}
\expandafter\def\csname pn@st.tiny.gt.epochs\endcsname{3, 8, 4}
\expandafter\def\csname pn@st.tiny.gt.epoch.max\endcsname{8}
\expandafter\def\csname pn@st.tiny.gt.epoch.min\endcsname{3}
\expandafter\def\csname pn@st.tiny.gt.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.gt.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.gt.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.gt.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.gt.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.gt.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.gt.gtsel.pooled\endcsname{0.208}
\expandafter\def\csname pn@st.tiny.gt.gtsel.pooled4\endcsname{0.2079}
\expandafter\def\csname pn@st.tiny.gt.gtsel.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.gt.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.gt.gtsel.pck05\endcsname{0.055}
\expandafter\def\csname pn@st.tiny.gt.gtsel.pck10\endcsname{0.201}
\expandafter\def\csname pn@st.tiny.gt.gtsel.vat\endcsname{0.215}
\expandafter\def\csname pn@st.tiny.gt.gtsel.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.gt.gtsel.childplay\endcsname{0.192}
\expandafter\def\csname pn@st.tiny.gt.gtsel.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.gt.gtsel.vacation\endcsname{0.223}
\expandafter\def\csname pn@st.tiny.gt.gtsel.vacation.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gt.gtsel.social\endcsname{0.178}
\expandafter\def\csname pn@st.tiny.gt.gtsel.social.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.gt.gtsel.object\endcsname{0.233}
\expandafter\def\csname pn@st.tiny.gt.gtsel.object.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gt.gtsel.collapse.min\endcsname{0.76}
\expandafter\def\csname pn@st.tiny.gt.gtsel.collapse.max\endcsname{0.83}
\expandafter\def\csname pn@st.tiny.gt.gtsel.collapse.mean\endcsname{0.80}
\expandafter\def\csname pn@st.tiny.gt.gtsel.epochs\endcsname{3, 8, 4}
\expandafter\def\csname pn@st.tiny.gt.gtsel.epoch.max\endcsname{8}
\expandafter\def\csname pn@st.tiny.gt.gtsel.epoch.min\endcsname{3}
\expandafter\def\csname pn@st.tiny.gt.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.gt.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.gt.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.gt.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.gt.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.gt.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.gt.val.vslabels\endcsname{0.210}
\expandafter\def\csname pn@st.tiny.gt.val.vsgt\endcsname{0.210}
\expandafter\def\csname pn@st.tiny.mtgs.pooled\endcsname{0.204}
\expandafter\def\csname pn@st.tiny.mtgs.pooled4\endcsname{0.2038}
\expandafter\def\csname pn@st.tiny.mtgs.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.mtgs.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.mtgs.pck05\endcsname{0.059}
\expandafter\def\csname pn@st.tiny.mtgs.pck10\endcsname{0.215}
\expandafter\def\csname pn@st.tiny.mtgs.vat\endcsname{0.208}
\expandafter\def\csname pn@st.tiny.mtgs.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.mtgs.childplay\endcsname{0.192}
\expandafter\def\csname pn@st.tiny.mtgs.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.mtgs.vacation\endcsname{0.216}
\expandafter\def\csname pn@st.tiny.mtgs.vacation.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.mtgs.social\endcsname{0.168}
\expandafter\def\csname pn@st.tiny.mtgs.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.mtgs.object\endcsname{0.234}
\expandafter\def\csname pn@st.tiny.mtgs.object.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.mtgs.collapse.min\endcsname{0.82}
\expandafter\def\csname pn@st.tiny.mtgs.collapse.max\endcsname{0.84}
\expandafter\def\csname pn@st.tiny.mtgs.collapse.mean\endcsname{0.83}
\expandafter\def\csname pn@st.tiny.mtgs.epochs\endcsname{13, 11, 11}
\expandafter\def\csname pn@st.tiny.mtgs.epoch.max\endcsname{13}
\expandafter\def\csname pn@st.tiny.mtgs.epoch.min\endcsname{11}
\expandafter\def\csname pn@st.tiny.mtgs.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.mtgs.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.mtgs.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.mtgs.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.mtgs.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.mtgs.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.pooled\endcsname{0.204}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.pooled4\endcsname{0.2040}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.pck05\endcsname{0.060}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.pck10\endcsname{0.215}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.vat\endcsname{0.209}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.childplay\endcsname{0.191}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.vacation\endcsname{0.218}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.vacation.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.social\endcsname{0.167}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.object\endcsname{0.236}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.object.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.collapse.min\endcsname{0.82}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.collapse.max\endcsname{0.86}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.collapse.mean\endcsname{0.84}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.epochs\endcsname{13, 14, 11}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.epoch.max\endcsname{14}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.epoch.min\endcsname{11}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.mtgs.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.mtgs.val.vslabels\endcsname{0.185}
\expandafter\def\csname pn@st.tiny.mtgs.val.vsgt\endcsname{0.201}
\expandafter\def\csname pn@st.tiny.gazelle.pooled\endcsname{0.204}
\expandafter\def\csname pn@st.tiny.gazelle.pooled4\endcsname{0.2038}
\expandafter\def\csname pn@st.tiny.gazelle.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.gazelle.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.gazelle.pck05\endcsname{0.056}
\expandafter\def\csname pn@st.tiny.gazelle.pck10\endcsname{0.213}
\expandafter\def\csname pn@st.tiny.gazelle.vat\endcsname{0.209}
\expandafter\def\csname pn@st.tiny.gazelle.vat.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.gazelle.childplay\endcsname{0.191}
\expandafter\def\csname pn@st.tiny.gazelle.childplay.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gazelle.vacation\endcsname{0.217}
\expandafter\def\csname pn@st.tiny.gazelle.vacation.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gazelle.social\endcsname{0.171}
\expandafter\def\csname pn@st.tiny.gazelle.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.gazelle.object\endcsname{0.232}
\expandafter\def\csname pn@st.tiny.gazelle.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.gazelle.collapse.min\endcsname{0.80}
\expandafter\def\csname pn@st.tiny.gazelle.collapse.max\endcsname{0.82}
\expandafter\def\csname pn@st.tiny.gazelle.collapse.mean\endcsname{0.81}
\expandafter\def\csname pn@st.tiny.gazelle.epochs\endcsname{11, 11, 13}
\expandafter\def\csname pn@st.tiny.gazelle.epoch.max\endcsname{13}
\expandafter\def\csname pn@st.tiny.gazelle.epoch.min\endcsname{11}
\expandafter\def\csname pn@st.tiny.gazelle.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.gazelle.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.gazelle.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.gazelle.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.gazelle.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.gazelle.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.pooled\endcsname{0.204}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.pooled4\endcsname{0.2038}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.pck05\endcsname{0.056}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.pck10\endcsname{0.213}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.vat\endcsname{0.209}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.vat.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.childplay\endcsname{0.191}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.childplay.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.vacation\endcsname{0.217}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.vacation.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.social\endcsname{0.171}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.object\endcsname{0.232}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.collapse.min\endcsname{0.80}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.collapse.max\endcsname{0.82}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.collapse.mean\endcsname{0.81}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.epochs\endcsname{11, 11, 13}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.epoch.max\endcsname{13}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.epoch.min\endcsname{11}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.gazelle.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.gazelle.val.vslabels\endcsname{0.178}
\expandafter\def\csname pn@st.tiny.gazelle.val.vsgt\endcsname{0.199}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.pooled\endcsname{0.247}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.pooled4\endcsname{0.2468}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.pck05\endcsname{0.035}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.pck10\endcsname{0.131}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.vat\endcsname{0.245}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.childplay\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.childplay.sd\endcsname{0.016}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.vacation\endcsname{0.238}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.social\endcsname{0.209}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.social.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.object\endcsname{0.279}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.object.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.collapse.min\endcsname{0.68}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.collapse.max\endcsname{0.71}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.collapse.mean\endcsname{0.69}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.epochs\endcsname{4, 8, 3}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.epoch.max\endcsname{8}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.epoch.min\endcsname{3}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.pooled\endcsname{0.246}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.pooled4\endcsname{0.2458}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.pck05\endcsname{0.035}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.pck10\endcsname{0.128}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.vat\endcsname{0.242}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.vat.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.childplay\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.childplay.sd\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.vacation\endcsname{0.238}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.vacation.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.social\endcsname{0.205}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.social.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.object\endcsname{0.281}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.object.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.collapse.min\endcsname{0.68}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.collapse.max\endcsname{0.75}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.collapse.mean\endcsname{0.70}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.epochs\endcsname{4, 9, 7}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.epoch.max\endcsname{9}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.epoch.min\endcsname{4}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.val.vslabels\endcsname{0.220}
\expandafter\def\csname pn@st.tiny.teacher_hybrid.val.vsgt\endcsname{0.230}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.pooled\endcsname{0.291}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.pooled4\endcsname{0.2914}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.pck05\endcsname{0.049}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.pck10\endcsname{0.163}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.vat\endcsname{0.247}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.vat.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.childplay\endcsname{0.353}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.childplay.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.vacation\endcsname{0.262}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.vacation.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.social\endcsname{0.168}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.social.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.object\endcsname{0.397}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.object.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.collapse.min\endcsname{0.77}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.collapse.max\endcsname{0.80}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.collapse.mean\endcsname{0.79}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.epochs\endcsname{11, 8, 10}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.epoch.max\endcsname{11}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.epoch.min\endcsname{8}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.pooled\endcsname{0.291}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.pooled4\endcsname{0.2910}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.pck05\endcsname{0.046}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.pck10\endcsname{0.154}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.vat\endcsname{0.249}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.vat.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.childplay\endcsname{0.350}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.childplay.sd\endcsname{0.015}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.vacation\endcsname{0.261}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.vacation.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.social\endcsname{0.170}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.social.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.object\endcsname{0.395}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.object.sd\endcsname{0.012}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.collapse.min\endcsname{0.78}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.collapse.max\endcsname{0.85}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.collapse.mean\endcsname{0.81}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.epochs\endcsname{4, 11, 4}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.epoch.max\endcsname{11}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.epoch.min\endcsname{4}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.val.vslabels\endcsname{0.185}
\expandafter\def\csname pn@st.tiny.teacher_internvl3_alone.val.vsgt\endcsname{0.302}
\expandafter\def\csname pn@st.tiny.copyb.pooled\endcsname{0.294}
\expandafter\def\csname pn@st.tiny.copyb.pooled4\endcsname{0.2937}
\expandafter\def\csname pn@st.tiny.copyb.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.copyb.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.copyb.pck05\endcsname{0.065}
\expandafter\def\csname pn@st.tiny.copyb.pck10\endcsname{0.199}
\expandafter\def\csname pn@st.tiny.copyb.vat\endcsname{0.243}
\expandafter\def\csname pn@st.tiny.copyb.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.copyb.childplay\endcsname{0.358}
\expandafter\def\csname pn@st.tiny.copyb.childplay.sd\endcsname{0.014}
\expandafter\def\csname pn@st.tiny.copyb.vacation\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.copyb.vacation.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.copyb.social\endcsname{0.163}
\expandafter\def\csname pn@st.tiny.copyb.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.copyb.object\endcsname{0.406}
\expandafter\def\csname pn@st.tiny.copyb.object.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.copyb.collapse.min\endcsname{0.90}
\expandafter\def\csname pn@st.tiny.copyb.collapse.max\endcsname{0.91}
\expandafter\def\csname pn@st.tiny.copyb.collapse.mean\endcsname{0.91}
\expandafter\def\csname pn@st.tiny.copyb.epochs\endcsname{12, 14, 10}
\expandafter\def\csname pn@st.tiny.copyb.epoch.max\endcsname{14}
\expandafter\def\csname pn@st.tiny.copyb.epoch.min\endcsname{10}
\expandafter\def\csname pn@st.tiny.copyb.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.copyb.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.copyb.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.copyb.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.copyb.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.copyb.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.pooled\endcsname{0.291}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.pooled4\endcsname{0.2905}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.pck05\endcsname{0.065}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.pck10\endcsname{0.194}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.vat\endcsname{0.241}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.childplay\endcsname{0.351}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.childplay.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.vacation\endcsname{0.271}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.vacation.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.social\endcsname{0.161}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.social.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.object\endcsname{0.402}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.object.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.collapse.min\endcsname{0.86}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.collapse.max\endcsname{0.91}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.collapse.mean\endcsname{0.89}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.epochs\endcsname{8, 13, 15}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.epoch.max\endcsname{15}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.epoch.min\endcsname{8}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.copyb.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.copyb.val.vslabels\endcsname{0.174}
\expandafter\def\csname pn@st.tiny.copyb.val.vsgt\endcsname{0.303}
\expandafter\def\csname pn@st.tiny.vlmnoleak.pooled\endcsname{0.333}
\expandafter\def\csname pn@st.tiny.vlmnoleak.pooled4\endcsname{0.3328}
\expandafter\def\csname pn@st.tiny.vlmnoleak.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.vlmnoleak.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.vlmnoleak.pck05\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.vlmnoleak.pck10\endcsname{0.052}
\expandafter\def\csname pn@st.tiny.vlmnoleak.vat\endcsname{0.321}
\expandafter\def\csname pn@st.tiny.vlmnoleak.vat.sd\endcsname{0.014}
\expandafter\def\csname pn@st.tiny.vlmnoleak.childplay\endcsname{0.344}
\expandafter\def\csname pn@st.tiny.vlmnoleak.childplay.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.vlmnoleak.vacation\endcsname{0.333}
\expandafter\def\csname pn@st.tiny.vlmnoleak.vacation.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.vlmnoleak.social\endcsname{0.287}
\expandafter\def\csname pn@st.tiny.vlmnoleak.social.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.vlmnoleak.object\endcsname{0.372}
\expandafter\def\csname pn@st.tiny.vlmnoleak.object.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.vlmnoleak.collapse.min\endcsname{0.40}
\expandafter\def\csname pn@st.tiny.vlmnoleak.collapse.max\endcsname{0.69}
\expandafter\def\csname pn@st.tiny.vlmnoleak.collapse.mean\endcsname{0.59}
\expandafter\def\csname pn@st.tiny.vlmnoleak.epochs\endcsname{10, 10, 1}
\expandafter\def\csname pn@st.tiny.vlmnoleak.epoch.max\endcsname{10}
\expandafter\def\csname pn@st.tiny.vlmnoleak.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.vlmnoleak.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.vlmnoleak.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.vlmnoleak.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.vlmnoleak.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.vlmnoleak.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.vlmnoleak.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.pooled\endcsname{0.308}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.pooled4\endcsname{0.3076}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.sd\endcsname{0.016}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.pck05\endcsname{0.020}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.pck10\endcsname{0.070}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.vat\endcsname{0.291}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.vat.sd\endcsname{0.013}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.childplay\endcsname{0.328}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.childplay.sd\endcsname{0.018}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.vacation\endcsname{0.301}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.vacation.sd\endcsname{0.021}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.social\endcsname{0.250}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.social.sd\endcsname{0.024}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.object\endcsname{0.357}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.object.sd\endcsname{0.012}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.collapse.max\endcsname{0.40}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.collapse.mean\endcsname{0.22}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.epochs\endcsname{1, 1, 1}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.epoch.max\endcsname{1}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.vlmnoleak.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.vlmnoleak.val.vslabels\endcsname{0.172}
\expandafter\def\csname pn@st.tiny.vlmnoleak.val.vsgt\endcsname{0.325}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.pooled\endcsname{0.275}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.pooled4\endcsname{0.2748}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.pck05\endcsname{0.020}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.pck10\endcsname{0.076}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.vat\endcsname{0.286}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.childplay\endcsname{0.263}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.childplay.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.vacation\endcsname{0.276}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.vacation.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.social\endcsname{0.259}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.social.sd\endcsname{0.001}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.object\endcsname{0.289}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.object.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.collapse.min\endcsname{0.23}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.collapse.max\endcsname{0.37}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.collapse.mean\endcsname{0.28}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.epochs\endcsname{2, 2, 2}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.epoch.min\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.pooled\endcsname{0.271}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.pooled4\endcsname{0.2707}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.pck05\endcsname{0.019}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.pck10\endcsname{0.069}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.vat\endcsname{0.279}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.vat.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.childplay\endcsname{0.260}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.childplay.sd\endcsname{0.016}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.vacation\endcsname{0.275}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.vacation.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.social\endcsname{0.250}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.social.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.object\endcsname{0.288}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.object.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.collapse.max\endcsname{0.23}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.collapse.mean\endcsname{0.12}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.epochs\endcsname{2, 1, 1}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.val.vslabels\endcsname{0.209}
\expandafter\def\csname pn@st.tiny.ovdalwaysdino.val.vsgt\endcsname{0.255}
\expandafter\def\csname pn@st.tiny.ovdgate55.pooled\endcsname{0.267}
\expandafter\def\csname pn@st.tiny.ovdgate55.pooled4\endcsname{0.2673}
\expandafter\def\csname pn@st.tiny.ovdgate55.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdgate55.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate55.pck05\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.ovdgate55.pck10\endcsname{0.066}
\expandafter\def\csname pn@st.tiny.ovdgate55.vat\endcsname{0.283}
\expandafter\def\csname pn@st.tiny.ovdgate55.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate55.childplay\endcsname{0.248}
\expandafter\def\csname pn@st.tiny.ovdgate55.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.ovdgate55.vacation\endcsname{0.273}
\expandafter\def\csname pn@st.tiny.ovdgate55.vacation.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate55.social\endcsname{0.258}
\expandafter\def\csname pn@st.tiny.ovdgate55.social.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate55.object\endcsname{0.276}
\expandafter\def\csname pn@st.tiny.ovdgate55.object.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdgate55.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdgate55.collapse.max\endcsname{0.17}
\expandafter\def\csname pn@st.tiny.ovdgate55.collapse.mean\endcsname{0.10}
\expandafter\def\csname pn@st.tiny.ovdgate55.epochs\endcsname{1, 2, 1}
\expandafter\def\csname pn@st.tiny.ovdgate55.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate55.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdgate55.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate55.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate55.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate55.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate55.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate55.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.pooled\endcsname{0.267}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.pooled4\endcsname{0.2673}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.pck05\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.pck10\endcsname{0.066}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.vat\endcsname{0.283}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.childplay\endcsname{0.248}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.vacation\endcsname{0.273}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.vacation.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.social\endcsname{0.258}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.social.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.object\endcsname{0.276}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.object.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.collapse.max\endcsname{0.17}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.collapse.mean\endcsname{0.10}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.epochs\endcsname{1, 2, 1}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate55.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate55.val.vslabels\endcsname{0.214}
\expandafter\def\csname pn@st.tiny.ovdgate55.val.vsgt\endcsname{0.245}
\expandafter\def\csname pn@st.tiny.ovdmixrand.pooled\endcsname{0.261}
\expandafter\def\csname pn@st.tiny.ovdmixrand.pooled4\endcsname{0.2614}
\expandafter\def\csname pn@st.tiny.ovdmixrand.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmixrand.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdmixrand.pck05\endcsname{0.016}
\expandafter\def\csname pn@st.tiny.ovdmixrand.pck10\endcsname{0.069}
\expandafter\def\csname pn@st.tiny.ovdmixrand.vat\endcsname{0.276}
\expandafter\def\csname pn@st.tiny.ovdmixrand.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmixrand.childplay\endcsname{0.240}
\expandafter\def\csname pn@st.tiny.ovdmixrand.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.ovdmixrand.vacation\endcsname{0.274}
\expandafter\def\csname pn@st.tiny.ovdmixrand.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdmixrand.social\endcsname{0.252}
\expandafter\def\csname pn@st.tiny.ovdmixrand.social.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmixrand.object\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.ovdmixrand.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.ovdmixrand.collapse.min\endcsname{0.05}
\expandafter\def\csname pn@st.tiny.ovdmixrand.collapse.max\endcsname{0.10}
\expandafter\def\csname pn@st.tiny.ovdmixrand.collapse.mean\endcsname{0.07}
\expandafter\def\csname pn@st.tiny.ovdmixrand.epochs\endcsname{2, 2, 2}
\expandafter\def\csname pn@st.tiny.ovdmixrand.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmixrand.epoch.min\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmixrand.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdmixrand.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdmixrand.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdmixrand.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdmixrand.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdmixrand.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.pooled\endcsname{0.261}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.pooled4\endcsname{0.2614}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.pck05\endcsname{0.016}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.pck10\endcsname{0.069}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.vat\endcsname{0.276}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.childplay\endcsname{0.240}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.vacation\endcsname{0.274}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.social\endcsname{0.252}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.social.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.object\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.collapse.min\endcsname{0.05}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.collapse.max\endcsname{0.10}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.collapse.mean\endcsname{0.07}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.epochs\endcsname{2, 2, 2}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.epoch.min\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdmixrand.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdmixrand.val.vslabels\endcsname{0.214}
\expandafter\def\csname pn@st.tiny.ovdmixrand.val.vsgt\endcsname{0.244}
\expandafter\def\csname pn@st.tiny.centre.pooled\endcsname{0.294}
\expandafter\def\csname pn@st.tiny.centre.pooled4\endcsname{0.2939}
\expandafter\def\csname pn@st.tiny.centre.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.centre.pck05\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.centre.pck10\endcsname{0.061}
\expandafter\def\csname pn@st.tiny.centre.vat\endcsname{0.305}
\expandafter\def\csname pn@st.tiny.centre.vat.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.childplay\endcsname{0.288}
\expandafter\def\csname pn@st.tiny.centre.childplay.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.vacation\endcsname{0.284}
\expandafter\def\csname pn@st.tiny.centre.vacation.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.social\endcsname{0.284}
\expandafter\def\csname pn@st.tiny.centre.social.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.object\endcsname{0.302}
\expandafter\def\csname pn@st.tiny.centre.object.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.collapse.min\endcsname{0.00}
\expandafter\def\csname pn@st.tiny.centre.collapse.max\endcsname{0.00}
\expandafter\def\csname pn@st.tiny.centre.collapse.mean\endcsname{0.00}
\expandafter\def\csname pn@st.tiny.centre.epochs\endcsname{10, 5, 15}
\expandafter\def\csname pn@st.tiny.centre.epoch.max\endcsname{15}
\expandafter\def\csname pn@st.tiny.centre.epoch.min\endcsname{5}
\expandafter\def\csname pn@st.tiny.centre.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.centre.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.centre.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.centre.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.centre.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.centre.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.centre.gtsel.pooled\endcsname{0.294}
\expandafter\def\csname pn@st.tiny.centre.gtsel.pooled4\endcsname{0.2937}
\expandafter\def\csname pn@st.tiny.centre.gtsel.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.centre.gtsel.pck05\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.centre.gtsel.pck10\endcsname{0.060}
\expandafter\def\csname pn@st.tiny.centre.gtsel.vat\endcsname{0.305}
\expandafter\def\csname pn@st.tiny.centre.gtsel.vat.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.gtsel.childplay\endcsname{0.288}
\expandafter\def\csname pn@st.tiny.centre.gtsel.childplay.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.gtsel.vacation\endcsname{0.284}
\expandafter\def\csname pn@st.tiny.centre.gtsel.vacation.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.gtsel.social\endcsname{0.284}
\expandafter\def\csname pn@st.tiny.centre.gtsel.social.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.gtsel.object\endcsname{0.302}
\expandafter\def\csname pn@st.tiny.centre.gtsel.object.sd\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.gtsel.collapse.min\endcsname{0.00}
\expandafter\def\csname pn@st.tiny.centre.gtsel.collapse.max\endcsname{0.01}
\expandafter\def\csname pn@st.tiny.centre.gtsel.collapse.mean\endcsname{0.01}
\expandafter\def\csname pn@st.tiny.centre.gtsel.epochs\endcsname{1, 1, 4}
\expandafter\def\csname pn@st.tiny.centre.gtsel.epoch.max\endcsname{4}
\expandafter\def\csname pn@st.tiny.centre.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.centre.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.centre.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.centre.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.centre.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.centre.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.centre.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.centre.val.vslabels\endcsname{0.000}
\expandafter\def\csname pn@st.tiny.centre.val.vsgt\endcsname{0.264}
\expandafter\def\csname pn@st.tiny.ovdgate40.pooled\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.ovdgate40.pooled4\endcsname{0.2688}
\expandafter\def\csname pn@st.tiny.ovdgate40.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate40.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate40.pck05\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.ovdgate40.pck10\endcsname{0.067}
\expandafter\def\csname pn@st.tiny.ovdgate40.vat\endcsname{0.282}
\expandafter\def\csname pn@st.tiny.ovdgate40.vat.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdgate40.childplay\endcsname{0.255}
\expandafter\def\csname pn@st.tiny.ovdgate40.childplay.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.ovdgate40.vacation\endcsname{0.270}
\expandafter\def\csname pn@st.tiny.ovdgate40.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdgate40.social\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.ovdgate40.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate40.object\endcsname{0.282}
\expandafter\def\csname pn@st.tiny.ovdgate40.object.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.ovdgate40.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdgate40.collapse.max\endcsname{0.19}
\expandafter\def\csname pn@st.tiny.ovdgate40.collapse.mean\endcsname{0.11}
\expandafter\def\csname pn@st.tiny.ovdgate40.epochs\endcsname{1, 2, 1}
\expandafter\def\csname pn@st.tiny.ovdgate40.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate40.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdgate40.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate40.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate40.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate40.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate40.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate40.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.pooled\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.pooled4\endcsname{0.2688}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.pck05\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.pck10\endcsname{0.067}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.vat\endcsname{0.282}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.vat.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.childplay\endcsname{0.255}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.childplay.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.vacation\endcsname{0.270}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.social\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.object\endcsname{0.282}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.object.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.collapse.max\endcsname{0.19}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.collapse.mean\endcsname{0.11}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.epochs\endcsname{1, 2, 1}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate40.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate40.val.vslabels\endcsname{0.215}
\expandafter\def\csname pn@st.tiny.ovdgate40.val.vsgt\endcsname{0.252}
\expandafter\def\csname pn@st.tiny.ovdmix40.pooled\endcsname{0.265}
\expandafter\def\csname pn@st.tiny.ovdmix40.pooled4\endcsname{0.2649}
\expandafter\def\csname pn@st.tiny.ovdmix40.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdmix40.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdmix40.pck05\endcsname{0.018}
\expandafter\def\csname pn@st.tiny.ovdmix40.pck10\endcsname{0.072}
\expandafter\def\csname pn@st.tiny.ovdmix40.vat\endcsname{0.276}
\expandafter\def\csname pn@st.tiny.ovdmix40.vat.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdmix40.childplay\endcsname{0.249}
\expandafter\def\csname pn@st.tiny.ovdmix40.childplay.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.ovdmix40.vacation\endcsname{0.273}
\expandafter\def\csname pn@st.tiny.ovdmix40.vacation.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdmix40.social\endcsname{0.249}
\expandafter\def\csname pn@st.tiny.ovdmix40.social.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmix40.object\endcsname{0.279}
\expandafter\def\csname pn@st.tiny.ovdmix40.object.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.ovdmix40.collapse.min\endcsname{0.05}
\expandafter\def\csname pn@st.tiny.ovdmix40.collapse.max\endcsname{0.08}
\expandafter\def\csname pn@st.tiny.ovdmix40.collapse.mean\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdmix40.epochs\endcsname{1, 2, 1}
\expandafter\def\csname pn@st.tiny.ovdmix40.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmix40.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdmix40.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdmix40.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdmix40.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdmix40.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdmix40.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdmix40.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.pooled\endcsname{0.270}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.pooled4\endcsname{0.2698}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.pck05\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.pck10\endcsname{0.071}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.vat\endcsname{0.277}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.childplay\endcsname{0.258}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.childplay.sd\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.vacation\endcsname{0.278}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.vacation.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.social\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.object\endcsname{0.283}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.object.sd\endcsname{0.014}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.collapse.min\endcsname{0.08}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.collapse.max\endcsname{0.26}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.collapse.mean\endcsname{0.17}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.epochs\endcsname{2, 2, 2}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.epoch.min\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdmix40.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdmix40.val.vslabels\endcsname{0.211}
\expandafter\def\csname pn@st.tiny.ovdmix40.val.vsgt\endcsname{0.251}
\expandafter\def\csname pn@st.tiny.ovdgate48.pooled\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.ovdgate48.pooled4\endcsname{0.2692}
\expandafter\def\csname pn@st.tiny.ovdgate48.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate48.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate48.pck05\endcsname{0.015}
\expandafter\def\csname pn@st.tiny.ovdgate48.pck10\endcsname{0.067}
\expandafter\def\csname pn@st.tiny.ovdgate48.vat\endcsname{0.278}
\expandafter\def\csname pn@st.tiny.ovdgate48.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate48.childplay\endcsname{0.257}
\expandafter\def\csname pn@st.tiny.ovdgate48.childplay.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.ovdgate48.vacation\endcsname{0.275}
\expandafter\def\csname pn@st.tiny.ovdgate48.vacation.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate48.social\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.ovdgate48.social.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate48.object\endcsname{0.283}
\expandafter\def\csname pn@st.tiny.ovdgate48.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.ovdgate48.collapse.min\endcsname{0.05}
\expandafter\def\csname pn@st.tiny.ovdgate48.collapse.max\endcsname{0.23}
\expandafter\def\csname pn@st.tiny.ovdgate48.collapse.mean\endcsname{0.11}
\expandafter\def\csname pn@st.tiny.ovdgate48.epochs\endcsname{1, 2, 1}
\expandafter\def\csname pn@st.tiny.ovdgate48.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate48.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdgate48.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate48.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate48.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate48.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate48.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate48.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.pooled\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.pooled4\endcsname{0.2692}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.pck05\endcsname{0.015}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.pck10\endcsname{0.067}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.vat\endcsname{0.278}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.childplay\endcsname{0.257}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.childplay.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.vacation\endcsname{0.275}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.vacation.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.social\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.social.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.object\endcsname{0.283}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.collapse.min\endcsname{0.05}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.collapse.max\endcsname{0.23}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.collapse.mean\endcsname{0.11}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.epochs\endcsname{1, 2, 1}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate48.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate48.val.vslabels\endcsname{0.210}
\expandafter\def\csname pn@st.tiny.ovdgate48.val.vsgt\endcsname{0.246}
\expandafter\def\csname pn@st.tiny.ovdmix48.pooled\endcsname{0.270}
\expandafter\def\csname pn@st.tiny.ovdmix48.pooled4\endcsname{0.2702}
\expandafter\def\csname pn@st.tiny.ovdmix48.sd\endcsname{0.010}
\expandafter\def\csname pn@st.tiny.ovdmix48.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdmix48.pck05\endcsname{0.021}
\expandafter\def\csname pn@st.tiny.ovdmix48.pck10\endcsname{0.075}
\expandafter\def\csname pn@st.tiny.ovdmix48.vat\endcsname{0.288}
\expandafter\def\csname pn@st.tiny.ovdmix48.vat.sd\endcsname{0.017}
\expandafter\def\csname pn@st.tiny.ovdmix48.childplay\endcsname{0.244}
\expandafter\def\csname pn@st.tiny.ovdmix48.childplay.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdmix48.vacation\endcsname{0.285}
\expandafter\def\csname pn@st.tiny.ovdmix48.vacation.sd\endcsname{0.019}
\expandafter\def\csname pn@st.tiny.ovdmix48.social\endcsname{0.269}
\expandafter\def\csname pn@st.tiny.ovdmix48.social.sd\endcsname{0.024}
\expandafter\def\csname pn@st.tiny.ovdmix48.object\endcsname{0.272}
\expandafter\def\csname pn@st.tiny.ovdmix48.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdmix48.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdmix48.collapse.max\endcsname{0.51}
\expandafter\def\csname pn@st.tiny.ovdmix48.collapse.mean\endcsname{0.25}
\expandafter\def\csname pn@st.tiny.ovdmix48.epochs\endcsname{1, 8, 2}
\expandafter\def\csname pn@st.tiny.ovdmix48.epoch.max\endcsname{8}
\expandafter\def\csname pn@st.tiny.ovdmix48.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.tiny.ovdmix48.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdmix48.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdmix48.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdmix48.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdmix48.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdmix48.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.pooled\endcsname{0.263}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.pooled4\endcsname{0.2632}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.pck05\endcsname{0.021}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.pck10\endcsname{0.071}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.vat\endcsname{0.276}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.childplay\endcsname{0.245}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.childplay.sd\endcsname{0.004}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.vacation\endcsname{0.272}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.social\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.social.sd\endcsname{0.009}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.object\endcsname{0.272}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.collapse.min\endcsname{0.05}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.collapse.max\endcsname{0.17}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.collapse.mean\endcsname{0.09}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.epochs\endcsname{2, 2, 2}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.epoch.min\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdmix48.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdmix48.val.vslabels\endcsname{0.212}
\expandafter\def\csname pn@st.tiny.ovdmix48.val.vsgt\endcsname{0.249}
\expandafter\def\csname pn@st.tiny.ovdgate100.pooled\endcsname{0.261}
\expandafter\def\csname pn@st.tiny.ovdgate100.pooled4\endcsname{0.2611}
\expandafter\def\csname pn@st.tiny.ovdgate100.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.ovdgate100.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate100.pck05\endcsname{0.019}
\expandafter\def\csname pn@st.tiny.ovdgate100.pck10\endcsname{0.071}
\expandafter\def\csname pn@st.tiny.ovdgate100.vat\endcsname{0.283}
\expandafter\def\csname pn@st.tiny.ovdgate100.vat.sd\endcsname{0.016}
\expandafter\def\csname pn@st.tiny.ovdgate100.childplay\endcsname{0.229}
\expandafter\def\csname pn@st.tiny.ovdgate100.childplay.sd\endcsname{0.008}
\expandafter\def\csname pn@st.tiny.ovdgate100.vacation\endcsname{0.280}
\expandafter\def\csname pn@st.tiny.ovdgate100.vacation.sd\endcsname{0.011}
\expandafter\def\csname pn@st.tiny.ovdgate100.social\endcsname{0.265}
\expandafter\def\csname pn@st.tiny.ovdgate100.social.sd\endcsname{0.020}
\expandafter\def\csname pn@st.tiny.ovdgate100.object\endcsname{0.258}
\expandafter\def\csname pn@st.tiny.ovdgate100.object.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdgate100.collapse.min\endcsname{0.07}
\expandafter\def\csname pn@st.tiny.ovdgate100.collapse.max\endcsname{0.54}
\expandafter\def\csname pn@st.tiny.ovdgate100.collapse.mean\endcsname{0.23}
\expandafter\def\csname pn@st.tiny.ovdgate100.epochs\endcsname{5, 2, 2}
\expandafter\def\csname pn@st.tiny.ovdgate100.epoch.max\endcsname{5}
\expandafter\def\csname pn@st.tiny.ovdgate100.epoch.min\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate100.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate100.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate100.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate100.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate100.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate100.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.pooled\endcsname{0.254}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.pooled4\endcsname{0.2539}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.sd\endcsname{0.003}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.pck05\endcsname{0.018}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.pck10\endcsname{0.073}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.vat\endcsname{0.272}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.childplay\endcsname{0.224}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.vacation\endcsname{0.275}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.social\endcsname{0.252}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.social.sd\endcsname{0.005}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.object\endcsname{0.256}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.collapse.max\endcsname{0.09}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.collapse.mean\endcsname{0.07}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.epochs\endcsname{2, 2, 2}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.epoch.min\endcsname{2}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.tiny.ovdgate100.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.tiny.ovdgate100.val.vslabels\endcsname{0.210}
\expandafter\def\csname pn@st.tiny.ovdgate100.val.vsgt\endcsname{0.244}
\expandafter\def\csname pn@st.tiny.ovdfamily.collapse.min\endcsname{0.05}
\expandafter\def\csname pn@st.tiny.ovdfamily.collapse.max\endcsname{0.37}
\expandafter\def\csname pn@st.tiny.gaterand.epochs\endcsname{7}
\expandafter\def\csname pn@st.tiny.gaterand.randwins\endcsname{6}
\expandafter\def\csname pn@io.tiny.gt.f1half\endcsname{0.13}
\expandafter\def\csname pn@io.tiny.gt.f1val\endcsname{0.32}
\expandafter\def\csname pn@io.tiny.gt.f1valvat\endcsname{0.37}
\expandafter\def\csname pn@io.tiny.gt.f1oracle\endcsname{0.36}
\expandafter\def\csname pn@io.tiny.gt.auc\endcsname{0.73}
\expandafter\def\csname pn@io.tiny.gt.thrmax\endcsname{$2.0{\times}10^{-2}$}
\expandafter\def\csname pn@io.tiny.gt.thrmin\endcsname{$3.8{\times}10^{-5}$}
\expandafter\def\csname pn@io.test.pos\endcsname{6{,}687}
\expandafter\def\csname pn@io.test.n\endcsname{58{,}278}
\expandafter\def\csname pn@io.val.pos\endcsname{1{,}045}
\expandafter\def\csname pn@io.val.n\endcsname{43{,}215}
\expandafter\def\csname pn@io.val.prev\endcsname{2.4\%}
\expandafter\def\csname pn@io.test.prev\endcsname{11.5\%}
\expandafter\def\csname pn@io.tiny.mtgs.f1half\endcsname{0.18}
\expandafter\def\csname pn@io.tiny.mtgs.f1val\endcsname{0.35}
\expandafter\def\csname pn@io.tiny.mtgs.f1valvat\endcsname{0.39}
\expandafter\def\csname pn@io.tiny.mtgs.f1oracle\endcsname{0.36}
\expandafter\def\csname pn@io.tiny.mtgs.auc\endcsname{0.73}
\expandafter\def\csname pn@io.tiny.mtgs.thrmax\endcsname{$3.9{\times}10^{-5}$}
\expandafter\def\csname pn@io.tiny.mtgs.thrmin\endcsname{$2.6{\times}10^{-5}$}
\expandafter\def\csname pn@io.tiny.gazelle.f1half\endcsname{0.15}
\expandafter\def\csname pn@io.tiny.gazelle.f1val\endcsname{0.32}
\expandafter\def\csname pn@io.tiny.gazelle.f1valvat\endcsname{0.34}
\expandafter\def\csname pn@io.tiny.gazelle.f1oracle\endcsname{0.35}
\expandafter\def\csname pn@io.tiny.gazelle.auc\endcsname{0.71}
\expandafter\def\csname pn@io.tiny.gazelle.thrmax\endcsname{$4.3{\times}10^{-5}$}
\expandafter\def\csname pn@io.tiny.gazelle.thrmin\endcsname{$2.8{\times}10^{-5}$}
\expandafter\def\csname pn@io.tiny.teacher_hybrid.f1half\endcsname{0.11}
\expandafter\def\csname pn@io.tiny.teacher_hybrid.f1val\endcsname{0.26}
\expandafter\def\csname pn@io.tiny.teacher_hybrid.f1valvat\endcsname{0.28}
\expandafter\def\csname pn@io.tiny.teacher_hybrid.f1oracle\endcsname{0.30}
\expandafter\def\csname pn@io.tiny.teacher_hybrid.auc\endcsname{0.69}
\expandafter\def\csname pn@io.tiny.teacher_hybrid.thrmax\endcsname{$3.0{\times}10^{-3}$}
\expandafter\def\csname pn@io.tiny.teacher_hybrid.thrmin\endcsname{$2.1{\times}10^{-4}$}
\expandafter\def\csname pn@io.tiny.teacher_internvl3_alone.f1half\endcsname{0.12}
\expandafter\def\csname pn@io.tiny.teacher_internvl3_alone.f1val\endcsname{0.29}
\expandafter\def\csname pn@io.tiny.teacher_internvl3_alone.f1valvat\endcsname{0.31}
\expandafter\def\csname pn@io.tiny.teacher_internvl3_alone.f1oracle\endcsname{0.34}
\expandafter\def\csname pn@io.tiny.teacher_internvl3_alone.auc\endcsname{0.72}
\expandafter\def\csname pn@io.tiny.teacher_internvl3_alone.thrmax\endcsname{$2.5{\times}10^{-4}$}
\expandafter\def\csname pn@io.tiny.teacher_internvl3_alone.thrmin\endcsname{$7.3{\times}10^{-5}$}
\expandafter\def\csname pn@io.tiny.copyb.f1half\endcsname{0.10}
\expandafter\def\csname pn@io.tiny.copyb.f1val\endcsname{0.23}
\expandafter\def\csname pn@io.tiny.copyb.f1valvat\endcsname{0.25}
\expandafter\def\csname pn@io.tiny.copyb.f1oracle\endcsname{0.33}
\expandafter\def\csname pn@io.tiny.copyb.auc\endcsname{0.67}
\expandafter\def\csname pn@io.tiny.copyb.thrmax\endcsname{$8.4{\times}10^{-4}$}
\expandafter\def\csname pn@io.tiny.copyb.thrmin\endcsname{$5.2{\times}10^{-5}$}
\expandafter\def\csname pn@io.tiny.vlmnoleak.f1half\endcsname{0.10}
\expandafter\def\csname pn@io.tiny.vlmnoleak.f1val\endcsname{0.23}
\expandafter\def\csname pn@io.tiny.vlmnoleak.f1valvat\endcsname{0.25}
\expandafter\def\csname pn@io.tiny.vlmnoleak.f1oracle\endcsname{0.29}
\expandafter\def\csname pn@io.tiny.vlmnoleak.auc\endcsname{0.65}
\expandafter\def\csname pn@io.tiny.vlmnoleak.thrmax\endcsname{$3.5{\times}10^{-2}$}
\expandafter\def\csname pn@io.tiny.vlmnoleak.thrmin\endcsname{$5.0{\times}10^{-5}$}
\expandafter\def\csname pn@io.tiny.centre.f1half\endcsname{0.12}
\expandafter\def\csname pn@io.tiny.centre.f1val\endcsname{0.29}
\expandafter\def\csname pn@io.tiny.centre.f1valvat\endcsname{0.31}
\expandafter\def\csname pn@io.tiny.centre.f1oracle\endcsname{0.34}
\expandafter\def\csname pn@io.tiny.centre.auc\endcsname{0.73}
\expandafter\def\csname pn@io.tiny.centre.thrmax\endcsname{$1.3{\times}10^{-3}$}
\expandafter\def\csname pn@io.tiny.centre.thrmin\endcsname{$4.5{\times}10^{-6}$}
\expandafter\def\csname pn@io.tiny.ovdalwaysdino.f1half\endcsname{0.11}
\expandafter\def\csname pn@io.tiny.ovdalwaysdino.f1val\endcsname{0.27}
\expandafter\def\csname pn@io.tiny.ovdalwaysdino.f1valvat\endcsname{0.30}
\expandafter\def\csname pn@io.tiny.ovdalwaysdino.f1oracle\endcsname{0.31}
\expandafter\def\csname pn@io.tiny.ovdalwaysdino.auc\endcsname{0.69}
\expandafter\def\csname pn@io.tiny.ovdalwaysdino.thrmax\endcsname{$5.2{\times}10^{-2}$}
\expandafter\def\csname pn@io.tiny.ovdalwaysdino.thrmin\endcsname{$4.5{\times}10^{-4}$}
\expandafter\def\csname pn@io.tiny.ovdgate55.f1half\endcsname{0.11}
\expandafter\def\csname pn@io.tiny.ovdgate55.f1val\endcsname{0.28}
\expandafter\def\csname pn@io.tiny.ovdgate55.f1valvat\endcsname{0.31}
\expandafter\def\csname pn@io.tiny.ovdgate55.f1oracle\endcsname{0.32}
\expandafter\def\csname pn@io.tiny.ovdgate55.auc\endcsname{0.71}
\expandafter\def\csname pn@io.tiny.ovdgate55.thrmax\endcsname{$1.1{\times}10^{-2}$}
\expandafter\def\csname pn@io.tiny.ovdgate55.thrmin\endcsname{$1.2{\times}10^{-3}$}
\expandafter\def\csname pn@io.tiny.ovdmixrand.f1half\endcsname{0.07}
\expandafter\def\csname pn@io.tiny.ovdmixrand.f1val\endcsname{0.25}
\expandafter\def\csname pn@io.tiny.ovdmixrand.f1valvat\endcsname{0.31}
\expandafter\def\csname pn@io.tiny.ovdmixrand.f1oracle\endcsname{0.29}
\expandafter\def\csname pn@io.tiny.ovdmixrand.auc\endcsname{0.66}
\expandafter\def\csname pn@io.tiny.ovdmixrand.thrmax\endcsname{$2.7{\times}10^{-3}$}
\expandafter\def\csname pn@io.tiny.ovdmixrand.thrmin\endcsname{$6.5{\times}10^{-4}$}
\expandafter\def\csname pn@io.tiny.f1half.min\endcsname{0.07}
\expandafter\def\csname pn@io.tiny.f1half.max\endcsname{0.18}
\expandafter\def\csname pn@io.tiny.f1val.min\endcsname{0.23}
\expandafter\def\csname pn@io.tiny.f1val.max\endcsname{0.35}
\expandafter\def\csname pn@io.tiny.auc.min\endcsname{0.65}
\expandafter\def\csname pn@io.tiny.auc.max\endcsname{0.73}
\expandafter\def\csname pn@io.tiny.thr.max\endcsname{$5.2{\times}10^{-2}$}
\expandafter\def\csname pn@io.tiny.thr.min\endcsname{$4.5{\times}10^{-6}$}
\expandafter\def\csname pn@st.small.gt.pooled\endcsname{0.196}
\expandafter\def\csname pn@st.small.gt.pooled4\endcsname{0.1955}
\expandafter\def\csname pn@st.small.gt.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.gt.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.gt.pck05\endcsname{0.070}
\expandafter\def\csname pn@st.small.gt.pck10\endcsname{0.243}
\expandafter\def\csname pn@st.small.gt.vat\endcsname{0.208}
\expandafter\def\csname pn@st.small.gt.vat.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.gt.childplay\endcsname{0.180}
\expandafter\def\csname pn@st.small.gt.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.gt.vacation\endcsname{0.201}
\expandafter\def\csname pn@st.small.gt.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.gt.social\endcsname{0.165}
\expandafter\def\csname pn@st.small.gt.social.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.gt.object\endcsname{0.222}
\expandafter\def\csname pn@st.small.gt.object.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.gt.collapse.min\endcsname{0.81}
\expandafter\def\csname pn@st.small.gt.collapse.max\endcsname{0.88}
\expandafter\def\csname pn@st.small.gt.collapse.mean\endcsname{0.85}
\expandafter\def\csname pn@st.small.gt.epochs\endcsname{5, 7, 11}
\expandafter\def\csname pn@st.small.gt.epoch.max\endcsname{11}
\expandafter\def\csname pn@st.small.gt.epoch.min\endcsname{5}
\expandafter\def\csname pn@st.small.gt.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.gt.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.gt.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.gt.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.gt.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.gt.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.gt.gtsel.pooled\endcsname{0.196}
\expandafter\def\csname pn@st.small.gt.gtsel.pooled4\endcsname{0.1955}
\expandafter\def\csname pn@st.small.gt.gtsel.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.gt.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.gt.gtsel.pck05\endcsname{0.070}
\expandafter\def\csname pn@st.small.gt.gtsel.pck10\endcsname{0.243}
\expandafter\def\csname pn@st.small.gt.gtsel.vat\endcsname{0.208}
\expandafter\def\csname pn@st.small.gt.gtsel.vat.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.gt.gtsel.childplay\endcsname{0.180}
\expandafter\def\csname pn@st.small.gt.gtsel.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.gt.gtsel.vacation\endcsname{0.201}
\expandafter\def\csname pn@st.small.gt.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.gt.gtsel.social\endcsname{0.165}
\expandafter\def\csname pn@st.small.gt.gtsel.social.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.gt.gtsel.object\endcsname{0.222}
\expandafter\def\csname pn@st.small.gt.gtsel.object.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.gt.gtsel.collapse.min\endcsname{0.81}
\expandafter\def\csname pn@st.small.gt.gtsel.collapse.max\endcsname{0.88}
\expandafter\def\csname pn@st.small.gt.gtsel.collapse.mean\endcsname{0.85}
\expandafter\def\csname pn@st.small.gt.gtsel.epochs\endcsname{5, 7, 11}
\expandafter\def\csname pn@st.small.gt.gtsel.epoch.max\endcsname{11}
\expandafter\def\csname pn@st.small.gt.gtsel.epoch.min\endcsname{5}
\expandafter\def\csname pn@st.small.gt.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.gt.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.gt.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.gt.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.gt.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.gt.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.gt.val.vslabels\endcsname{0.189}
\expandafter\def\csname pn@st.small.gt.val.vsgt\endcsname{0.189}
\expandafter\def\csname pn@st.small.mtgs.pooled\endcsname{0.185}
\expandafter\def\csname pn@st.small.mtgs.pooled4\endcsname{0.1854}
\expandafter\def\csname pn@st.small.mtgs.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.mtgs.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.mtgs.pck05\endcsname{0.085}
\expandafter\def\csname pn@st.small.mtgs.pck10\endcsname{0.282}
\expandafter\def\csname pn@st.small.mtgs.vat\endcsname{0.192}
\expandafter\def\csname pn@st.small.mtgs.vat.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.mtgs.childplay\endcsname{0.174}
\expandafter\def\csname pn@st.small.mtgs.childplay.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.mtgs.vacation\endcsname{0.193}
\expandafter\def\csname pn@st.small.mtgs.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.mtgs.social\endcsname{0.148}
\expandafter\def\csname pn@st.small.mtgs.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.mtgs.object\endcsname{0.217}
\expandafter\def\csname pn@st.small.mtgs.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.mtgs.collapse.min\endcsname{0.88}
\expandafter\def\csname pn@st.small.mtgs.collapse.max\endcsname{0.88}
\expandafter\def\csname pn@st.small.mtgs.collapse.mean\endcsname{0.88}
\expandafter\def\csname pn@st.small.mtgs.epochs\endcsname{14, 14, 11}
\expandafter\def\csname pn@st.small.mtgs.epoch.max\endcsname{14}
\expandafter\def\csname pn@st.small.mtgs.epoch.min\endcsname{11}
\expandafter\def\csname pn@st.small.mtgs.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.mtgs.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.mtgs.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.mtgs.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.mtgs.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.mtgs.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.mtgs.gtsel.pooled\endcsname{0.185}
\expandafter\def\csname pn@st.small.mtgs.gtsel.pooled4\endcsname{0.1853}
\expandafter\def\csname pn@st.small.mtgs.gtsel.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.mtgs.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.mtgs.gtsel.pck05\endcsname{0.084}
\expandafter\def\csname pn@st.small.mtgs.gtsel.pck10\endcsname{0.281}
\expandafter\def\csname pn@st.small.mtgs.gtsel.vat\endcsname{0.192}
\expandafter\def\csname pn@st.small.mtgs.gtsel.vat.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.mtgs.gtsel.childplay\endcsname{0.173}
\expandafter\def\csname pn@st.small.mtgs.gtsel.childplay.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.mtgs.gtsel.vacation\endcsname{0.194}
\expandafter\def\csname pn@st.small.mtgs.gtsel.vacation.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.mtgs.gtsel.social\endcsname{0.150}
\expandafter\def\csname pn@st.small.mtgs.gtsel.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.mtgs.gtsel.object\endcsname{0.216}
\expandafter\def\csname pn@st.small.mtgs.gtsel.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.mtgs.gtsel.collapse.min\endcsname{0.87}
\expandafter\def\csname pn@st.small.mtgs.gtsel.collapse.max\endcsname{0.88}
\expandafter\def\csname pn@st.small.mtgs.gtsel.collapse.mean\endcsname{0.87}
\expandafter\def\csname pn@st.small.mtgs.gtsel.epochs\endcsname{15, 12, 11}
\expandafter\def\csname pn@st.small.mtgs.gtsel.epoch.max\endcsname{15}
\expandafter\def\csname pn@st.small.mtgs.gtsel.epoch.min\endcsname{11}
\expandafter\def\csname pn@st.small.mtgs.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.mtgs.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.mtgs.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.mtgs.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.mtgs.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.mtgs.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.mtgs.val.vslabels\endcsname{0.165}
\expandafter\def\csname pn@st.small.mtgs.val.vsgt\endcsname{0.180}
\expandafter\def\csname pn@st.small.gazelle.pooled\endcsname{0.187}
\expandafter\def\csname pn@st.small.gazelle.pooled4\endcsname{0.1872}
\expandafter\def\csname pn@st.small.gazelle.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.gazelle.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.gazelle.pck05\endcsname{0.080}
\expandafter\def\csname pn@st.small.gazelle.pck10\endcsname{0.276}
\expandafter\def\csname pn@st.small.gazelle.vat\endcsname{0.197}
\expandafter\def\csname pn@st.small.gazelle.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.gazelle.childplay\endcsname{0.175}
\expandafter\def\csname pn@st.small.gazelle.childplay.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.gazelle.vacation\endcsname{0.192}
\expandafter\def\csname pn@st.small.gazelle.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.gazelle.social\endcsname{0.160}
\expandafter\def\csname pn@st.small.gazelle.social.sd\endcsname{0.007}
\expandafter\def\csname pn@st.small.gazelle.object\endcsname{0.210}
\expandafter\def\csname pn@st.small.gazelle.object.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.gazelle.collapse.min\endcsname{0.77}
\expandafter\def\csname pn@st.small.gazelle.collapse.max\endcsname{0.83}
\expandafter\def\csname pn@st.small.gazelle.collapse.mean\endcsname{0.79}
\expandafter\def\csname pn@st.small.gazelle.epochs\endcsname{13, 8, 8}
\expandafter\def\csname pn@st.small.gazelle.epoch.max\endcsname{13}
\expandafter\def\csname pn@st.small.gazelle.epoch.min\endcsname{8}
\expandafter\def\csname pn@st.small.gazelle.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.gazelle.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.gazelle.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.gazelle.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.gazelle.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.gazelle.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.gazelle.gtsel.pooled\endcsname{0.188}
\expandafter\def\csname pn@st.small.gazelle.gtsel.pooled4\endcsname{0.1877}
\expandafter\def\csname pn@st.small.gazelle.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.gazelle.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.gazelle.gtsel.pck05\endcsname{0.078}
\expandafter\def\csname pn@st.small.gazelle.gtsel.pck10\endcsname{0.273}
\expandafter\def\csname pn@st.small.gazelle.gtsel.vat\endcsname{0.196}
\expandafter\def\csname pn@st.small.gazelle.gtsel.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.gazelle.gtsel.childplay\endcsname{0.177}
\expandafter\def\csname pn@st.small.gazelle.gtsel.childplay.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.gazelle.gtsel.vacation\endcsname{0.193}
\expandafter\def\csname pn@st.small.gazelle.gtsel.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.gazelle.gtsel.social\endcsname{0.156}
\expandafter\def\csname pn@st.small.gazelle.gtsel.social.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.gazelle.gtsel.object\endcsname{0.215}
\expandafter\def\csname pn@st.small.gazelle.gtsel.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.gazelle.gtsel.collapse.min\endcsname{0.79}
\expandafter\def\csname pn@st.small.gazelle.gtsel.collapse.max\endcsname{0.82}
\expandafter\def\csname pn@st.small.gazelle.gtsel.collapse.mean\endcsname{0.81}
\expandafter\def\csname pn@st.small.gazelle.gtsel.epochs\endcsname{11, 8, 11}
\expandafter\def\csname pn@st.small.gazelle.gtsel.epoch.max\endcsname{11}
\expandafter\def\csname pn@st.small.gazelle.gtsel.epoch.min\endcsname{8}
\expandafter\def\csname pn@st.small.gazelle.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.gazelle.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.gazelle.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.gazelle.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.gazelle.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.gazelle.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.gazelle.val.vslabels\endcsname{0.156}
\expandafter\def\csname pn@st.small.gazelle.val.vsgt\endcsname{0.179}
\expandafter\def\csname pn@st.small.teacher_hybrid.pooled\endcsname{0.238}
\expandafter\def\csname pn@st.small.teacher_hybrid.pooled4\endcsname{0.2381}
\expandafter\def\csname pn@st.small.teacher_hybrid.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.teacher_hybrid.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.teacher_hybrid.pck05\endcsname{0.045}
\expandafter\def\csname pn@st.small.teacher_hybrid.pck10\endcsname{0.155}
\expandafter\def\csname pn@st.small.teacher_hybrid.vat\endcsname{0.239}
\expandafter\def\csname pn@st.small.teacher_hybrid.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.teacher_hybrid.childplay\endcsname{0.240}
\expandafter\def\csname pn@st.small.teacher_hybrid.childplay.sd\endcsname{0.011}
\expandafter\def\csname pn@st.small.teacher_hybrid.vacation\endcsname{0.234}
\expandafter\def\csname pn@st.small.teacher_hybrid.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.teacher_hybrid.social\endcsname{0.195}
\expandafter\def\csname pn@st.small.teacher_hybrid.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.teacher_hybrid.object\endcsname{0.275}
\expandafter\def\csname pn@st.small.teacher_hybrid.object.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.teacher_hybrid.collapse.min\endcsname{0.73}
\expandafter\def\csname pn@st.small.teacher_hybrid.collapse.max\endcsname{0.81}
\expandafter\def\csname pn@st.small.teacher_hybrid.collapse.mean\endcsname{0.77}
\expandafter\def\csname pn@st.small.teacher_hybrid.epochs\endcsname{11, 8, 7}
\expandafter\def\csname pn@st.small.teacher_hybrid.epoch.max\endcsname{11}
\expandafter\def\csname pn@st.small.teacher_hybrid.epoch.min\endcsname{7}
\expandafter\def\csname pn@st.small.teacher_hybrid.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.teacher_hybrid.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.teacher_hybrid.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.teacher_hybrid.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.teacher_hybrid.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.teacher_hybrid.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.pooled\endcsname{0.240}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.pooled4\endcsname{0.2401}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.sd\endcsname{0.001}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.pck05\endcsname{0.039}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.pck10\endcsname{0.140}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.vat\endcsname{0.249}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.vat.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.childplay\endcsname{0.237}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.childplay.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.vacation\endcsname{0.231}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.social\endcsname{0.203}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.social.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.object\endcsname{0.272}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.object.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.collapse.min\endcsname{0.42}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.collapse.max\endcsname{0.77}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.collapse.mean\endcsname{0.62}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.epochs\endcsname{6, 9, 1}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.epoch.max\endcsname{9}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.teacher_hybrid.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.teacher_hybrid.val.vslabels\endcsname{0.219}
\expandafter\def\csname pn@st.small.teacher_hybrid.val.vsgt\endcsname{0.226}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.pooled\endcsname{0.289}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.pooled4\endcsname{0.2889}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.pck05\endcsname{0.073}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.pck10\endcsname{0.212}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.vat\endcsname{0.242}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.childplay\endcsname{0.346}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.childplay.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.vacation\endcsname{0.268}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.vacation.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.social\endcsname{0.155}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.social.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.object\endcsname{0.404}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.object.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.collapse.min\endcsname{0.81}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.collapse.max\endcsname{0.88}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.collapse.mean\endcsname{0.85}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.epochs\endcsname{9, 8, 7}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.epoch.max\endcsname{9}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.epoch.min\endcsname{7}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.pooled\endcsname{0.286}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.pooled4\endcsname{0.2863}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.pck05\endcsname{0.069}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.pck10\endcsname{0.204}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.vat\endcsname{0.244}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.childplay\endcsname{0.338}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.childplay.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.vacation\endcsname{0.269}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.vacation.sd\endcsname{0.011}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.social\endcsname{0.157}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.object\endcsname{0.397}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.object.sd\endcsname{0.007}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.collapse.min\endcsname{0.78}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.collapse.max\endcsname{0.89}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.collapse.mean\endcsname{0.84}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.epochs\endcsname{5, 12, 13}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.epoch.max\endcsname{13}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.epoch.min\endcsname{5}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.val.vslabels\endcsname{0.178}
\expandafter\def\csname pn@st.small.teacher_internvl3_alone.val.vsgt\endcsname{0.298}
\expandafter\def\csname pn@st.small.copyb.pooled\endcsname{0.287}
\expandafter\def\csname pn@st.small.copyb.pooled4\endcsname{0.2873}
\expandafter\def\csname pn@st.small.copyb.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.copyb.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.copyb.pck05\endcsname{0.103}
\expandafter\def\csname pn@st.small.copyb.pck10\endcsname{0.241}
\expandafter\def\csname pn@st.small.copyb.vat\endcsname{0.235}
\expandafter\def\csname pn@st.small.copyb.vat.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.copyb.childplay\endcsname{0.351}
\expandafter\def\csname pn@st.small.copyb.childplay.sd\endcsname{0.001}
\expandafter\def\csname pn@st.small.copyb.vacation\endcsname{0.265}
\expandafter\def\csname pn@st.small.copyb.vacation.sd\endcsname{0.001}
\expandafter\def\csname pn@st.small.copyb.social\endcsname{0.147}
\expandafter\def\csname pn@st.small.copyb.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.copyb.object\endcsname{0.408}
\expandafter\def\csname pn@st.small.copyb.object.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.copyb.collapse.min\endcsname{0.92}
\expandafter\def\csname pn@st.small.copyb.collapse.max\endcsname{0.94}
\expandafter\def\csname pn@st.small.copyb.collapse.mean\endcsname{0.93}
\expandafter\def\csname pn@st.small.copyb.epochs\endcsname{14, 12, 13}
\expandafter\def\csname pn@st.small.copyb.epoch.max\endcsname{14}
\expandafter\def\csname pn@st.small.copyb.epoch.min\endcsname{12}
\expandafter\def\csname pn@st.small.copyb.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.copyb.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.copyb.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.copyb.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.copyb.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.copyb.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.copyb.gtsel.pooled\endcsname{0.293}
\expandafter\def\csname pn@st.small.copyb.gtsel.pooled4\endcsname{0.2926}
\expandafter\def\csname pn@st.small.copyb.gtsel.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.copyb.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.copyb.gtsel.pck05\endcsname{0.064}
\expandafter\def\csname pn@st.small.copyb.gtsel.pck10\endcsname{0.187}
\expandafter\def\csname pn@st.small.copyb.gtsel.vat\endcsname{0.242}
\expandafter\def\csname pn@st.small.copyb.gtsel.vat.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.copyb.gtsel.childplay\endcsname{0.359}
\expandafter\def\csname pn@st.small.copyb.gtsel.childplay.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.copyb.gtsel.vacation\endcsname{0.265}
\expandafter\def\csname pn@st.small.copyb.gtsel.vacation.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.copyb.gtsel.social\endcsname{0.162}
\expandafter\def\csname pn@st.small.copyb.gtsel.social.sd\endcsname{0.013}
\expandafter\def\csname pn@st.small.copyb.gtsel.object\endcsname{0.405}
\expandafter\def\csname pn@st.small.copyb.gtsel.object.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.copyb.gtsel.collapse.min\endcsname{0.70}
\expandafter\def\csname pn@st.small.copyb.gtsel.collapse.max\endcsname{0.90}
\expandafter\def\csname pn@st.small.copyb.gtsel.collapse.mean\endcsname{0.83}
\expandafter\def\csname pn@st.small.copyb.gtsel.epochs\endcsname{8, 5, 1}
\expandafter\def\csname pn@st.small.copyb.gtsel.epoch.max\endcsname{8}
\expandafter\def\csname pn@st.small.copyb.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.copyb.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.copyb.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.copyb.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.copyb.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.copyb.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.copyb.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.copyb.val.vslabels\endcsname{0.154}
\expandafter\def\csname pn@st.small.copyb.val.vsgt\endcsname{0.301}
\expandafter\def\csname pn@st.small.vlmnoleak.pooled\endcsname{0.330}
\expandafter\def\csname pn@st.small.vlmnoleak.pooled4\endcsname{0.3303}
\expandafter\def\csname pn@st.small.vlmnoleak.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.vlmnoleak.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.vlmnoleak.pck05\endcsname{0.009}
\expandafter\def\csname pn@st.small.vlmnoleak.pck10\endcsname{0.042}
\expandafter\def\csname pn@st.small.vlmnoleak.vat\endcsname{0.330}
\expandafter\def\csname pn@st.small.vlmnoleak.vat.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.vlmnoleak.childplay\endcsname{0.326}
\expandafter\def\csname pn@st.small.vlmnoleak.childplay.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.vlmnoleak.vacation\endcsname{0.337}
\expandafter\def\csname pn@st.small.vlmnoleak.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.vlmnoleak.social\endcsname{0.291}
\expandafter\def\csname pn@st.small.vlmnoleak.social.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.vlmnoleak.object\endcsname{0.364}
\expandafter\def\csname pn@st.small.vlmnoleak.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.vlmnoleak.collapse.min\endcsname{0.61}
\expandafter\def\csname pn@st.small.vlmnoleak.collapse.max\endcsname{0.67}
\expandafter\def\csname pn@st.small.vlmnoleak.collapse.mean\endcsname{0.64}
\expandafter\def\csname pn@st.small.vlmnoleak.epochs\endcsname{9, 9, 3}
\expandafter\def\csname pn@st.small.vlmnoleak.epoch.max\endcsname{9}
\expandafter\def\csname pn@st.small.vlmnoleak.epoch.min\endcsname{3}
\expandafter\def\csname pn@st.small.vlmnoleak.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.vlmnoleak.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.vlmnoleak.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.vlmnoleak.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.vlmnoleak.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.vlmnoleak.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.pooled\endcsname{0.331}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.pooled4\endcsname{0.3307}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.sd\endcsname{0.001}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.pck05\endcsname{0.010}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.pck10\endcsname{0.043}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.vat\endcsname{0.333}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.childplay\endcsname{0.323}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.childplay.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.vacation\endcsname{0.341}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.social\endcsname{0.292}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.object\endcsname{0.364}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.object.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.collapse.min\endcsname{0.64}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.collapse.max\endcsname{0.67}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.collapse.mean\endcsname{0.65}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.epochs\endcsname{5, 13, 8}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.epoch.max\endcsname{13}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.epoch.min\endcsname{5}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.vlmnoleak.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.vlmnoleak.val.vslabels\endcsname{0.167}
\expandafter\def\csname pn@st.small.vlmnoleak.val.vsgt\endcsname{0.332}
\expandafter\def\csname pn@st.small.ovdalwaysdino.pooled\endcsname{0.274}
\expandafter\def\csname pn@st.small.ovdalwaysdino.pooled4\endcsname{0.2743}
\expandafter\def\csname pn@st.small.ovdalwaysdino.sd\endcsname{0.017}
\expandafter\def\csname pn@st.small.ovdalwaysdino.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdalwaysdino.pck05\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdalwaysdino.pck10\endcsname{0.073}
\expandafter\def\csname pn@st.small.ovdalwaysdino.vat\endcsname{0.291}
\expandafter\def\csname pn@st.small.ovdalwaysdino.vat.sd\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdalwaysdino.childplay\endcsname{0.255}
\expandafter\def\csname pn@st.small.ovdalwaysdino.childplay.sd\endcsname{0.011}
\expandafter\def\csname pn@st.small.ovdalwaysdino.vacation\endcsname{0.280}
\expandafter\def\csname pn@st.small.ovdalwaysdino.vacation.sd\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdalwaysdino.social\endcsname{0.265}
\expandafter\def\csname pn@st.small.ovdalwaysdino.social.sd\endcsname{0.029}
\expandafter\def\csname pn@st.small.ovdalwaysdino.object\endcsname{0.282}
\expandafter\def\csname pn@st.small.ovdalwaysdino.object.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.ovdalwaysdino.collapse.min\endcsname{0.08}
\expandafter\def\csname pn@st.small.ovdalwaysdino.collapse.max\endcsname{0.52}
\expandafter\def\csname pn@st.small.ovdalwaysdino.collapse.mean\endcsname{0.24}
\expandafter\def\csname pn@st.small.ovdalwaysdino.epochs\endcsname{1, 9, 1}
\expandafter\def\csname pn@st.small.ovdalwaysdino.epoch.max\endcsname{9}
\expandafter\def\csname pn@st.small.ovdalwaysdino.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdalwaysdino.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdalwaysdino.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdalwaysdino.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdalwaysdino.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdalwaysdino.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdalwaysdino.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.pooled\endcsname{0.265}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.pooled4\endcsname{0.2654}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.pck05\endcsname{0.020}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.pck10\endcsname{0.076}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.vat\endcsname{0.278}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.childplay\endcsname{0.250}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.childplay.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.vacation\endcsname{0.270}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.vacation.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.social\endcsname{0.249}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.social.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.object\endcsname{0.280}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.collapse.min\endcsname{0.08}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.collapse.max\endcsname{0.16}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.collapse.mean\endcsname{0.12}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.epochs\endcsname{1, 1, 1}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.epoch.max\endcsname{1}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdalwaysdino.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdalwaysdino.val.vslabels\endcsname{0.208}
\expandafter\def\csname pn@st.small.ovdalwaysdino.val.vsgt\endcsname{0.250}
\expandafter\def\csname pn@st.small.ovdgate55.pooled\endcsname{0.269}
\expandafter\def\csname pn@st.small.ovdgate55.pooled4\endcsname{0.2691}
\expandafter\def\csname pn@st.small.ovdgate55.sd\endcsname{0.013}
\expandafter\def\csname pn@st.small.ovdgate55.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate55.pck05\endcsname{0.020}
\expandafter\def\csname pn@st.small.ovdgate55.pck10\endcsname{0.075}
\expandafter\def\csname pn@st.small.ovdgate55.vat\endcsname{0.289}
\expandafter\def\csname pn@st.small.ovdgate55.vat.sd\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdgate55.childplay\endcsname{0.241}
\expandafter\def\csname pn@st.small.ovdgate55.childplay.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.ovdgate55.vacation\endcsname{0.285}
\expandafter\def\csname pn@st.small.ovdgate55.vacation.sd\endcsname{0.017}
\expandafter\def\csname pn@st.small.ovdgate55.social\endcsname{0.270}
\expandafter\def\csname pn@st.small.ovdgate55.social.sd\endcsname{0.032}
\expandafter\def\csname pn@st.small.ovdgate55.object\endcsname{0.268}
\expandafter\def\csname pn@st.small.ovdgate55.object.sd\endcsname{0.007}
\expandafter\def\csname pn@st.small.ovdgate55.collapse.min\endcsname{0.11}
\expandafter\def\csname pn@st.small.ovdgate55.collapse.max\endcsname{0.48}
\expandafter\def\csname pn@st.small.ovdgate55.collapse.mean\endcsname{0.35}
\expandafter\def\csname pn@st.small.ovdgate55.epochs\endcsname{2, 1, 2}
\expandafter\def\csname pn@st.small.ovdgate55.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.small.ovdgate55.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate55.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate55.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate55.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate55.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate55.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate55.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.pooled\endcsname{0.258}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.pooled4\endcsname{0.2575}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.pck05\endcsname{0.024}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.pck10\endcsname{0.078}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.vat\endcsname{0.267}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.vat.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.childplay\endcsname{0.242}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.childplay.sd\endcsname{0.015}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.vacation\endcsname{0.268}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.social\endcsname{0.239}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.social.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.object\endcsname{0.274}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.object.sd\endcsname{0.012}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.collapse.max\endcsname{0.11}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.collapse.mean\endcsname{0.09}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.epochs\endcsname{1, 1, 1}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.epoch.max\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate55.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate55.val.vslabels\endcsname{0.210}
\expandafter\def\csname pn@st.small.ovdgate55.val.vsgt\endcsname{0.248}
\expandafter\def\csname pn@st.small.ovdmixrand.pooled\endcsname{0.270}
\expandafter\def\csname pn@st.small.ovdmixrand.pooled4\endcsname{0.2700}
\expandafter\def\csname pn@st.small.ovdmixrand.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.ovdmixrand.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdmixrand.pck05\endcsname{0.020}
\expandafter\def\csname pn@st.small.ovdmixrand.pck10\endcsname{0.085}
\expandafter\def\csname pn@st.small.ovdmixrand.vat\endcsname{0.301}
\expandafter\def\csname pn@st.small.ovdmixrand.vat.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.ovdmixrand.childplay\endcsname{0.227}
\expandafter\def\csname pn@st.small.ovdmixrand.childplay.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.ovdmixrand.vacation\endcsname{0.292}
\expandafter\def\csname pn@st.small.ovdmixrand.vacation.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdmixrand.social\endcsname{0.287}
\expandafter\def\csname pn@st.small.ovdmixrand.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdmixrand.object\endcsname{0.255}
\expandafter\def\csname pn@st.small.ovdmixrand.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdmixrand.collapse.min\endcsname{0.50}
\expandafter\def\csname pn@st.small.ovdmixrand.collapse.max\endcsname{0.55}
\expandafter\def\csname pn@st.small.ovdmixrand.collapse.mean\endcsname{0.53}
\expandafter\def\csname pn@st.small.ovdmixrand.epochs\endcsname{10, 7, 4}
\expandafter\def\csname pn@st.small.ovdmixrand.epoch.max\endcsname{10}
\expandafter\def\csname pn@st.small.ovdmixrand.epoch.min\endcsname{4}
\expandafter\def\csname pn@st.small.ovdmixrand.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdmixrand.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdmixrand.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdmixrand.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdmixrand.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdmixrand.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.pooled\endcsname{0.252}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.pooled4\endcsname{0.2524}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.pck05\endcsname{0.022}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.pck10\endcsname{0.086}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.vat\endcsname{0.273}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.vat.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.childplay\endcsname{0.223}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.vacation\endcsname{0.267}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.social\endcsname{0.248}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.social.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.object\endcsname{0.256}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.object.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.collapse.max\endcsname{0.21}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.collapse.mean\endcsname{0.11}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.epochs\endcsname{1, 1, 2}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdmixrand.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdmixrand.val.vslabels\endcsname{0.205}
\expandafter\def\csname pn@st.small.ovdmixrand.val.vsgt\endcsname{0.250}
\expandafter\def\csname pn@st.small.centre.pooled\endcsname{0.294}
\expandafter\def\csname pn@st.small.centre.pooled4\endcsname{0.2939}
\expandafter\def\csname pn@st.small.centre.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.centre.pck05\endcsname{0.008}
\expandafter\def\csname pn@st.small.centre.pck10\endcsname{0.061}
\expandafter\def\csname pn@st.small.centre.vat\endcsname{0.305}
\expandafter\def\csname pn@st.small.centre.vat.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.childplay\endcsname{0.288}
\expandafter\def\csname pn@st.small.centre.childplay.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.vacation\endcsname{0.284}
\expandafter\def\csname pn@st.small.centre.vacation.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.social\endcsname{0.284}
\expandafter\def\csname pn@st.small.centre.social.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.object\endcsname{0.302}
\expandafter\def\csname pn@st.small.centre.object.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.collapse.min\endcsname{0.00}
\expandafter\def\csname pn@st.small.centre.collapse.max\endcsname{0.00}
\expandafter\def\csname pn@st.small.centre.collapse.mean\endcsname{0.00}
\expandafter\def\csname pn@st.small.centre.epochs\endcsname{14, 8, 15}
\expandafter\def\csname pn@st.small.centre.epoch.max\endcsname{15}
\expandafter\def\csname pn@st.small.centre.epoch.min\endcsname{8}
\expandafter\def\csname pn@st.small.centre.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.centre.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.centre.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.centre.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.centre.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.centre.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.centre.gtsel.pooled\endcsname{0.294}
\expandafter\def\csname pn@st.small.centre.gtsel.pooled4\endcsname{0.2939}
\expandafter\def\csname pn@st.small.centre.gtsel.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.centre.gtsel.pck05\endcsname{0.008}
\expandafter\def\csname pn@st.small.centre.gtsel.pck10\endcsname{0.061}
\expandafter\def\csname pn@st.small.centre.gtsel.vat\endcsname{0.305}
\expandafter\def\csname pn@st.small.centre.gtsel.vat.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.gtsel.childplay\endcsname{0.288}
\expandafter\def\csname pn@st.small.centre.gtsel.childplay.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.gtsel.vacation\endcsname{0.284}
\expandafter\def\csname pn@st.small.centre.gtsel.vacation.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.gtsel.social\endcsname{0.284}
\expandafter\def\csname pn@st.small.centre.gtsel.social.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.gtsel.object\endcsname{0.303}
\expandafter\def\csname pn@st.small.centre.gtsel.object.sd\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.gtsel.collapse.min\endcsname{0.00}
\expandafter\def\csname pn@st.small.centre.gtsel.collapse.max\endcsname{0.01}
\expandafter\def\csname pn@st.small.centre.gtsel.collapse.mean\endcsname{0.01}
\expandafter\def\csname pn@st.small.centre.gtsel.epochs\endcsname{1, 3, 1}
\expandafter\def\csname pn@st.small.centre.gtsel.epoch.max\endcsname{3}
\expandafter\def\csname pn@st.small.centre.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.centre.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.centre.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.centre.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.centre.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.centre.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.centre.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.centre.val.vslabels\endcsname{0.000}
\expandafter\def\csname pn@st.small.centre.val.vsgt\endcsname{0.264}
\expandafter\def\csname pn@st.small.ovdgate40.pooled\endcsname{0.278}
\expandafter\def\csname pn@st.small.ovdgate40.pooled4\endcsname{0.2778}
\expandafter\def\csname pn@st.small.ovdgate40.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.ovdgate40.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate40.pck05\endcsname{0.023}
\expandafter\def\csname pn@st.small.ovdgate40.pck10\endcsname{0.083}
\expandafter\def\csname pn@st.small.ovdgate40.vat\endcsname{0.302}
\expandafter\def\csname pn@st.small.ovdgate40.vat.sd\endcsname{0.022}
\expandafter\def\csname pn@st.small.ovdgate40.childplay\endcsname{0.245}
\expandafter\def\csname pn@st.small.ovdgate40.childplay.sd\endcsname{0.011}
\expandafter\def\csname pn@st.small.ovdgate40.vacation\endcsname{0.295}
\expandafter\def\csname pn@st.small.ovdgate40.vacation.sd\endcsname{0.023}
\expandafter\def\csname pn@st.small.ovdgate40.social\endcsname{0.278}
\expandafter\def\csname pn@st.small.ovdgate40.social.sd\endcsname{0.026}
\expandafter\def\csname pn@st.small.ovdgate40.object\endcsname{0.277}
\expandafter\def\csname pn@st.small.ovdgate40.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdgate40.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.small.ovdgate40.collapse.max\endcsname{0.58}
\expandafter\def\csname pn@st.small.ovdgate40.collapse.mean\endcsname{0.40}
\expandafter\def\csname pn@st.small.ovdgate40.epochs\endcsname{4, 8, 1}
\expandafter\def\csname pn@st.small.ovdgate40.epoch.max\endcsname{8}
\expandafter\def\csname pn@st.small.ovdgate40.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate40.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate40.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate40.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate40.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate40.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate40.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.pooled\endcsname{0.267}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.pooled4\endcsname{0.2665}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.sd\endcsname{0.001}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.pck05\endcsname{0.019}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.pck10\endcsname{0.074}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.vat\endcsname{0.276}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.childplay\endcsname{0.254}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.childplay.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.vacation\endcsname{0.272}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.social\endcsname{0.249}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.social.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.object\endcsname{0.281}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.object.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.collapse.max\endcsname{0.15}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.collapse.mean\endcsname{0.10}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.epochs\endcsname{1, 1, 1}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.epoch.max\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate40.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate40.val.vslabels\endcsname{0.209}
\expandafter\def\csname pn@st.small.ovdgate40.val.vsgt\endcsname{0.259}
\expandafter\def\csname pn@st.small.ovdmix40.pooled\endcsname{0.272}
\expandafter\def\csname pn@st.small.ovdmix40.pooled4\endcsname{0.2717}
\expandafter\def\csname pn@st.small.ovdmix40.sd\endcsname{0.013}
\expandafter\def\csname pn@st.small.ovdmix40.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdmix40.pck05\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdmix40.pck10\endcsname{0.079}
\expandafter\def\csname pn@st.small.ovdmix40.vat\endcsname{0.294}
\expandafter\def\csname pn@st.small.ovdmix40.vat.sd\endcsname{0.019}
\expandafter\def\csname pn@st.small.ovdmix40.childplay\endcsname{0.241}
\expandafter\def\csname pn@st.small.ovdmix40.childplay.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.ovdmix40.vacation\endcsname{0.287}
\expandafter\def\csname pn@st.small.ovdmix40.vacation.sd\endcsname{0.018}
\expandafter\def\csname pn@st.small.ovdmix40.social\endcsname{0.273}
\expandafter\def\csname pn@st.small.ovdmix40.social.sd\endcsname{0.023}
\expandafter\def\csname pn@st.small.ovdmix40.object\endcsname{0.270}
\expandafter\def\csname pn@st.small.ovdmix40.object.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdmix40.collapse.min\endcsname{0.11}
\expandafter\def\csname pn@st.small.ovdmix40.collapse.max\endcsname{0.55}
\expandafter\def\csname pn@st.small.ovdmix40.collapse.mean\endcsname{0.39}
\expandafter\def\csname pn@st.small.ovdmix40.epochs\endcsname{1, 9, 6}
\expandafter\def\csname pn@st.small.ovdmix40.epoch.max\endcsname{9}
\expandafter\def\csname pn@st.small.ovdmix40.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdmix40.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdmix40.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdmix40.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdmix40.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdmix40.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdmix40.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.pooled\endcsname{0.259}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.pooled4\endcsname{0.2586}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.sd\endcsname{0.003}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.pck05\endcsname{0.020}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.pck10\endcsname{0.077}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.vat\endcsname{0.268}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.childplay\endcsname{0.246}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.childplay.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.vacation\endcsname{0.265}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.social\endcsname{0.239}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.social.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.object\endcsname{0.275}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.object.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.collapse.min\endcsname{0.08}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.collapse.max\endcsname{0.11}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.collapse.mean\endcsname{0.09}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.epochs\endcsname{1, 1, 1}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.epoch.max\endcsname{1}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdmix40.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdmix40.val.vslabels\endcsname{0.210}
\expandafter\def\csname pn@st.small.ovdmix40.val.vsgt\endcsname{0.255}
\expandafter\def\csname pn@st.small.ovdgate48.pooled\endcsname{0.276}
\expandafter\def\csname pn@st.small.ovdgate48.pooled4\endcsname{0.2756}
\expandafter\def\csname pn@st.small.ovdgate48.sd\endcsname{0.015}
\expandafter\def\csname pn@st.small.ovdgate48.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate48.pck05\endcsname{0.022}
\expandafter\def\csname pn@st.small.ovdgate48.pck10\endcsname{0.076}
\expandafter\def\csname pn@st.small.ovdgate48.vat\endcsname{0.301}
\expandafter\def\csname pn@st.small.ovdgate48.vat.sd\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdgate48.childplay\endcsname{0.242}
\expandafter\def\csname pn@st.small.ovdgate48.childplay.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.ovdgate48.vacation\endcsname{0.292}
\expandafter\def\csname pn@st.small.ovdgate48.vacation.sd\endcsname{0.025}
\expandafter\def\csname pn@st.small.ovdgate48.social\endcsname{0.281}
\expandafter\def\csname pn@st.small.ovdgate48.social.sd\endcsname{0.027}
\expandafter\def\csname pn@st.small.ovdgate48.object\endcsname{0.271}
\expandafter\def\csname pn@st.small.ovdgate48.object.sd\endcsname{0.007}
\expandafter\def\csname pn@st.small.ovdgate48.collapse.min\endcsname{0.11}
\expandafter\def\csname pn@st.small.ovdgate48.collapse.max\endcsname{0.59}
\expandafter\def\csname pn@st.small.ovdgate48.collapse.mean\endcsname{0.43}
\expandafter\def\csname pn@st.small.ovdgate48.epochs\endcsname{1, 8, 11}
\expandafter\def\csname pn@st.small.ovdgate48.epoch.max\endcsname{11}
\expandafter\def\csname pn@st.small.ovdgate48.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate48.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate48.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate48.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate48.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate48.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate48.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.pooled\endcsname{0.262}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.pooled4\endcsname{0.2620}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.pck05\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.pck10\endcsname{0.077}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.vat\endcsname{0.278}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.vat.sd\endcsname{0.015}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.childplay\endcsname{0.240}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.childplay.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.vacation\endcsname{0.272}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.vacation.sd\endcsname{0.012}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.social\endcsname{0.255}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.social.sd\endcsname{0.019}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.object\endcsname{0.268}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.object.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.collapse.min\endcsname{0.11}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.collapse.max\endcsname{0.38}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.collapse.mean\endcsname{0.20}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.epochs\endcsname{1, 1, 2}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate48.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate48.val.vslabels\endcsname{0.209}
\expandafter\def\csname pn@st.small.ovdgate48.val.vsgt\endcsname{0.258}
\expandafter\def\csname pn@st.small.ovdmix48.pooled\endcsname{0.275}
\expandafter\def\csname pn@st.small.ovdmix48.pooled4\endcsname{0.2749}
\expandafter\def\csname pn@st.small.ovdmix48.sd\endcsname{0.011}
\expandafter\def\csname pn@st.small.ovdmix48.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdmix48.pck05\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdmix48.pck10\endcsname{0.085}
\expandafter\def\csname pn@st.small.ovdmix48.vat\endcsname{0.301}
\expandafter\def\csname pn@st.small.ovdmix48.vat.sd\endcsname{0.011}
\expandafter\def\csname pn@st.small.ovdmix48.childplay\endcsname{0.234}
\expandafter\def\csname pn@st.small.ovdmix48.childplay.sd\endcsname{0.019}
\expandafter\def\csname pn@st.small.ovdmix48.vacation\endcsname{0.302}
\expandafter\def\csname pn@st.small.ovdmix48.vacation.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.ovdmix48.social\endcsname{0.289}
\expandafter\def\csname pn@st.small.ovdmix48.social.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.ovdmix48.object\endcsname{0.263}
\expandafter\def\csname pn@st.small.ovdmix48.object.sd\endcsname{0.016}
\expandafter\def\csname pn@st.small.ovdmix48.collapse.min\endcsname{0.51}
\expandafter\def\csname pn@st.small.ovdmix48.collapse.max\endcsname{0.53}
\expandafter\def\csname pn@st.small.ovdmix48.collapse.mean\endcsname{0.52}
\expandafter\def\csname pn@st.small.ovdmix48.epochs\endcsname{5, 7, 9}
\expandafter\def\csname pn@st.small.ovdmix48.epoch.max\endcsname{9}
\expandafter\def\csname pn@st.small.ovdmix48.epoch.min\endcsname{5}
\expandafter\def\csname pn@st.small.ovdmix48.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdmix48.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdmix48.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdmix48.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdmix48.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdmix48.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.pooled\endcsname{0.257}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.pooled4\endcsname{0.2568}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.sd\endcsname{0.002}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.pck05\endcsname{0.021}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.pck10\endcsname{0.079}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.vat\endcsname{0.270}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.childplay\endcsname{0.239}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.childplay.sd\endcsname{0.001}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.vacation\endcsname{0.266}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.social\endcsname{0.243}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.social.sd\endcsname{0.008}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.object\endcsname{0.269}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.object.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.collapse.min\endcsname{0.06}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.collapse.max\endcsname{0.08}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.collapse.mean\endcsname{0.07}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.epochs\endcsname{1, 1, 1}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.epoch.max\endcsname{1}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdmix48.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdmix48.val.vslabels\endcsname{0.208}
\expandafter\def\csname pn@st.small.ovdmix48.val.vsgt\endcsname{0.257}
\expandafter\def\csname pn@st.small.ovdgate100.pooled\endcsname{0.260}
\expandafter\def\csname pn@st.small.ovdgate100.pooled4\endcsname{0.2604}
\expandafter\def\csname pn@st.small.ovdgate100.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdgate100.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate100.pck05\endcsname{0.032}
\expandafter\def\csname pn@st.small.ovdgate100.pck10\endcsname{0.128}
\expandafter\def\csname pn@st.small.ovdgate100.vat\endcsname{0.296}
\expandafter\def\csname pn@st.small.ovdgate100.vat.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.ovdgate100.childplay\endcsname{0.207}
\expandafter\def\csname pn@st.small.ovdgate100.childplay.sd\endcsname{0.005}
\expandafter\def\csname pn@st.small.ovdgate100.vacation\endcsname{0.292}
\expandafter\def\csname pn@st.small.ovdgate100.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@st.small.ovdgate100.social\endcsname{0.286}
\expandafter\def\csname pn@st.small.ovdgate100.social.sd\endcsname{0.007}
\expandafter\def\csname pn@st.small.ovdgate100.object\endcsname{0.238}
\expandafter\def\csname pn@st.small.ovdgate100.object.sd\endcsname{0.006}
\expandafter\def\csname pn@st.small.ovdgate100.collapse.min\endcsname{0.57}
\expandafter\def\csname pn@st.small.ovdgate100.collapse.max\endcsname{0.63}
\expandafter\def\csname pn@st.small.ovdgate100.collapse.mean\endcsname{0.59}
\expandafter\def\csname pn@st.small.ovdgate100.epochs\endcsname{9, 10, 7}
\expandafter\def\csname pn@st.small.ovdgate100.epoch.max\endcsname{10}
\expandafter\def\csname pn@st.small.ovdgate100.epoch.min\endcsname{7}
\expandafter\def\csname pn@st.small.ovdgate100.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate100.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate100.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate100.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate100.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate100.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.pooled\endcsname{0.254}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.pooled4\endcsname{0.2536}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.sd\endcsname{0.010}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.pck05\endcsname{0.019}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.pck10\endcsname{0.085}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.vat\endcsname{0.273}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.vat.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.childplay\endcsname{0.222}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.childplay.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.vacation\endcsname{0.276}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.vacation.sd\endcsname{0.014}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.social\endcsname{0.261}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.social.sd\endcsname{0.012}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.object\endcsname{0.248}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.object.sd\endcsname{0.009}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.collapse.min\endcsname{0.07}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.collapse.max\endcsname{0.44}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.collapse.mean\endcsname{0.30}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.epochs\endcsname{1, 2, 2}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.epoch.max\endcsname{2}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@st.small.ovdgate100.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@st.small.ovdgate100.val.vslabels\endcsname{0.199}
\expandafter\def\csname pn@st.small.ovdgate100.val.vsgt\endcsname{0.248}
\expandafter\def\csname pn@st.small.ovdfamily.collapse.min\endcsname{0.08}
\expandafter\def\csname pn@st.small.ovdfamily.collapse.max\endcsname{0.55}
\expandafter\def\csname pn@io.small.gt.f1half\endcsname{0.23}
\expandafter\def\csname pn@io.small.gt.f1val\endcsname{0.39}
\expandafter\def\csname pn@io.small.gt.f1valvat\endcsname{0.43}
\expandafter\def\csname pn@io.small.gt.f1oracle\endcsname{0.42}
\expandafter\def\csname pn@io.small.gt.auc\endcsname{0.78}
\expandafter\def\csname pn@io.small.gt.thrmax\endcsname{$5.2{\times}10^{-3}$}
\expandafter\def\csname pn@io.small.gt.thrmin\endcsname{$4.4{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.mtgs.f1half\endcsname{0.21}
\expandafter\def\csname pn@io.small.mtgs.f1val\endcsname{0.39}
\expandafter\def\csname pn@io.small.mtgs.f1valvat\endcsname{0.40}
\expandafter\def\csname pn@io.small.mtgs.f1oracle\endcsname{0.44}
\expandafter\def\csname pn@io.small.mtgs.auc\endcsname{0.78}
\expandafter\def\csname pn@io.small.mtgs.thrmax\endcsname{$2.4{\times}10^{-4}$}
\expandafter\def\csname pn@io.small.mtgs.thrmin\endcsname{$5.1{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.gazelle.f1half\endcsname{0.16}
\expandafter\def\csname pn@io.small.gazelle.f1val\endcsname{0.37}
\expandafter\def\csname pn@io.small.gazelle.f1valvat\endcsname{0.39}
\expandafter\def\csname pn@io.small.gazelle.f1oracle\endcsname{0.38}
\expandafter\def\csname pn@io.small.gazelle.auc\endcsname{0.76}
\expandafter\def\csname pn@io.small.gazelle.thrmax\endcsname{$2.0{\times}10^{-4}$}
\expandafter\def\csname pn@io.small.gazelle.thrmin\endcsname{$3.2{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.teacher_hybrid.f1half\endcsname{0.17}
\expandafter\def\csname pn@io.small.teacher_hybrid.f1val\endcsname{0.32}
\expandafter\def\csname pn@io.small.teacher_hybrid.f1valvat\endcsname{0.33}
\expandafter\def\csname pn@io.small.teacher_hybrid.f1oracle\endcsname{0.38}
\expandafter\def\csname pn@io.small.teacher_hybrid.auc\endcsname{0.75}
\expandafter\def\csname pn@io.small.teacher_hybrid.thrmax\endcsname{$1.2{\times}10^{-3}$}
\expandafter\def\csname pn@io.small.teacher_hybrid.thrmin\endcsname{$1.8{\times}10^{-4}$}
\expandafter\def\csname pn@io.small.teacher_internvl3_alone.f1half\endcsname{0.19}
\expandafter\def\csname pn@io.small.teacher_internvl3_alone.f1val\endcsname{0.35}
\expandafter\def\csname pn@io.small.teacher_internvl3_alone.f1valvat\endcsname{0.38}
\expandafter\def\csname pn@io.small.teacher_internvl3_alone.f1oracle\endcsname{0.38}
\expandafter\def\csname pn@io.small.teacher_internvl3_alone.auc\endcsname{0.76}
\expandafter\def\csname pn@io.small.teacher_internvl3_alone.thrmax\endcsname{$8.6{\times}10^{-4}$}
\expandafter\def\csname pn@io.small.teacher_internvl3_alone.thrmin\endcsname{$2.4{\times}10^{-4}$}
\expandafter\def\csname pn@io.small.copyb.f1half\endcsname{0.13}
\expandafter\def\csname pn@io.small.copyb.f1val\endcsname{0.32}
\expandafter\def\csname pn@io.small.copyb.f1valvat\endcsname{0.34}
\expandafter\def\csname pn@io.small.copyb.f1oracle\endcsname{0.34}
\expandafter\def\csname pn@io.small.copyb.auc\endcsname{0.67}
\expandafter\def\csname pn@io.small.copyb.thrmax\endcsname{$3.0{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.copyb.thrmin\endcsname{$2.8{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.vlmnoleak.f1half\endcsname{0.14}
\expandafter\def\csname pn@io.small.vlmnoleak.f1val\endcsname{0.33}
\expandafter\def\csname pn@io.small.vlmnoleak.f1valvat\endcsname{0.36}
\expandafter\def\csname pn@io.small.vlmnoleak.f1oracle\endcsname{0.36}
\expandafter\def\csname pn@io.small.vlmnoleak.auc\endcsname{0.74}
\expandafter\def\csname pn@io.small.vlmnoleak.thrmax\endcsname{$6.5{\times}10^{-4}$}
\expandafter\def\csname pn@io.small.vlmnoleak.thrmin\endcsname{$4.9{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.centre.f1half\endcsname{0.08}
\expandafter\def\csname pn@io.small.centre.f1val\endcsname{0.28}
\expandafter\def\csname pn@io.small.centre.f1valvat\endcsname{0.31}
\expandafter\def\csname pn@io.small.centre.f1oracle\endcsname{0.36}
\expandafter\def\csname pn@io.small.centre.auc\endcsname{0.74}
\expandafter\def\csname pn@io.small.centre.thrmax\endcsname{$5.4{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.centre.thrmin\endcsname{$7.9{\times}10^{-6}$}
\expandafter\def\csname pn@io.small.ovdalwaysdino.f1half\endcsname{0.15}
\expandafter\def\csname pn@io.small.ovdalwaysdino.f1val\endcsname{0.32}
\expandafter\def\csname pn@io.small.ovdalwaysdino.f1valvat\endcsname{0.34}
\expandafter\def\csname pn@io.small.ovdalwaysdino.f1oracle\endcsname{0.39}
\expandafter\def\csname pn@io.small.ovdalwaysdino.auc\endcsname{0.77}
\expandafter\def\csname pn@io.small.ovdalwaysdino.thrmax\endcsname{$2.6{\times}10^{-2}$}
\expandafter\def\csname pn@io.small.ovdalwaysdino.thrmin\endcsname{$5.7{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.ovdgate55.f1half\endcsname{0.11}
\expandafter\def\csname pn@io.small.ovdgate55.f1val\endcsname{0.33}
\expandafter\def\csname pn@io.small.ovdgate55.f1valvat\endcsname{0.38}
\expandafter\def\csname pn@io.small.ovdgate55.f1oracle\endcsname{0.36}
\expandafter\def\csname pn@io.small.ovdgate55.auc\endcsname{0.76}
\expandafter\def\csname pn@io.small.ovdgate55.thrmax\endcsname{$6.5{\times}10^{-3}$}
\expandafter\def\csname pn@io.small.ovdgate55.thrmin\endcsname{$3.3{\times}10^{-4}$}
\expandafter\def\csname pn@io.small.ovdmixrand.f1half\endcsname{0.20}
\expandafter\def\csname pn@io.small.ovdmixrand.f1val\endcsname{0.35}
\expandafter\def\csname pn@io.small.ovdmixrand.f1valvat\endcsname{0.38}
\expandafter\def\csname pn@io.small.ovdmixrand.f1oracle\endcsname{0.39}
\expandafter\def\csname pn@io.small.ovdmixrand.auc\endcsname{0.77}
\expandafter\def\csname pn@io.small.ovdmixrand.thrmax\endcsname{$4.3{\times}10^{-3}$}
\expandafter\def\csname pn@io.small.ovdmixrand.thrmin\endcsname{$5.9{\times}10^{-5}$}
\expandafter\def\csname pn@io.small.f1half.min\endcsname{0.08}
\expandafter\def\csname pn@io.small.f1half.max\endcsname{0.23}
\expandafter\def\csname pn@io.small.f1val.min\endcsname{0.28}
\expandafter\def\csname pn@io.small.f1val.max\endcsname{0.39}
\expandafter\def\csname pn@io.small.auc.min\endcsname{0.67}
\expandafter\def\csname pn@io.small.auc.max\endcsname{0.78}
\expandafter\def\csname pn@io.small.thr.max\endcsname{$2.6{\times}10^{-2}$}
\expandafter\def\csname pn@io.small.thr.min\endcsname{$7.9{\times}10^{-6}$}
\expandafter\def\csname pn@headpos.tiny.gt.pooled\endcsname{0.199}
\expandafter\def\csname pn@headpos.tiny.gt.pooled4\endcsname{0.1989}
\expandafter\def\csname pn@headpos.tiny.gt.sd\endcsname{0.002}
\expandafter\def\csname pn@headpos.tiny.gt.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.tiny.gt.pck05\endcsname{0.062}
\expandafter\def\csname pn@headpos.tiny.gt.pck10\endcsname{0.218}
\expandafter\def\csname pn@headpos.tiny.gt.vat\endcsname{0.204}
\expandafter\def\csname pn@headpos.tiny.gt.vat.sd\endcsname{0.001}
\expandafter\def\csname pn@headpos.tiny.gt.childplay\endcsname{0.187}
\expandafter\def\csname pn@headpos.tiny.gt.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.gt.vacation\endcsname{0.212}
\expandafter\def\csname pn@headpos.tiny.gt.vacation.sd\endcsname{0.009}
\expandafter\def\csname pn@headpos.tiny.gt.social\endcsname{0.174}
\expandafter\def\csname pn@headpos.tiny.gt.social.sd\endcsname{0.001}
\expandafter\def\csname pn@headpos.tiny.gt.object\endcsname{0.220}
\expandafter\def\csname pn@headpos.tiny.gt.object.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.tiny.gt.collapse.min\endcsname{0.82}
\expandafter\def\csname pn@headpos.tiny.gt.collapse.max\endcsname{0.85}
\expandafter\def\csname pn@headpos.tiny.gt.collapse.mean\endcsname{0.83}
\expandafter\def\csname pn@headpos.tiny.gt.epochs\endcsname{11, 11, 7}
\expandafter\def\csname pn@headpos.tiny.gt.epoch.max\endcsname{11}
\expandafter\def\csname pn@headpos.tiny.gt.epoch.min\endcsname{7}
\expandafter\def\csname pn@headpos.tiny.gt.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.tiny.gt.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.tiny.gt.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.tiny.gt.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.tiny.gt.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.tiny.gt.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.pooled\endcsname{0.199}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.pooled4\endcsname{0.1989}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.sd\endcsname{0.002}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.pck05\endcsname{0.062}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.pck10\endcsname{0.218}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.vat\endcsname{0.204}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.vat.sd\endcsname{0.001}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.childplay\endcsname{0.187}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.vacation\endcsname{0.212}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.vacation.sd\endcsname{0.009}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.social\endcsname{0.174}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.social.sd\endcsname{0.001}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.object\endcsname{0.220}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.object.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.collapse.min\endcsname{0.82}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.collapse.max\endcsname{0.85}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.collapse.mean\endcsname{0.83}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.epochs\endcsname{11, 11, 7}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.epoch.max\endcsname{11}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.epoch.min\endcsname{7}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.tiny.gt.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.tiny.gt.val.vslabels\endcsname{0.204}
\expandafter\def\csname pn@headpos.tiny.gt.val.vsgt\endcsname{0.204}
\expandafter\def\csname pn@headpos.tiny.gazelle.pooled\endcsname{0.193}
\expandafter\def\csname pn@headpos.tiny.gazelle.pooled4\endcsname{0.1934}
\expandafter\def\csname pn@headpos.tiny.gazelle.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.tiny.gazelle.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.tiny.gazelle.pck05\endcsname{0.067}
\expandafter\def\csname pn@headpos.tiny.gazelle.pck10\endcsname{0.252}
\expandafter\def\csname pn@headpos.tiny.gazelle.vat\endcsname{0.195}
\expandafter\def\csname pn@headpos.tiny.gazelle.vat.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.tiny.gazelle.childplay\endcsname{0.183}
\expandafter\def\csname pn@headpos.tiny.gazelle.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.gazelle.vacation\endcsname{0.209}
\expandafter\def\csname pn@headpos.tiny.gazelle.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.tiny.gazelle.social\endcsname{0.165}
\expandafter\def\csname pn@headpos.tiny.gazelle.social.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.gazelle.object\endcsname{0.218}
\expandafter\def\csname pn@headpos.tiny.gazelle.object.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.gazelle.collapse.min\endcsname{0.75}
\expandafter\def\csname pn@headpos.tiny.gazelle.collapse.max\endcsname{0.83}
\expandafter\def\csname pn@headpos.tiny.gazelle.collapse.mean\endcsname{0.80}
\expandafter\def\csname pn@headpos.tiny.gazelle.epochs\endcsname{12, 12, 8}
\expandafter\def\csname pn@headpos.tiny.gazelle.epoch.max\endcsname{12}
\expandafter\def\csname pn@headpos.tiny.gazelle.epoch.min\endcsname{8}
\expandafter\def\csname pn@headpos.tiny.gazelle.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.tiny.gazelle.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.tiny.gazelle.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.tiny.gazelle.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.tiny.gazelle.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.tiny.gazelle.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.pooled\endcsname{0.193}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.pooled4\endcsname{0.1934}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.pck05\endcsname{0.065}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.pck10\endcsname{0.252}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.vat\endcsname{0.195}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.vat.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.childplay\endcsname{0.183}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.vacation\endcsname{0.208}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.vacation.sd\endcsname{0.003}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.social\endcsname{0.164}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.social.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.object\endcsname{0.218}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.object.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.collapse.min\endcsname{0.75}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.collapse.max\endcsname{0.84}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.collapse.mean\endcsname{0.81}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.epochs\endcsname{11, 12, 8}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.epoch.max\endcsname{12}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.epoch.min\endcsname{8}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.tiny.gazelle.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.tiny.gazelle.val.vslabels\endcsname{0.170}
\expandafter\def\csname pn@headpos.tiny.gazelle.val.vsgt\endcsname{0.192}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.pooled\endcsname{0.333}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.pooled4\endcsname{0.3327}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.sd\endcsname{0.003}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.pck05\endcsname{0.010}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.pck10\endcsname{0.047}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.vat\endcsname{0.333}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.vat.sd\endcsname{0.002}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.childplay\endcsname{0.323}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.childplay.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.vacation\endcsname{0.349}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.social\endcsname{0.311}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.social.sd\endcsname{0.003}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.object\endcsname{0.352}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.object.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.collapse.min\endcsname{0.69}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.collapse.max\endcsname{0.74}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.collapse.mean\endcsname{0.72}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.epochs\endcsname{9, 3, 7}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.epoch.max\endcsname{9}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.epoch.min\endcsname{3}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.pooled\endcsname{0.321}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.pooled4\endcsname{0.3213}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.pck05\endcsname{0.018}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.pck10\endcsname{0.062}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.vat\endcsname{0.313}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.vat.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.childplay\endcsname{0.328}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.childplay.sd\endcsname{0.009}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.vacation\endcsname{0.323}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.social\endcsname{0.280}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.social.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.object\endcsname{0.357}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.object.sd\endcsname{0.008}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.collapse.min\endcsname{0.40}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.collapse.max\endcsname{0.49}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.collapse.mean\endcsname{0.45}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.epochs\endcsname{1, 1, 1}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.epoch.max\endcsname{1}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.epoch.min\endcsname{1}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.val.vslabels\endcsname{0.154}
\expandafter\def\csname pn@headpos.tiny.vlmnoleak.val.vsgt\endcsname{0.331}
\expandafter\def\csname pn@headpos.small.gt.pooled\endcsname{0.186}
\expandafter\def\csname pn@headpos.small.gt.pooled4\endcsname{0.1860}
\expandafter\def\csname pn@headpos.small.gt.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.small.gt.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.small.gt.pck05\endcsname{0.078}
\expandafter\def\csname pn@headpos.small.gt.pck10\endcsname{0.273}
\expandafter\def\csname pn@headpos.small.gt.vat\endcsname{0.200}
\expandafter\def\csname pn@headpos.small.gt.vat.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gt.childplay\endcsname{0.167}
\expandafter\def\csname pn@headpos.small.gt.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.small.gt.vacation\endcsname{0.196}
\expandafter\def\csname pn@headpos.small.gt.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.small.gt.social\endcsname{0.164}
\expandafter\def\csname pn@headpos.small.gt.social.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gt.object\endcsname{0.205}
\expandafter\def\csname pn@headpos.small.gt.object.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gt.collapse.min\endcsname{0.81}
\expandafter\def\csname pn@headpos.small.gt.collapse.max\endcsname{0.91}
\expandafter\def\csname pn@headpos.small.gt.collapse.mean\endcsname{0.87}
\expandafter\def\csname pn@headpos.small.gt.epochs\endcsname{6, 9, 15}
\expandafter\def\csname pn@headpos.small.gt.epoch.max\endcsname{15}
\expandafter\def\csname pn@headpos.small.gt.epoch.min\endcsname{6}
\expandafter\def\csname pn@headpos.small.gt.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.small.gt.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.small.gt.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.small.gt.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.small.gt.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.small.gt.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.small.gt.gtsel.pooled\endcsname{0.186}
\expandafter\def\csname pn@headpos.small.gt.gtsel.pooled4\endcsname{0.1860}
\expandafter\def\csname pn@headpos.small.gt.gtsel.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.small.gt.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.small.gt.gtsel.pck05\endcsname{0.078}
\expandafter\def\csname pn@headpos.small.gt.gtsel.pck10\endcsname{0.273}
\expandafter\def\csname pn@headpos.small.gt.gtsel.vat\endcsname{0.200}
\expandafter\def\csname pn@headpos.small.gt.gtsel.vat.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gt.gtsel.childplay\endcsname{0.167}
\expandafter\def\csname pn@headpos.small.gt.gtsel.childplay.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.small.gt.gtsel.vacation\endcsname{0.196}
\expandafter\def\csname pn@headpos.small.gt.gtsel.vacation.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.small.gt.gtsel.social\endcsname{0.164}
\expandafter\def\csname pn@headpos.small.gt.gtsel.social.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gt.gtsel.object\endcsname{0.205}
\expandafter\def\csname pn@headpos.small.gt.gtsel.object.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gt.gtsel.collapse.min\endcsname{0.81}
\expandafter\def\csname pn@headpos.small.gt.gtsel.collapse.max\endcsname{0.91}
\expandafter\def\csname pn@headpos.small.gt.gtsel.collapse.mean\endcsname{0.87}
\expandafter\def\csname pn@headpos.small.gt.gtsel.epochs\endcsname{6, 9, 15}
\expandafter\def\csname pn@headpos.small.gt.gtsel.epoch.max\endcsname{15}
\expandafter\def\csname pn@headpos.small.gt.gtsel.epoch.min\endcsname{6}
\expandafter\def\csname pn@headpos.small.gt.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.small.gt.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.small.gt.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.small.gt.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.small.gt.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.small.gt.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.small.gt.val.vslabels\endcsname{0.183}
\expandafter\def\csname pn@headpos.small.gt.val.vsgt\endcsname{0.183}
\expandafter\def\csname pn@headpos.small.gazelle.pooled\endcsname{0.183}
\expandafter\def\csname pn@headpos.small.gazelle.pooled4\endcsname{0.1829}
\expandafter\def\csname pn@headpos.small.gazelle.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.small.gazelle.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.small.gazelle.pck05\endcsname{0.083}
\expandafter\def\csname pn@headpos.small.gazelle.pck10\endcsname{0.292}
\expandafter\def\csname pn@headpos.small.gazelle.vat\endcsname{0.193}
\expandafter\def\csname pn@headpos.small.gazelle.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.small.gazelle.childplay\endcsname{0.168}
\expandafter\def\csname pn@headpos.small.gazelle.childplay.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.small.gazelle.vacation\endcsname{0.192}
\expandafter\def\csname pn@headpos.small.gazelle.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.small.gazelle.social\endcsname{0.157}
\expandafter\def\csname pn@headpos.small.gazelle.social.sd\endcsname{0.003}
\expandafter\def\csname pn@headpos.small.gazelle.object\endcsname{0.205}
\expandafter\def\csname pn@headpos.small.gazelle.object.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gazelle.collapse.min\endcsname{0.79}
\expandafter\def\csname pn@headpos.small.gazelle.collapse.max\endcsname{0.82}
\expandafter\def\csname pn@headpos.small.gazelle.collapse.mean\endcsname{0.80}
\expandafter\def\csname pn@headpos.small.gazelle.epochs\endcsname{13, 11, 9}
\expandafter\def\csname pn@headpos.small.gazelle.epoch.max\endcsname{13}
\expandafter\def\csname pn@headpos.small.gazelle.epoch.min\endcsname{9}
\expandafter\def\csname pn@headpos.small.gazelle.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.small.gazelle.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.small.gazelle.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.small.gazelle.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.small.gazelle.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.small.gazelle.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.pooled\endcsname{0.183}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.pooled4\endcsname{0.1826}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.pck05\endcsname{0.086}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.pck10\endcsname{0.297}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.vat\endcsname{0.193}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.childplay\endcsname{0.168}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.childplay.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.vacation\endcsname{0.190}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.vacation.sd\endcsname{0.006}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.social\endcsname{0.156}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.social.sd\endcsname{0.005}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.object\endcsname{0.205}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.object.sd\endcsname{0.007}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.collapse.min\endcsname{0.80}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.collapse.max\endcsname{0.85}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.collapse.mean\endcsname{0.82}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.epochs\endcsname{13, 11, 11}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.epoch.max\endcsname{13}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.epoch.min\endcsname{11}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@headpos.small.gazelle.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@headpos.small.gazelle.val.vslabels\endcsname{0.151}
\expandafter\def\csname pn@headpos.small.gazelle.val.vsgt\endcsname{0.174}
\expandafter\def\csname pn@matched.tiny.gt.pooled\endcsname{0.208}
\expandafter\def\csname pn@matched.tiny.gt.pooled4\endcsname{0.2084}
\expandafter\def\csname pn@matched.tiny.gt.sd\endcsname{0.008}
\expandafter\def\csname pn@matched.tiny.gt.nseeds\endcsname{3}
\expandafter\def\csname pn@matched.tiny.gt.pck05\endcsname{0.054}
\expandafter\def\csname pn@matched.tiny.gt.pck10\endcsname{0.206}
\expandafter\def\csname pn@matched.tiny.gt.vat\endcsname{0.212}
\expandafter\def\csname pn@matched.tiny.gt.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@matched.tiny.gt.childplay\endcsname{0.198}
\expandafter\def\csname pn@matched.tiny.gt.childplay.sd\endcsname{0.016}
\expandafter\def\csname pn@matched.tiny.gt.vacation\endcsname{0.220}
\expandafter\def\csname pn@matched.tiny.gt.vacation.sd\endcsname{0.008}
\expandafter\def\csname pn@matched.tiny.gt.social\endcsname{0.173}
\expandafter\def\csname pn@matched.tiny.gt.social.sd\endcsname{0.007}
\expandafter\def\csname pn@matched.tiny.gt.object\endcsname{0.239}
\expandafter\def\csname pn@matched.tiny.gt.object.sd\endcsname{0.012}
\expandafter\def\csname pn@matched.tiny.gt.collapse.min\endcsname{0.82}
\expandafter\def\csname pn@matched.tiny.gt.collapse.max\endcsname{0.83}
\expandafter\def\csname pn@matched.tiny.gt.collapse.mean\endcsname{0.83}
\expandafter\def\csname pn@matched.tiny.gt.epochs\endcsname{2, 10, 13}
\expandafter\def\csname pn@matched.tiny.gt.epoch.max\endcsname{13}
\expandafter\def\csname pn@matched.tiny.gt.epoch.min\endcsname{2}
\expandafter\def\csname pn@matched.tiny.gt.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@matched.tiny.gt.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@matched.tiny.gt.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@matched.tiny.gt.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@matched.tiny.gt.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@matched.tiny.gt.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.pooled\endcsname{0.208}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.pooled4\endcsname{0.2084}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.sd\endcsname{0.008}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.pck05\endcsname{0.054}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.pck10\endcsname{0.206}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.vat\endcsname{0.212}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.vat.sd\endcsname{0.006}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.childplay\endcsname{0.198}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.childplay.sd\endcsname{0.016}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.vacation\endcsname{0.220}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.vacation.sd\endcsname{0.008}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.social\endcsname{0.173}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.social.sd\endcsname{0.007}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.object\endcsname{0.239}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.object.sd\endcsname{0.012}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.collapse.min\endcsname{0.82}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.collapse.max\endcsname{0.83}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.collapse.mean\endcsname{0.83}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.epochs\endcsname{2, 10, 13}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.epoch.max\endcsname{13}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.epoch.min\endcsname{2}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@matched.tiny.gt.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@matched.tiny.gt.val.vslabels\endcsname{0.210}
\expandafter\def\csname pn@matched.tiny.gt.val.vsgt\endcsname{0.210}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.pooled\endcsname{0.293}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.pooled4\endcsname{0.2933}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.sd\endcsname{0.008}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.nseeds\endcsname{3}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.pck05\endcsname{0.047}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.pck10\endcsname{0.162}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.vat\endcsname{0.247}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.childplay\endcsname{0.354}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.childplay.sd\endcsname{0.013}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.vacation\endcsname{0.268}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.vacation.sd\endcsname{0.007}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.social\endcsname{0.168}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.social.sd\endcsname{0.008}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.object\endcsname{0.401}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.object.sd\endcsname{0.009}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.collapse.min\endcsname{0.82}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.collapse.max\endcsname{0.89}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.collapse.mean\endcsname{0.85}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.epochs\endcsname{9, 8, 4}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.epoch.max\endcsname{9}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.epoch.min\endcsname{4}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.pooled\endcsname{0.289}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.pooled4\endcsname{0.2887}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.sd\endcsname{0.003}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.nseeds\endcsname{3}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.pck05\endcsname{0.048}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.pck10\endcsname{0.162}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.vat\endcsname{0.247}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.vat.sd\endcsname{0.004}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.childplay\endcsname{0.346}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.childplay.sd\endcsname{0.004}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.vacation\endcsname{0.261}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.vacation.sd\endcsname{0.005}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.social\endcsname{0.166}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.social.sd\endcsname{0.006}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.object\endcsname{0.394}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.object.sd\endcsname{0.001}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.collapse.min\endcsname{0.77}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.collapse.max\endcsname{0.87}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.collapse.mean\endcsname{0.81}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.epochs\endcsname{15, 7, 5}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.epoch.max\endcsname{15}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.epoch.min\endcsname{5}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.ntest\endcsname{51{,}591}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.ntest.vat\endcsname{19{,}563}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.ntest.childplay\endcsname{20{,}100}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.ntest.vacation\endcsname{11{,}928}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.ntest.social\endcsname{23{,}849}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.gtsel.ntest.object\endcsname{27{,}742}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.val.vslabels\endcsname{0.188}
\expandafter\def\csname pn@matched.tiny.teacher_internvl3_alone.val.vsgt\endcsname{0.304}
\expandafter\def\csname pn@tp.tiny.gt.h100.copy.ade\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.gt.h100.copy.obj\endcsname{0.233}
\expandafter\def\csname pn@tp.tiny.gt.h100.copy.soc\endcsname{0.176}
\expandafter\def\csname pn@tp.tiny.gt.h100.head.ade\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.gt.h100.head.obj\endcsname{0.233}
\expandafter\def\csname pn@tp.tiny.gt.h100.head.soc\endcsname{0.179}
\expandafter\def\csname pn@tp.tiny.gt.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.gt.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.gt.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.gt.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gt.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gt.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.gt.h100.shrink.ade\endcsname{0.209}
\expandafter\def\csname pn@tp.tiny.gt.h100.shrink.obj\endcsname{0.239}
\expandafter\def\csname pn@tp.tiny.gt.h100.shrink.soc\endcsname{0.176}
\expandafter\def\csname pn@tp.tiny.gt.h100.shrink.a\endcsname{0.07}
\expandafter\def\csname pn@tp.tiny.gt.h100.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.gt.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.copy.ade\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.copy.obj\endcsname{0.233}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.copy.soc\endcsname{0.176}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.head.ade\endcsname{0.209}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.head.obj\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.head.soc\endcsname{0.180}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.delta\endcsname{+0.004}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gt.h300.copy.ade\endcsname{0.208}
\expandafter\def\csname pn@tp.tiny.gt.h300.copy.obj\endcsname{0.235}
\expandafter\def\csname pn@tp.tiny.gt.h300.copy.soc\endcsname{0.179}
\expandafter\def\csname pn@tp.tiny.gt.h300.head.ade\endcsname{0.210}
\expandafter\def\csname pn@tp.tiny.gt.h300.head.obj\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.gt.h300.head.soc\endcsname{0.181}
\expandafter\def\csname pn@tp.tiny.gt.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.gt.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.gt.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.gt.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gt.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.gt.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.gt.h300.shrink.ade\endcsname{0.212}
\expandafter\def\csname pn@tp.tiny.gt.h300.shrink.obj\endcsname{0.242}
\expandafter\def\csname pn@tp.tiny.gt.h300.shrink.soc\endcsname{0.179}
\expandafter\def\csname pn@tp.tiny.gt.h300.shrink.a\endcsname{0.07}
\expandafter\def\csname pn@tp.tiny.gt.h300.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.gt.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.copy.ade\endcsname{0.208}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.copy.obj\endcsname{0.235}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.copy.soc\endcsname{0.179}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.head.ade\endcsname{0.210}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.head.obj\endcsname{0.235}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.head.soc\endcsname{0.182}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gt.h500.copy.ade\endcsname{0.211}
\expandafter\def\csname pn@tp.tiny.gt.h500.copy.obj\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.gt.h500.copy.soc\endcsname{0.181}
\expandafter\def\csname pn@tp.tiny.gt.h500.head.ade\endcsname{0.212}
\expandafter\def\csname pn@tp.tiny.gt.h500.head.obj\endcsname{0.239}
\expandafter\def\csname pn@tp.tiny.gt.h500.head.soc\endcsname{0.184}
\expandafter\def\csname pn@tp.tiny.gt.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.gt.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.gt.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.gt.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.gt.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gt.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.gt.h500.shrink.ade\endcsname{0.215}
\expandafter\def\csname pn@tp.tiny.gt.h500.shrink.obj\endcsname{0.245}
\expandafter\def\csname pn@tp.tiny.gt.h500.shrink.soc\endcsname{0.182}
\expandafter\def\csname pn@tp.tiny.gt.h500.shrink.a\endcsname{0.08}
\expandafter\def\csname pn@tp.tiny.gt.h500.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.gt.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.copy.ade\endcsname{0.211}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.copy.obj\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.copy.soc\endcsname{0.181}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.head.ade\endcsname{0.212}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.head.obj\endcsname{0.238}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.head.soc\endcsname{0.184}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gt.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gt.v.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.gt.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gt.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gt.v.object.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.gt.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gt.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gt.v.social.ns\endcsname{8}
\expandafter\def\csname pn@tp.tiny.gt.v.social.REALm\endcsname{1}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.copy.ade\endcsname{0.201}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.copy.obj\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.copy.soc\endcsname{0.166}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.head.ade\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.head.obj\endcsname{0.233}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.head.soc\endcsname{0.172}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.shrink.ade\endcsname{0.203}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.shrink.obj\endcsname{0.238}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.shrink.soc\endcsname{0.166}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.shrink.a\endcsname{0.07}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.copy.ade\endcsname{0.201}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.copy.obj\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.copy.soc\endcsname{0.166}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.head.ade\endcsname{0.202}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.head.obj\endcsname{0.230}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.head.soc\endcsname{0.173}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.delta\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.copy.ade\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.copy.obj\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.copy.soc\endcsname{0.169}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.head.ade\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.head.obj\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.head.soc\endcsname{0.174}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.shrink.ade\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.shrink.obj\endcsname{0.242}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.shrink.soc\endcsname{0.169}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.shrink.a\endcsname{0.08}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.delta\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.copy.ade\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.copy.obj\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.copy.soc\endcsname{0.169}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.head.ade\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.head.obj\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.head.soc\endcsname{0.175}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.delta\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.copy.ade\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.copy.obj\endcsname{0.240}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.copy.soc\endcsname{0.172}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.head.ade\endcsname{0.208}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.head.obj\endcsname{0.238}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.head.soc\endcsname{0.176}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.shrink.ade\endcsname{0.210}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.shrink.obj\endcsname{0.245}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.shrink.soc\endcsname{0.172}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.shrink.a\endcsname{0.09}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.delta\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.copy.ade\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.copy.obj\endcsname{0.240}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.copy.soc\endcsname{0.172}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.head.ade\endcsname{0.208}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.head.obj\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.head.soc\endcsname{0.177}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.delta\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.mtgs.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.mtgs.v.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.mtgs.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.mtgs.v.object.REALp\endcsname{1}
\expandafter\def\csname pn@tp.tiny.mtgs.v.object.ns\endcsname{8}
\expandafter\def\csname pn@tp.tiny.mtgs.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.mtgs.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.mtgs.v.social.ns\endcsname{6}
\expandafter\def\csname pn@tp.tiny.mtgs.v.social.REALm\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.copy.ade\endcsname{0.201}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.copy.obj\endcsname{0.231}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.copy.soc\endcsname{0.168}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.head.ade\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.head.obj\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.head.soc\endcsname{0.171}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.shrink.ade\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.shrink.obj\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.shrink.soc\endcsname{0.168}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.shrink.a\endcsname{0.03}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.delta\endcsname{+0.004}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.copy.ade\endcsname{0.201}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.copy.obj\endcsname{0.231}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.copy.soc\endcsname{0.168}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.head.ade\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.head.obj\endcsname{0.235}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.head.soc\endcsname{0.173}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.delta\endcsname{+0.004}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.copy.ade\endcsname{0.203}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.copy.obj\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.copy.soc\endcsname{0.170}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.head.ade\endcsname{0.206}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.head.obj\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.head.soc\endcsname{0.175}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.shrink.ade\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.shrink.obj\endcsname{0.240}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.shrink.soc\endcsname{0.171}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.shrink.a\endcsname{0.04}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.delta\endcsname{+0.003}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.copy.ade\endcsname{0.203}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.copy.obj\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.copy.soc\endcsname{0.170}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.head.ade\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.head.obj\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.head.soc\endcsname{0.176}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.delta\endcsname{+0.004}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.copy.ade\endcsname{0.206}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.copy.obj\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.copy.soc\endcsname{0.173}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.head.ade\endcsname{0.209}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.head.obj\endcsname{0.239}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.head.soc\endcsname{0.177}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.shrink.ade\endcsname{0.210}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.shrink.obj\endcsname{0.243}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.shrink.soc\endcsname{0.174}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.shrink.a\endcsname{0.05}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.delta\endcsname{+0.003}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.copy.ade\endcsname{0.206}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.copy.obj\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.copy.soc\endcsname{0.173}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.head.ade\endcsname{0.210}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.head.obj\endcsname{0.239}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.head.soc\endcsname{0.178}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.delta\endcsname{+0.004}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.gazelle.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gazelle.v.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.gazelle.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gazelle.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gazelle.v.object.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.gazelle.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gazelle.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.gazelle.v.social.ns\endcsname{8}
\expandafter\def\csname pn@tp.tiny.gazelle.v.social.REALm\endcsname{1}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.copy.ade\endcsname{0.242}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.copy.obj\endcsname{0.277}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.copy.soc\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.head.ade\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.head.obj\endcsname{0.268}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.head.soc\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.shrink.ade\endcsname{0.244}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.shrink.obj\endcsname{0.280}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.shrink.soc\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.shrink.a\endcsname{0.07}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.delta\endcsname{$-$0.005}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.copy.ade\endcsname{0.242}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.copy.obj\endcsname{0.277}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.copy.soc\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.head.ade\endcsname{0.239}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.head.obj\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.head.soc\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.delta\endcsname{$-$0.003}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.copy.ade\endcsname{0.243}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.copy.obj\endcsname{0.277}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.copy.soc\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.head.ade\endcsname{0.238}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.head.obj\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.head.soc\endcsname{0.202}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.shrink.ade\endcsname{0.245}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.shrink.obj\endcsname{0.281}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.shrink.soc\endcsname{0.206}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.shrink.a\endcsname{0.07}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.delta\endcsname{$-$0.005}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.copy.ade\endcsname{0.243}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.copy.obj\endcsname{0.277}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.copy.soc\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.head.ade\endcsname{0.240}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.head.obj\endcsname{0.273}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.head.soc\endcsname{0.203}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.delta\endcsname{$-$0.003}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.copy.ade\endcsname{0.244}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.copy.obj\endcsname{0.278}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.copy.soc\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.head.ade\endcsname{0.240}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.head.obj\endcsname{0.274}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.head.soc\endcsname{0.203}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.shrink.ade\endcsname{0.246}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.shrink.obj\endcsname{0.282}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.shrink.soc\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.shrink.a\endcsname{0.08}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.delta\endcsname{$-$0.004}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.copy.ade\endcsname{0.244}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.copy.obj\endcsname{0.278}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.copy.soc\endcsname{0.207}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.head.ade\endcsname{0.242}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.head.obj\endcsname{0.276}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.head.soc\endcsname{0.205}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.delta\endcsname{$-$0.002}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.object.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.social.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.v.social.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.copy.ade\endcsname{0.283}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.copy.obj\endcsname{0.394}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.copy.soc\endcsname{0.162}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.head.ade\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.head.obj\endcsname{0.325}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.head.soc\endcsname{0.212}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.shrink.ade\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.shrink.obj\endcsname{0.348}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.shrink.soc\endcsname{0.185}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.shrink.a\endcsname{0.41}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.delta\endcsname{$-$0.012}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.copy.ade\endcsname{0.283}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.copy.obj\endcsname{0.394}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.copy.soc\endcsname{0.162}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.head.ade\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.head.obj\endcsname{0.324}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.head.soc\endcsname{0.211}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.delta\endcsname{$-$0.013}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.copy.ade\endcsname{0.283}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.copy.obj\endcsname{0.394}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.copy.soc\endcsname{0.163}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.head.ade\endcsname{0.273}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.head.obj\endcsname{0.326}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.head.soc\endcsname{0.214}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.shrink.ade\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.shrink.obj\endcsname{0.347}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.shrink.soc\endcsname{0.186}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.shrink.a\endcsname{0.41}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.delta\endcsname{$-$0.010}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.copy.ade\endcsname{0.283}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.copy.obj\endcsname{0.394}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.copy.soc\endcsname{0.163}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.head.ade\endcsname{0.272}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.head.obj\endcsname{0.327}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.head.soc\endcsname{0.212}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.delta\endcsname{$-$0.011}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.copy.ade\endcsname{0.283}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.copy.obj\endcsname{0.393}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.copy.soc\endcsname{0.163}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.head.ade\endcsname{0.272}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.head.obj\endcsname{0.322}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.head.soc\endcsname{0.217}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.shrink.ade\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.shrink.obj\endcsname{0.347}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.shrink.soc\endcsname{0.185}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.shrink.a\endcsname{0.41}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.delta\endcsname{$-$0.011}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.copy.ade\endcsname{0.283}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.copy.obj\endcsname{0.393}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.copy.soc\endcsname{0.163}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.head.ade\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.head.obj\endcsname{0.323}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.head.soc\endcsname{0.215}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.delta\endcsname{$-$0.012}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.object.REALp\endcsname{9}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.object.ns\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.social.ns\endcsname{0}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.v.social.REALm\endcsname{9}
\expandafter\def\csname pn@tp.tiny.copyb.h100.copy.ade\endcsname{0.284}
\expandafter\def\csname pn@tp.tiny.copyb.h100.copy.obj\endcsname{0.403}
\expandafter\def\csname pn@tp.tiny.copyb.h100.copy.soc\endcsname{0.157}
\expandafter\def\csname pn@tp.tiny.copyb.h100.head.ade\endcsname{0.266}
\expandafter\def\csname pn@tp.tiny.copyb.h100.head.obj\endcsname{0.321}
\expandafter\def\csname pn@tp.tiny.copyb.h100.head.soc\endcsname{0.206}
\expandafter\def\csname pn@tp.tiny.copyb.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.copyb.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.copyb.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.copyb.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.copyb.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.copyb.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.copyb.h100.shrink.ade\endcsname{0.267}
\expandafter\def\csname pn@tp.tiny.copyb.h100.shrink.obj\endcsname{0.348}
\expandafter\def\csname pn@tp.tiny.copyb.h100.shrink.soc\endcsname{0.180}
\expandafter\def\csname pn@tp.tiny.copyb.h100.shrink.a\endcsname{0.42}
\expandafter\def\csname pn@tp.tiny.copyb.h100.delta\endcsname{$-$0.019}
\expandafter\def\csname pn@tp.tiny.copyb.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.copy.ade\endcsname{0.284}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.copy.obj\endcsname{0.403}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.copy.soc\endcsname{0.157}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.head.ade\endcsname{0.264}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.head.obj\endcsname{0.321}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.head.soc\endcsname{0.203}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.delta\endcsname{$-$0.020}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.copyb.h300.copy.ade\endcsname{0.285}
\expandafter\def\csname pn@tp.tiny.copyb.h300.copy.obj\endcsname{0.402}
\expandafter\def\csname pn@tp.tiny.copyb.h300.copy.soc\endcsname{0.158}
\expandafter\def\csname pn@tp.tiny.copyb.h300.head.ade\endcsname{0.265}
\expandafter\def\csname pn@tp.tiny.copyb.h300.head.obj\endcsname{0.322}
\expandafter\def\csname pn@tp.tiny.copyb.h300.head.soc\endcsname{0.203}
\expandafter\def\csname pn@tp.tiny.copyb.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.copyb.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.copyb.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.copyb.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.copyb.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.copyb.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.copyb.h300.shrink.ade\endcsname{0.267}
\expandafter\def\csname pn@tp.tiny.copyb.h300.shrink.obj\endcsname{0.348}
\expandafter\def\csname pn@tp.tiny.copyb.h300.shrink.soc\endcsname{0.180}
\expandafter\def\csname pn@tp.tiny.copyb.h300.shrink.a\endcsname{0.43}
\expandafter\def\csname pn@tp.tiny.copyb.h300.delta\endcsname{$-$0.020}
\expandafter\def\csname pn@tp.tiny.copyb.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.copy.ade\endcsname{0.285}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.copy.obj\endcsname{0.402}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.copy.soc\endcsname{0.158}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.head.ade\endcsname{0.266}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.head.obj\endcsname{0.323}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.head.soc\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.delta\endcsname{$-$0.020}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.copyb.h500.copy.ade\endcsname{0.285}
\expandafter\def\csname pn@tp.tiny.copyb.h500.copy.obj\endcsname{0.401}
\expandafter\def\csname pn@tp.tiny.copyb.h500.copy.soc\endcsname{0.158}
\expandafter\def\csname pn@tp.tiny.copyb.h500.head.ade\endcsname{0.264}
\expandafter\def\csname pn@tp.tiny.copyb.h500.head.obj\endcsname{0.317}
\expandafter\def\csname pn@tp.tiny.copyb.h500.head.soc\endcsname{0.206}
\expandafter\def\csname pn@tp.tiny.copyb.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.copyb.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.copyb.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.copyb.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.copyb.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.copyb.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.copyb.h500.shrink.ade\endcsname{0.267}
\expandafter\def\csname pn@tp.tiny.copyb.h500.shrink.obj\endcsname{0.348}
\expandafter\def\csname pn@tp.tiny.copyb.h500.shrink.soc\endcsname{0.179}
\expandafter\def\csname pn@tp.tiny.copyb.h500.shrink.a\endcsname{0.42}
\expandafter\def\csname pn@tp.tiny.copyb.h500.delta\endcsname{$-$0.021}
\expandafter\def\csname pn@tp.tiny.copyb.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.copy.ade\endcsname{0.285}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.copy.obj\endcsname{0.401}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.copy.soc\endcsname{0.158}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.head.ade\endcsname{0.265}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.head.obj\endcsname{0.320}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.head.soc\endcsname{0.204}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.delta\endcsname{$-$0.020}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.copyb.v.pooled.REALp\endcsname{3}
\expandafter\def\csname pn@tp.tiny.copyb.v.pooled.ns\endcsname{6}
\expandafter\def\csname pn@tp.tiny.copyb.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.copyb.v.object.REALp\endcsname{9}
\expandafter\def\csname pn@tp.tiny.copyb.v.object.ns\endcsname{0}
\expandafter\def\csname pn@tp.tiny.copyb.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.copyb.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.copyb.v.social.ns\endcsname{0}
\expandafter\def\csname pn@tp.tiny.copyb.v.social.REALm\endcsname{9}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.copy.ade\endcsname{0.331}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.copy.obj\endcsname{0.369}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.copy.soc\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.head.ade\endcsname{0.279}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.head.obj\endcsname{0.321}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.head.soc\endcsname{0.233}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.shrink.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.shrink.obj\endcsname{0.311}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.shrink.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.shrink.a\endcsname{0.96}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.delta\endcsname{$-$0.053}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.copy.ade\endcsname{0.331}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.copy.obj\endcsname{0.369}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.copy.soc\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.head.ade\endcsname{0.280}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.head.obj\endcsname{0.320}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.head.soc\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.delta\endcsname{$-$0.052}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.copy.ade\endcsname{0.330}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.copy.obj\endcsname{0.368}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.copy.soc\endcsname{0.289}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.head.ade\endcsname{0.279}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.head.obj\endcsname{0.321}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.head.soc\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.shrink.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.shrink.obj\endcsname{0.311}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.shrink.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.shrink.a\endcsname{0.96}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.delta\endcsname{$-$0.051}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.copy.ade\endcsname{0.330}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.copy.obj\endcsname{0.368}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.copy.soc\endcsname{0.289}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.head.ade\endcsname{0.280}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.head.obj\endcsname{0.320}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.head.soc\endcsname{0.237}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.delta\endcsname{$-$0.050}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.copy.ade\endcsname{0.329}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.copy.obj\endcsname{0.367}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.copy.soc\endcsname{0.289}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.head.ade\endcsname{0.280}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.head.obj\endcsname{0.322}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.head.soc\endcsname{0.234}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.shrink.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.shrink.obj\endcsname{0.311}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.shrink.soc\endcsname{0.268}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.shrink.a\endcsname{0.96}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.delta\endcsname{$-$0.050}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.copy.ade\endcsname{0.329}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.copy.obj\endcsname{0.367}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.copy.soc\endcsname{0.289}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.head.ade\endcsname{0.280}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.head.obj\endcsname{0.322}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.head.soc\endcsname{0.236}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.delta\endcsname{$-$0.049}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.pooled.REALp\endcsname{9}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.pooled.ns\endcsname{0}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.object.REALp\endcsname{9}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.object.ns\endcsname{0}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.social.REALp\endcsname{9}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.social.ns\endcsname{0}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.v.social.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.copy.ade\endcsname{0.274}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.copy.obj\endcsname{0.288}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.copy.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.head.ade\endcsname{0.267}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.head.obj\endcsname{0.286}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.head.soc\endcsname{0.246}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.shrink.ade\endcsname{0.278}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.shrink.obj\endcsname{0.296}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.shrink.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.shrink.a\endcsname{0.11}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.delta\endcsname{$-$0.007}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.copy.ade\endcsname{0.274}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.copy.obj\endcsname{0.288}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.copy.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.head.ade\endcsname{0.272}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.head.obj\endcsname{0.292}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.head.soc\endcsname{0.249}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.delta\endcsname{$-$0.002}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.copy.ade\endcsname{0.273}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.copy.obj\endcsname{0.286}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.copy.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.head.ade\endcsname{0.267}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.head.obj\endcsname{0.287}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.head.soc\endcsname{0.246}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.shrink.ade\endcsname{0.278}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.shrink.obj\endcsname{0.295}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.shrink.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.shrink.a\endcsname{0.12}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.delta\endcsname{$-$0.006}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.copy.ade\endcsname{0.273}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.copy.obj\endcsname{0.286}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.copy.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.head.ade\endcsname{0.272}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.head.obj\endcsname{0.295}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.head.soc\endcsname{0.247}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.delta\endcsname{$-$0.001}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.copy.ade\endcsname{0.273}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.copy.obj\endcsname{0.285}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.copy.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.head.ade\endcsname{0.268}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.head.obj\endcsname{0.287}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.head.soc\endcsname{0.247}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.shrink.ade\endcsname{0.278}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.shrink.obj\endcsname{0.295}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.shrink.soc\endcsname{0.260}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.shrink.a\endcsname{0.13}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.delta\endcsname{$-$0.005}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.copy.ade\endcsname{0.273}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.copy.obj\endcsname{0.285}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.copy.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.head.ade\endcsname{0.272}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.head.obj\endcsname{0.294}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.head.soc\endcsname{0.248}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.delta\endcsname{$-$0.001}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctx1.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.pooled.REALp\endcsname{1}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.pooled.ns\endcsname{8}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.object.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.social.REALp\endcsname{6}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.social.ns\endcsname{3}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.v.social.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.pooled.REALp\endcsname{47}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.pooled.REALm\endcsname{16}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.pooled.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.object.REALp\endcsname{50}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.object.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.object.REALm\endcsname{13}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.object.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.social.REALp\endcsname{29}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.social.ns\endcsname{1}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.social.REALm\endcsname{42}
\expandafter\def\csname pn@tp.tiny.proto.evalpick_row.social.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.pooled.REALp\endcsname{42}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.pooled.ns\endcsname{10}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.pooled.REALm\endcsname{20}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.pooled.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.object.REALp\endcsname{43}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.object.ns\endcsname{14}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.object.REALm\endcsname{15}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.object.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.social.REALp\endcsname{24}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.social.ns\endcsname{9}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.social.REALm\endcsname{39}
\expandafter\def\csname pn@tp.tiny.proto.sel_row.social.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.pooled.REALp\endcsname{13}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.pooled.ns\endcsname{59}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.pooled.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.object.REALp\endcsname{28}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.object.ns\endcsname{44}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.object.total\endcsname{72}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.social.REALp\endcsname{15}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.social.ns\endcsname{34}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.social.REALm\endcsname{23}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.social.total\endcsname{72}
\expandafter\def\csname pn@tp.h100.rows\endcsname{12{,}441}
\expandafter\def\csname pn@tp.h100.matched\endcsname{12{,}335}
\expandafter\def\csname pn@tp.h100.clips\endcsname{175}
\expandafter\def\csname pn@tp.h300.rows\endcsname{11{,}484}
\expandafter\def\csname pn@tp.h300.matched\endcsname{11{,}227}
\expandafter\def\csname pn@tp.h300.clips\endcsname{175}
\expandafter\def\csname pn@tp.h500.rows\endcsname{10{,}763}
\expandafter\def\csname pn@tp.h500.matched\endcsname{10{,}389}
\expandafter\def\csname pn@tp.h500.clips\endcsname{174}
\expandafter\def\csname pn@tp.tiny.selected.ResidualTransformer\endcsname{106}
\expandafter\def\csname pn@tp.tiny.selected.Transformer\endcsname{136}
\expandafter\def\csname pn@tp.tiny.selected.ResidualGRU\endcsname{78}
\expandafter\def\csname pn@tp.tiny.selected.GRU\endcsname{40}
\expandafter\def\csname pn@tp.tiny.selected.total\endcsname{360}
\expandafter\def\csname pn@tp.tiny.runs\endcsname{72}
\expandafter\def\csname pn@tp.globalmean.h100\endcsname{0.291}
\expandafter\def\csname pn@tp.tiny.gt.h100.ctxdiff\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.gt.h300.ctxdiff\endcsname{0.000}
\expandafter\def\csname pn@tp.tiny.gt.h500.ctxdiff\endcsname{0.000}
\expandafter\def\csname pn@tp.tiny.mtgs.h100.ctxdiff\endcsname{$-$0.001}
\expandafter\def\csname pn@tp.tiny.mtgs.h300.ctxdiff\endcsname{0.000}
\expandafter\def\csname pn@tp.tiny.mtgs.h500.ctxdiff\endcsname{0.000}
\expandafter\def\csname pn@tp.tiny.gazelle.h100.ctxdiff\endcsname{0.000}
\expandafter\def\csname pn@tp.tiny.gazelle.h300.ctxdiff\endcsname{0.000}
\expandafter\def\csname pn@tp.tiny.gazelle.h500.ctxdiff\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h100.ctxdiff\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h300.ctxdiff\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.teacher_hybrid.h500.ctxdiff\endcsname{+0.002}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h100.ctxdiff\endcsname{0.000}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h300.ctxdiff\endcsname{$-$0.001}
\expandafter\def\csname pn@tp.tiny.teacher_internvl3_alone.h500.ctxdiff\endcsname{$-$0.001}
\expandafter\def\csname pn@tp.tiny.copyb.h100.ctxdiff\endcsname{$-$0.001}
\expandafter\def\csname pn@tp.tiny.copyb.h300.ctxdiff\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.copyb.h500.ctxdiff\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h100.ctxdiff\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h300.ctxdiff\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.vlmnoleak.h500.ctxdiff\endcsname{+0.001}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h100.ctxdiff\endcsname{+0.005}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h300.ctxdiff\endcsname{+0.005}
\expandafter\def\csname pn@tp.tiny.ovdalwaysdino.h500.ctxdiff\endcsname{+0.005}
\expandafter\def\csname pn@tp.tiny.ctxdiff.maxabs\endcsname{0.005}
\expandafter\def\csname pn@tp.small.gt.h100.copy.ade\endcsname{0.193}
\expandafter\def\csname pn@tp.small.gt.h100.copy.obj\endcsname{0.222}
\expandafter\def\csname pn@tp.small.gt.h100.copy.soc\endcsname{0.162}
\expandafter\def\csname pn@tp.small.gt.h100.head.ade\endcsname{0.197}
\expandafter\def\csname pn@tp.small.gt.h100.head.obj\endcsname{0.229}
\expandafter\def\csname pn@tp.small.gt.h100.head.soc\endcsname{0.163}
\expandafter\def\csname pn@tp.small.gt.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.gt.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.gt.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.gt.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.gt.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.gt.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.gt.h100.shrink.ade\endcsname{0.194}
\expandafter\def\csname pn@tp.small.gt.h100.shrink.obj\endcsname{0.224}
\expandafter\def\csname pn@tp.small.gt.h100.shrink.soc\endcsname{0.162}
\expandafter\def\csname pn@tp.small.gt.h100.shrink.a\endcsname{0.04}
\expandafter\def\csname pn@tp.small.gt.h100.delta\endcsname{+0.004}
\expandafter\def\csname pn@tp.small.gt.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.gt.h300.copy.ade\endcsname{0.196}
\expandafter\def\csname pn@tp.small.gt.h300.copy.obj\endcsname{0.225}
\expandafter\def\csname pn@tp.small.gt.h300.copy.soc\endcsname{0.166}
\expandafter\def\csname pn@tp.small.gt.h300.head.ade\endcsname{0.199}
\expandafter\def\csname pn@tp.small.gt.h300.head.obj\endcsname{0.229}
\expandafter\def\csname pn@tp.small.gt.h300.head.soc\endcsname{0.167}
\expandafter\def\csname pn@tp.small.gt.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.gt.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.gt.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.gt.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.gt.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.gt.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.gt.h300.shrink.ade\endcsname{0.198}
\expandafter\def\csname pn@tp.small.gt.h300.shrink.obj\endcsname{0.227}
\expandafter\def\csname pn@tp.small.gt.h300.shrink.soc\endcsname{0.166}
\expandafter\def\csname pn@tp.small.gt.h300.shrink.a\endcsname{0.04}
\expandafter\def\csname pn@tp.small.gt.h300.delta\endcsname{+0.003}
\expandafter\def\csname pn@tp.small.gt.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.gt.h500.copy.ade\endcsname{0.200}
\expandafter\def\csname pn@tp.small.gt.h500.copy.obj\endcsname{0.227}
\expandafter\def\csname pn@tp.small.gt.h500.copy.soc\endcsname{0.169}
\expandafter\def\csname pn@tp.small.gt.h500.head.ade\endcsname{0.203}
\expandafter\def\csname pn@tp.small.gt.h500.head.obj\endcsname{0.232}
\expandafter\def\csname pn@tp.small.gt.h500.head.soc\endcsname{0.171}
\expandafter\def\csname pn@tp.small.gt.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.gt.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.gt.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.gt.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.gt.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.gt.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.gt.h500.shrink.ade\endcsname{0.201}
\expandafter\def\csname pn@tp.small.gt.h500.shrink.obj\endcsname{0.230}
\expandafter\def\csname pn@tp.small.gt.h500.shrink.soc\endcsname{0.169}
\expandafter\def\csname pn@tp.small.gt.h500.shrink.a\endcsname{0.05}
\expandafter\def\csname pn@tp.small.gt.h500.delta\endcsname{+0.003}
\expandafter\def\csname pn@tp.small.gt.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.gt.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.gt.v.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.small.gt.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.gt.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.gt.v.object.ns\endcsname{6}
\expandafter\def\csname pn@tp.small.gt.v.object.REALm\endcsname{3}
\expandafter\def\csname pn@tp.small.gt.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.gt.v.social.ns\endcsname{7}
\expandafter\def\csname pn@tp.small.gt.v.social.REALm\endcsname{2}
\expandafter\def\csname pn@tp.small.mtgs.h100.copy.ade\endcsname{0.183}
\expandafter\def\csname pn@tp.small.mtgs.h100.copy.obj\endcsname{0.217}
\expandafter\def\csname pn@tp.small.mtgs.h100.copy.soc\endcsname{0.146}
\expandafter\def\csname pn@tp.small.mtgs.h100.head.ade\endcsname{0.185}
\expandafter\def\csname pn@tp.small.mtgs.h100.head.obj\endcsname{0.217}
\expandafter\def\csname pn@tp.small.mtgs.h100.head.soc\endcsname{0.150}
\expandafter\def\csname pn@tp.small.mtgs.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.mtgs.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.mtgs.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.mtgs.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.mtgs.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.mtgs.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.mtgs.h100.shrink.ade\endcsname{0.184}
\expandafter\def\csname pn@tp.small.mtgs.h100.shrink.obj\endcsname{0.219}
\expandafter\def\csname pn@tp.small.mtgs.h100.shrink.soc\endcsname{0.146}
\expandafter\def\csname pn@tp.small.mtgs.h100.shrink.a\endcsname{0.04}
\expandafter\def\csname pn@tp.small.mtgs.h100.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.small.mtgs.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.mtgs.h300.copy.ade\endcsname{0.187}
\expandafter\def\csname pn@tp.small.mtgs.h300.copy.obj\endcsname{0.221}
\expandafter\def\csname pn@tp.small.mtgs.h300.copy.soc\endcsname{0.150}
\expandafter\def\csname pn@tp.small.mtgs.h300.head.ade\endcsname{0.189}
\expandafter\def\csname pn@tp.small.mtgs.h300.head.obj\endcsname{0.221}
\expandafter\def\csname pn@tp.small.mtgs.h300.head.soc\endcsname{0.154}
\expandafter\def\csname pn@tp.small.mtgs.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.mtgs.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.mtgs.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.mtgs.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.mtgs.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.mtgs.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.mtgs.h300.shrink.ade\endcsname{0.188}
\expandafter\def\csname pn@tp.small.mtgs.h300.shrink.obj\endcsname{0.223}
\expandafter\def\csname pn@tp.small.mtgs.h300.shrink.soc\endcsname{0.149}
\expandafter\def\csname pn@tp.small.mtgs.h300.shrink.a\endcsname{0.05}
\expandafter\def\csname pn@tp.small.mtgs.h300.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.small.mtgs.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.mtgs.h500.copy.ade\endcsname{0.190}
\expandafter\def\csname pn@tp.small.mtgs.h500.copy.obj\endcsname{0.224}
\expandafter\def\csname pn@tp.small.mtgs.h500.copy.soc\endcsname{0.154}
\expandafter\def\csname pn@tp.small.mtgs.h500.head.ade\endcsname{0.193}
\expandafter\def\csname pn@tp.small.mtgs.h500.head.obj\endcsname{0.225}
\expandafter\def\csname pn@tp.small.mtgs.h500.head.soc\endcsname{0.158}
\expandafter\def\csname pn@tp.small.mtgs.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.mtgs.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.mtgs.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.mtgs.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.mtgs.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.mtgs.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.mtgs.h500.shrink.ade\endcsname{0.191}
\expandafter\def\csname pn@tp.small.mtgs.h500.shrink.obj\endcsname{0.227}
\expandafter\def\csname pn@tp.small.mtgs.h500.shrink.soc\endcsname{0.153}
\expandafter\def\csname pn@tp.small.mtgs.h500.shrink.a\endcsname{0.06}
\expandafter\def\csname pn@tp.small.mtgs.h500.delta\endcsname{+0.002}
\expandafter\def\csname pn@tp.small.mtgs.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.mtgs.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.mtgs.v.pooled.ns\endcsname{7}
\expandafter\def\csname pn@tp.small.mtgs.v.pooled.REALm\endcsname{2}
\expandafter\def\csname pn@tp.small.mtgs.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.mtgs.v.object.ns\endcsname{9}
\expandafter\def\csname pn@tp.small.mtgs.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.mtgs.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.mtgs.v.social.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.mtgs.v.social.REALm\endcsname{9}
\expandafter\def\csname pn@tp.small.gazelle.h100.copy.ade\endcsname{0.184}
\expandafter\def\csname pn@tp.small.gazelle.h100.copy.obj\endcsname{0.209}
\expandafter\def\csname pn@tp.small.gazelle.h100.copy.soc\endcsname{0.157}
\expandafter\def\csname pn@tp.small.gazelle.h100.head.ade\endcsname{0.187}
\expandafter\def\csname pn@tp.small.gazelle.h100.head.obj\endcsname{0.214}
\expandafter\def\csname pn@tp.small.gazelle.h100.head.soc\endcsname{0.159}
\expandafter\def\csname pn@tp.small.gazelle.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.gazelle.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.gazelle.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.gazelle.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.gazelle.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.gazelle.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.gazelle.h100.shrink.ade\endcsname{0.184}
\expandafter\def\csname pn@tp.small.gazelle.h100.shrink.obj\endcsname{0.210}
\expandafter\def\csname pn@tp.small.gazelle.h100.shrink.soc\endcsname{0.157}
\expandafter\def\csname pn@tp.small.gazelle.h100.shrink.a\endcsname{0.01}
\expandafter\def\csname pn@tp.small.gazelle.h100.delta\endcsname{+0.003}
\expandafter\def\csname pn@tp.small.gazelle.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.gazelle.h300.copy.ade\endcsname{0.187}
\expandafter\def\csname pn@tp.small.gazelle.h300.copy.obj\endcsname{0.212}
\expandafter\def\csname pn@tp.small.gazelle.h300.copy.soc\endcsname{0.160}
\expandafter\def\csname pn@tp.small.gazelle.h300.head.ade\endcsname{0.192}
\expandafter\def\csname pn@tp.small.gazelle.h300.head.obj\endcsname{0.219}
\expandafter\def\csname pn@tp.small.gazelle.h300.head.soc\endcsname{0.162}
\expandafter\def\csname pn@tp.small.gazelle.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.gazelle.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.gazelle.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.gazelle.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.gazelle.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.gazelle.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.gazelle.h300.shrink.ade\endcsname{0.188}
\expandafter\def\csname pn@tp.small.gazelle.h300.shrink.obj\endcsname{0.214}
\expandafter\def\csname pn@tp.small.gazelle.h300.shrink.soc\endcsname{0.160}
\expandafter\def\csname pn@tp.small.gazelle.h300.shrink.a\endcsname{0.01}
\expandafter\def\csname pn@tp.small.gazelle.h300.delta\endcsname{+0.005}
\expandafter\def\csname pn@tp.small.gazelle.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.gazelle.h500.copy.ade\endcsname{0.190}
\expandafter\def\csname pn@tp.small.gazelle.h500.copy.obj\endcsname{0.214}
\expandafter\def\csname pn@tp.small.gazelle.h500.copy.soc\endcsname{0.164}
\expandafter\def\csname pn@tp.small.gazelle.h500.head.ade\endcsname{0.195}
\expandafter\def\csname pn@tp.small.gazelle.h500.head.obj\endcsname{0.222}
\expandafter\def\csname pn@tp.small.gazelle.h500.head.soc\endcsname{0.166}
\expandafter\def\csname pn@tp.small.gazelle.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.gazelle.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.gazelle.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.gazelle.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.gazelle.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.gazelle.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.gazelle.h500.shrink.ade\endcsname{0.191}
\expandafter\def\csname pn@tp.small.gazelle.h500.shrink.obj\endcsname{0.217}
\expandafter\def\csname pn@tp.small.gazelle.h500.shrink.soc\endcsname{0.164}
\expandafter\def\csname pn@tp.small.gazelle.h500.shrink.a\endcsname{0.01}
\expandafter\def\csname pn@tp.small.gazelle.h500.delta\endcsname{+0.005}
\expandafter\def\csname pn@tp.small.gazelle.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.gazelle.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.gazelle.v.pooled.ns\endcsname{3}
\expandafter\def\csname pn@tp.small.gazelle.v.pooled.REALm\endcsname{6}
\expandafter\def\csname pn@tp.small.gazelle.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.gazelle.v.object.ns\endcsname{7}
\expandafter\def\csname pn@tp.small.gazelle.v.object.REALm\endcsname{2}
\expandafter\def\csname pn@tp.small.gazelle.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.gazelle.v.social.ns\endcsname{8}
\expandafter\def\csname pn@tp.small.gazelle.v.social.REALm\endcsname{1}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.copy.ade\endcsname{0.233}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.copy.obj\endcsname{0.273}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.copy.soc\endcsname{0.191}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.head.ade\endcsname{0.230}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.head.obj\endcsname{0.266}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.head.soc\endcsname{0.191}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.shrink.ade\endcsname{0.234}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.shrink.obj\endcsname{0.275}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.shrink.soc\endcsname{0.191}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.shrink.a\endcsname{0.05}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.delta\endcsname{$-$0.004}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.copy.ade\endcsname{0.236}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.copy.obj\endcsname{0.275}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.copy.soc\endcsname{0.193}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.head.ade\endcsname{0.232}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.head.obj\endcsname{0.268}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.head.soc\endcsname{0.194}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.shrink.ade\endcsname{0.237}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.shrink.obj\endcsname{0.276}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.shrink.soc\endcsname{0.194}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.shrink.a\endcsname{0.06}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.delta\endcsname{$-$0.003}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.copy.ade\endcsname{0.238}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.copy.obj\endcsname{0.277}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.copy.soc\endcsname{0.195}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.head.ade\endcsname{0.235}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.head.obj\endcsname{0.271}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.head.soc\endcsname{0.196}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.shrink.ade\endcsname{0.239}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.shrink.obj\endcsname{0.278}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.shrink.soc\endcsname{0.196}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.shrink.a\endcsname{0.07}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.delta\endcsname{$-$0.003}
\expandafter\def\csname pn@tp.small.teacher_hybrid.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.pooled.ns\endcsname{9}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.object.REALp\endcsname{2}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.object.ns\endcsname{7}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.social.ns\endcsname{9}
\expandafter\def\csname pn@tp.small.teacher_hybrid.v.social.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.copy.ade\endcsname{0.280}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.copy.obj\endcsname{0.401}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.copy.soc\endcsname{0.151}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.head.ade\endcsname{0.255}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.head.obj\endcsname{0.302}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.head.soc\endcsname{0.205}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.shrink.ade\endcsname{0.266}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.shrink.obj\endcsname{0.352}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.shrink.soc\endcsname{0.174}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.shrink.a\endcsname{0.38}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.delta\endcsname{$-$0.025}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.copy.ade\endcsname{0.280}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.copy.obj\endcsname{0.399}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.copy.soc\endcsname{0.151}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.head.ade\endcsname{0.258}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.head.obj\endcsname{0.306}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.head.soc\endcsname{0.205}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.shrink.ade\endcsname{0.266}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.shrink.obj\endcsname{0.351}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.shrink.soc\endcsname{0.174}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.shrink.a\endcsname{0.38}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.delta\endcsname{$-$0.023}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.copy.ade\endcsname{0.280}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.copy.obj\endcsname{0.398}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.copy.soc\endcsname{0.152}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.head.ade\endcsname{0.260}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.head.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.head.soc\endcsname{0.207}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.shrink.ade\endcsname{0.266}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.shrink.obj\endcsname{0.351}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.shrink.soc\endcsname{0.174}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.shrink.a\endcsname{0.38}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.delta\endcsname{$-$0.020}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.pooled.REALp\endcsname{6}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.pooled.ns\endcsname{3}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.object.REALp\endcsname{9}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.object.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.social.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.teacher_internvl3_alone.v.social.REALm\endcsname{9}
\expandafter\def\csname pn@tp.small.copyb.h100.copy.ade\endcsname{0.277}
\expandafter\def\csname pn@tp.small.copyb.h100.copy.obj\endcsname{0.403}
\expandafter\def\csname pn@tp.small.copyb.h100.copy.soc\endcsname{0.142}
\expandafter\def\csname pn@tp.small.copyb.h100.head.ade\endcsname{0.259}
\expandafter\def\csname pn@tp.small.copyb.h100.head.obj\endcsname{0.318}
\expandafter\def\csname pn@tp.small.copyb.h100.head.soc\endcsname{0.196}
\expandafter\def\csname pn@tp.small.copyb.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.copyb.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.copyb.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.copyb.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.copyb.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.copyb.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.copyb.h100.shrink.ade\endcsname{0.264}
\expandafter\def\csname pn@tp.small.copyb.h100.shrink.obj\endcsname{0.354}
\expandafter\def\csname pn@tp.small.copyb.h100.shrink.soc\endcsname{0.168}
\expandafter\def\csname pn@tp.small.copyb.h100.shrink.a\endcsname{0.37}
\expandafter\def\csname pn@tp.small.copyb.h100.delta\endcsname{$-$0.018}
\expandafter\def\csname pn@tp.small.copyb.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.copyb.h300.copy.ade\endcsname{0.278}
\expandafter\def\csname pn@tp.small.copyb.h300.copy.obj\endcsname{0.402}
\expandafter\def\csname pn@tp.small.copyb.h300.copy.soc\endcsname{0.143}
\expandafter\def\csname pn@tp.small.copyb.h300.head.ade\endcsname{0.258}
\expandafter\def\csname pn@tp.small.copyb.h300.head.obj\endcsname{0.315}
\expandafter\def\csname pn@tp.small.copyb.h300.head.soc\endcsname{0.196}
\expandafter\def\csname pn@tp.small.copyb.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.copyb.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.copyb.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.copyb.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.copyb.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.copyb.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.copyb.h300.shrink.ade\endcsname{0.264}
\expandafter\def\csname pn@tp.small.copyb.h300.shrink.obj\endcsname{0.353}
\expandafter\def\csname pn@tp.small.copyb.h300.shrink.soc\endcsname{0.168}
\expandafter\def\csname pn@tp.small.copyb.h300.shrink.a\endcsname{0.37}
\expandafter\def\csname pn@tp.small.copyb.h300.delta\endcsname{$-$0.020}
\expandafter\def\csname pn@tp.small.copyb.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.copyb.h500.copy.ade\endcsname{0.278}
\expandafter\def\csname pn@tp.small.copyb.h500.copy.obj\endcsname{0.401}
\expandafter\def\csname pn@tp.small.copyb.h500.copy.soc\endcsname{0.144}
\expandafter\def\csname pn@tp.small.copyb.h500.head.ade\endcsname{0.259}
\expandafter\def\csname pn@tp.small.copyb.h500.head.obj\endcsname{0.318}
\expandafter\def\csname pn@tp.small.copyb.h500.head.soc\endcsname{0.196}
\expandafter\def\csname pn@tp.small.copyb.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.copyb.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.copyb.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.copyb.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.copyb.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.copyb.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.copyb.h500.shrink.ade\endcsname{0.264}
\expandafter\def\csname pn@tp.small.copyb.h500.shrink.obj\endcsname{0.352}
\expandafter\def\csname pn@tp.small.copyb.h500.shrink.soc\endcsname{0.168}
\expandafter\def\csname pn@tp.small.copyb.h500.shrink.a\endcsname{0.37}
\expandafter\def\csname pn@tp.small.copyb.h500.delta\endcsname{$-$0.019}
\expandafter\def\csname pn@tp.small.copyb.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.copyb.v.pooled.REALp\endcsname{4}
\expandafter\def\csname pn@tp.small.copyb.v.pooled.ns\endcsname{5}
\expandafter\def\csname pn@tp.small.copyb.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.copyb.v.object.REALp\endcsname{9}
\expandafter\def\csname pn@tp.small.copyb.v.object.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.copyb.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.copyb.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@tp.small.copyb.v.social.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.copyb.v.social.REALm\endcsname{9}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.copy.ade\endcsname{0.330}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.copy.obj\endcsname{0.362}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.copy.soc\endcsname{0.297}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.head.ade\endcsname{0.276}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.head.obj\endcsname{0.314}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.head.soc\endcsname{0.235}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.shrink.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.shrink.obj\endcsname{0.311}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.shrink.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.shrink.a\endcsname{0.91}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.delta\endcsname{$-$0.055}
\expandafter\def\csname pn@tp.small.vlmnoleak.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.copy.ade\endcsname{0.329}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.copy.obj\endcsname{0.360}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.copy.soc\endcsname{0.296}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.head.ade\endcsname{0.277}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.head.obj\endcsname{0.315}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.head.soc\endcsname{0.236}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.shrink.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.shrink.obj\endcsname{0.311}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.shrink.soc\endcsname{0.268}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.shrink.a\endcsname{0.90}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.delta\endcsname{$-$0.052}
\expandafter\def\csname pn@tp.small.vlmnoleak.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.copy.ade\endcsname{0.328}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.copy.obj\endcsname{0.358}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.copy.soc\endcsname{0.296}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.head.ade\endcsname{0.278}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.head.obj\endcsname{0.317}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.head.soc\endcsname{0.236}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.shrink.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.shrink.obj\endcsname{0.311}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.shrink.soc\endcsname{0.267}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.shrink.a\endcsname{0.90}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.delta\endcsname{$-$0.050}
\expandafter\def\csname pn@tp.small.vlmnoleak.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.pooled.REALp\endcsname{9}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.pooled.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.object.REALp\endcsname{9}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.object.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.social.REALp\endcsname{9}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.social.ns\endcsname{0}
\expandafter\def\csname pn@tp.small.vlmnoleak.v.social.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.copy.ade\endcsname{0.274}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.copy.obj\endcsname{0.280}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.copy.soc\endcsname{0.266}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.head.ade\endcsname{0.251}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.head.obj\endcsname{0.272}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.head.soc\endcsname{0.228}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.lkgt.ade\endcsname{0.012}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.lkgt.obj\endcsname{0.013}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.lkgt.soc\endcsname{0.010}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.mean.soc\endcsname{0.271}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.shrink.ade\endcsname{0.272}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.shrink.obj\endcsname{0.285}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.shrink.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.shrink.a\endcsname{0.20}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.delta\endcsname{$-$0.023}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h100.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.copy.ade\endcsname{0.274}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.copy.obj\endcsname{0.280}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.copy.soc\endcsname{0.267}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.head.ade\endcsname{0.255}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.head.obj\endcsname{0.278}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.head.soc\endcsname{0.231}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.mean.ade\endcsname{0.291}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.mean.obj\endcsname{0.309}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.mean.soc\endcsname{0.270}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.shrink.ade\endcsname{0.273}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.shrink.obj\endcsname{0.285}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.shrink.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.shrink.a\endcsname{0.20}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.delta\endcsname{$-$0.018}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.copy.ade\endcsname{0.274}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.copy.obj\endcsname{0.280}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.copy.soc\endcsname{0.267}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.head.ade\endcsname{0.255}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.head.obj\endcsname{0.278}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.head.soc\endcsname{0.231}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.mean.ade\endcsname{0.290}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.mean.obj\endcsname{0.310}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.mean.soc\endcsname{0.269}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.shrink.ade\endcsname{0.273}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.shrink.obj\endcsname{0.286}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.shrink.soc\endcsname{0.259}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.shrink.a\endcsname{0.21}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.delta\endcsname{$-$0.018}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.h500.nseeds\endcsname{3}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.pooled.REALp\endcsname{3}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.pooled.ns\endcsname{6}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.object.REALp\endcsname{1}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.object.ns\endcsname{8}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.social.REALp\endcsname{6}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.social.ns\endcsname{3}
\expandafter\def\csname pn@tp.small.ovdalwaysdino.v.social.REALm\endcsname{0}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.pooled.REALp\endcsname{44}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.pooled.ns\endcsname{4}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.pooled.REALm\endcsname{24}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.pooled.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.object.REALp\endcsname{48}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.object.ns\endcsname{9}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.object.REALm\endcsname{15}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.object.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.social.REALp\endcsname{26}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.social.ns\endcsname{8}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.social.REALm\endcsname{38}
\expandafter\def\csname pn@tp.small.proto.evalpick_row.social.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.sel_row.pooled.REALp\endcsname{42}
\expandafter\def\csname pn@tp.small.proto.sel_row.pooled.ns\endcsname{1}
\expandafter\def\csname pn@tp.small.proto.sel_row.pooled.REALm\endcsname{29}
\expandafter\def\csname pn@tp.small.proto.sel_row.pooled.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.sel_row.object.REALp\endcsname{38}
\expandafter\def\csname pn@tp.small.proto.sel_row.object.ns\endcsname{8}
\expandafter\def\csname pn@tp.small.proto.sel_row.object.REALm\endcsname{26}
\expandafter\def\csname pn@tp.small.proto.sel_row.object.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.sel_row.social.REALp\endcsname{24}
\expandafter\def\csname pn@tp.small.proto.sel_row.social.ns\endcsname{8}
\expandafter\def\csname pn@tp.small.proto.sel_row.social.REALm\endcsname{40}
\expandafter\def\csname pn@tp.small.proto.sel_row.social.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.sel_clip.pooled.REALp\endcsname{22}
\expandafter\def\csname pn@tp.small.proto.sel_clip.pooled.ns\endcsname{42}
\expandafter\def\csname pn@tp.small.proto.sel_clip.pooled.REALm\endcsname{8}
\expandafter\def\csname pn@tp.small.proto.sel_clip.pooled.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.sel_clip.object.REALp\endcsname{30}
\expandafter\def\csname pn@tp.small.proto.sel_clip.object.ns\endcsname{37}
\expandafter\def\csname pn@tp.small.proto.sel_clip.object.REALm\endcsname{5}
\expandafter\def\csname pn@tp.small.proto.sel_clip.object.total\endcsname{72}
\expandafter\def\csname pn@tp.small.proto.sel_clip.social.REALp\endcsname{15}
\expandafter\def\csname pn@tp.small.proto.sel_clip.social.ns\endcsname{27}
\expandafter\def\csname pn@tp.small.proto.sel_clip.social.REALm\endcsname{30}
\expandafter\def\csname pn@tp.small.proto.sel_clip.social.total\endcsname{72}
\expandafter\def\csname pn@tp.small.selected.Transformer\endcsname{128}
\expandafter\def\csname pn@tp.small.selected.GRU\endcsname{37}
\expandafter\def\csname pn@tp.small.selected.ResidualGRU\endcsname{102}
\expandafter\def\csname pn@tp.small.selected.ResidualTransformer\endcsname{93}
\expandafter\def\csname pn@tp.small.selected.total\endcsname{360}
\expandafter\def\csname pn@tp.small.runs\endcsname{72}
\expandafter\def\csname pn@diss.tiny.gt.pooled4\endcsname{0.202}
\expandafter\def\csname pn@diss.tiny.teacher_internvl3_alone.pooled4\endcsname{0.196}
\expandafter\def\csname pn@diss.tiny.teacher_hybrid.pooled4\endcsname{0.235}
\expandafter\def\csname pn@diss.tiny.mtgs.pooled4\endcsname{0.182}
\expandafter\def\csname pn@diss.tiny.gt.pooled3\endcsname{0.211}
\expandafter\def\csname pn@diss.tiny.gt.vat\endcsname{0.216}
\expandafter\def\csname pn@diss.tiny.gt.childplay\endcsname{0.203}
\expandafter\def\csname pn@diss.tiny.gt.vacation\endcsname{0.215}
\expandafter\def\csname pn@diss.tiny.gt.ucolaeo\endcsname{0.179}
\expandafter\def\csname pn@diss.tiny.teacher_hybrid.pooled3\endcsname{0.242}
\expandafter\def\csname pn@diss.tiny.teacher_hybrid.vat\endcsname{0.260}
\expandafter\def\csname pn@diss.tiny.teacher_hybrid.childplay\endcsname{0.234}
\expandafter\def\csname pn@diss.tiny.teacher_hybrid.vacation\endcsname{0.226}
\expandafter\def\csname pn@diss.tiny.teacher_hybrid.ucolaeo\endcsname{0.214}
\expandafter\def\csname pn@diss.tiny.teacher_internvl3_alone.pooled3\endcsname{0.200}
\expandafter\def\csname pn@diss.tiny.teacher_internvl3_alone.vat\endcsname{0.218}
\expandafter\def\csname pn@diss.tiny.teacher_internvl3_alone.childplay\endcsname{0.205}
\expandafter\def\csname pn@diss.tiny.teacher_internvl3_alone.vacation\endcsname{0.162}
\expandafter\def\csname pn@diss.tiny.teacher_internvl3_alone.ucolaeo\endcsname{0.184}
\expandafter\def\csname pn@diss.tiny.mtgs.pooled3\endcsname{0.186}
\expandafter\def\csname pn@diss.tiny.mtgs.vat\endcsname{0.192}
\expandafter\def\csname pn@diss.tiny.mtgs.childplay\endcsname{0.176}
\expandafter\def\csname pn@diss.tiny.mtgs.vacation\endcsname{0.195}
\expandafter\def\csname pn@diss.tiny.mtgs.ucolaeo\endcsname{0.170}
\expandafter\def\csname pn@diss.tiny.teacher_internvl3_alone.tverd\endcsname{12/0/0}
\expandafter\def\csname pn@diss.tiny.teacher_hybrid.tverd\endcsname{12/0/0}
\expandafter\def\csname pn@diss.tiny.mtgs.tverd\endcsname{8/4/0}
\expandafter\def\csname pn@diss.tiny.gt.tverd\endcsname{4/4/4}
\expandafter\def\csname pn@diss.small.gt.pooled4\endcsname{0.189}
\expandafter\def\csname pn@diss.small.teacher_internvl3_alone.pooled4\endcsname{0.181}
\expandafter\def\csname pn@diss.small.teacher_hybrid.pooled4\endcsname{0.213}
\expandafter\def\csname pn@diss.small.mtgs.pooled4\endcsname{0.170}
\expandafter\def\csname pn@diss.small.gt.pooled3\endcsname{0.196}
\expandafter\def\csname pn@diss.small.gt.vat\endcsname{0.212}
\expandafter\def\csname pn@diss.small.gt.childplay\endcsname{0.177}
\expandafter\def\csname pn@diss.small.gt.vacation\endcsname{0.202}
\expandafter\def\csname pn@diss.small.gt.ucolaeo\endcsname{0.167}
\expandafter\def\csname pn@diss.small.teacher_hybrid.pooled3\endcsname{0.226}
\expandafter\def\csname pn@diss.small.teacher_hybrid.vat\endcsname{0.224}
\expandafter\def\csname pn@diss.small.teacher_hybrid.childplay\endcsname{0.230}
\expandafter\def\csname pn@diss.small.teacher_hybrid.vacation\endcsname{0.222}
\expandafter\def\csname pn@diss.small.teacher_hybrid.ucolaeo\endcsname{0.177}
\expandafter\def\csname pn@diss.small.teacher_internvl3_alone.pooled3\endcsname{0.192}
\expandafter\def\csname pn@diss.small.teacher_internvl3_alone.vat\endcsname{0.211}
\expandafter\def\csname pn@diss.small.teacher_internvl3_alone.childplay\endcsname{0.193}
\expandafter\def\csname pn@diss.small.teacher_internvl3_alone.vacation\endcsname{0.159}
\expandafter\def\csname pn@diss.small.teacher_internvl3_alone.ucolaeo\endcsname{0.152}
\expandafter\def\csname pn@diss.small.mtgs.pooled3\endcsname{0.177}
\expandafter\def\csname pn@diss.small.mtgs.vat\endcsname{0.190}
\expandafter\def\csname pn@diss.small.mtgs.childplay\endcsname{0.162}
\expandafter\def\csname pn@diss.small.mtgs.vacation\endcsname{0.182}
\expandafter\def\csname pn@diss.small.mtgs.ucolaeo\endcsname{0.151}
\expandafter\def\csname pn@diss.small.teacher_internvl3_alone.tverd\endcsname{12/0/0}
\expandafter\def\csname pn@diss.small.teacher_hybrid.tverd\endcsname{12/0/0}
\expandafter\def\csname pn@diss.small.mtgs.tverd\endcsname{0/1/11}
\expandafter\def\csname pn@diss.small.gt.tverd\endcsname{6/2/4}
\expandafter\def\csname pn@diss.oldck.tiny.gt.pooled\endcsname{0.211}
\expandafter\def\csname pn@diss.oldck.tiny.gt.childplay\endcsname{0.203}
\expandafter\def\csname pn@diss.oldck.tiny.gt.vacation\endcsname{0.215}
\expandafter\def\csname pn@diss.oldck.tiny.gt.vat\endcsname{0.216}
\expandafter\def\csname pn@diss.oldck.tiny.gt.epoch\endcsname{9}
\expandafter\def\csname pn@diss.oldck.tiny.mtgs.pooled\endcsname{0.203}
\expandafter\def\csname pn@diss.oldck.tiny.mtgs.childplay\endcsname{0.192}
\expandafter\def\csname pn@diss.oldck.tiny.mtgs.vacation\endcsname{0.216}
\expandafter\def\csname pn@diss.oldck.tiny.mtgs.vat\endcsname{0.206}
\expandafter\def\csname pn@diss.oldck.tiny.mtgs.epoch\endcsname{10}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_hybrid.pooled\endcsname{0.248}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_hybrid.childplay\endcsname{0.253}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_hybrid.vacation\endcsname{0.251}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_hybrid.vat\endcsname{0.240}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_hybrid.epoch\endcsname{5}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_internvl3_alone.pooled\endcsname{0.286}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_internvl3_alone.childplay\endcsname{0.345}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_internvl3_alone.vacation\endcsname{0.263}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_internvl3_alone.vat\endcsname{0.241}
\expandafter\def\csname pn@diss.oldck.tiny.teacher_internvl3_alone.epoch\endcsname{12}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.all.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.all.lo\endcsname{$-$0.009}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.all.hi\endcsname{+0.001}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.all.ci\endcsname{[$-$0.009, +0.001]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.all.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vat.diff\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vat.lo\endcsname{$-$0.014}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vat.hi\endcsname{+0.003}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vat.ci\endcsname{[$-$0.014, +0.003]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.childplay.diff\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.childplay.lo\endcsname{$-$0.010}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.childplay.hi\endcsname{+0.005}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.childplay.ci\endcsname{[$-$0.010, +0.005]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vacation.diff\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vacation.lo\endcsname{$-$0.015}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vacation.hi\endcsname{+0.004}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vacation.ci\endcsname{[$-$0.015, +0.004]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.gt.vacation.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.all.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.all.lo\endcsname{$-$0.011}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.all.hi\endcsname{+0.002}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.all.ci\endcsname{[$-$0.011, +0.002]}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vat.diff\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vat.lo\endcsname{$-$0.014}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vat.hi\endcsname{+0.001}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vat.ci\endcsname{[$-$0.014, +0.001]}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.childplay.diff\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.childplay.lo\endcsname{$-$0.014}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.childplay.hi\endcsname{+0.009}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.childplay.ci\endcsname{[$-$0.014, +0.009]}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vacation.diff\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vacation.lo\endcsname{$-$0.019}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vacation.hi\endcsname{+0.007}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vacation.ci\endcsname{[$-$0.019, +0.007]}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.mtgs.vs.gt.vacation.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.all.diff\endcsname{0.000}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.all.lo\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.all.hi\endcsname{+0.005}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.all.ci\endcsname{[$-$0.005, +0.005]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vat.diff\endcsname{0.000}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vat.lo\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vat.hi\endcsname{+0.008}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vat.ci\endcsname{[$-$0.007, +0.008]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.childplay.diff\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.childplay.lo\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.childplay.hi\endcsname{+0.009}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.childplay.ci\endcsname{[$-$0.007, +0.009]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vacation.diff\endcsname{+0.001}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vacation.lo\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vacation.hi\endcsname{+0.008}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vacation.ci\endcsname{[$-$0.008, +0.008]}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.gazelle.vs.mtgs.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.all.diff\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.all.lo\endcsname{$-$0.009}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.all.hi\endcsname{$-$0.003}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.all.ci\endcsname{[$-$0.009, $-$0.003]}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.all.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vat.diff\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vat.lo\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vat.hi\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vat.ci\endcsname{[$-$0.013, $-$0.001]}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.childplay.diff\endcsname{$-$0.009}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.childplay.lo\endcsname{$-$0.012}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.childplay.hi\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.childplay.ci\endcsname{[$-$0.012, $-$0.004]}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.childplay.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vacation.diff\endcsname{+0.001}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vacation.lo\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vacation.hi\endcsname{+0.005}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vacation.ci\endcsname{[$-$0.005, +0.005]}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.ovdmixrand.vs.ovdgate55.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.all.diff\endcsname{$-$0.002}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.all.lo\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.all.hi\endcsname{+0.002}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.all.ci\endcsname{[$-$0.006, +0.002]}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vat.diff\endcsname{+0.004}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vat.lo\endcsname{$-$0.003}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vat.hi\endcsname{+0.010}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vat.ci\endcsname{[$-$0.003, +0.010]}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.childplay.diff\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.childplay.lo\endcsname{$-$0.012}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.childplay.hi\endcsname{+0.002}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.childplay.ci\endcsname{[$-$0.012, +0.002]}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vacation.diff\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vacation.lo\endcsname{$-$0.015}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vacation.hi\endcsname{+0.001}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vacation.ci\endcsname{[$-$0.015, +0.001]}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.teacher_internvl3_alone.vs.copyb.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.all.diff\endcsname{+0.125}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.all.lo\endcsname{+0.092}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.all.hi\endcsname{+0.162}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.all.ci\endcsname{[+0.092, +0.162]}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.all.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.all.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vat.diff\endcsname{+0.106}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vat.lo\endcsname{+0.080}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vat.hi\endcsname{+0.133}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vat.ci\endcsname{[+0.080, +0.133]}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vat.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.childplay.diff\endcsname{+0.152}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.childplay.lo\endcsname{+0.079}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.childplay.hi\endcsname{+0.214}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.childplay.ci\endcsname{[+0.079, +0.214]}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.childplay.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.childplay.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vacation.diff\endcsname{+0.109}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vacation.lo\endcsname{+0.077}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vacation.hi\endcsname{+0.151}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vacation.ci\endcsname{[+0.077, +0.151]}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vacation.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.vlmnoleak.vs.gt.vacation.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.all.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.all.lo\endcsname{$-$0.009}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.all.hi\endcsname{0.000}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.all.ci\endcsname{[$-$0.009, +0.000]}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vat.diff\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vat.lo\endcsname{$-$0.010}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vat.hi\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vat.ci\endcsname{[$-$0.010, $-$0.001]}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vat.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.childplay.diff\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.childplay.lo\endcsname{$-$0.014}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.childplay.hi\endcsname{+0.003}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.childplay.ci\endcsname{[$-$0.014, +0.003]}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vacation.diff\endcsname{+0.003}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vacation.lo\endcsname{$-$0.002}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vacation.hi\endcsname{+0.007}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vacation.ci\endcsname{[$-$0.002, +0.007]}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.ovdmix40.vs.ovdgate40.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.all.diff\endcsname{+0.001}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.all.lo\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.all.hi\endcsname{+0.009}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.all.ci\endcsname{[$-$0.008, +0.009]}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vat.diff\endcsname{+0.010}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vat.lo\endcsname{+0.003}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vat.hi\endcsname{+0.016}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vat.ci\endcsname{[+0.003, +0.016]}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.childplay.diff\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.childplay.lo\endcsname{$-$0.026}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.childplay.hi\endcsname{+0.002}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.childplay.ci\endcsname{[$-$0.026, +0.002]}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.childplay.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vacation.diff\endcsname{+0.010}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vacation.lo\endcsname{+0.004}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vacation.hi\endcsname{+0.016}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vacation.ci\endcsname{[+0.004, +0.016]}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vacation.sig\endcsname{significant}
\expandafter\def\csname pn@sig.tiny.ovdmix48.vs.ovdgate48.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.all.diff\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.all.lo\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.all.hi\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.all.ci\endcsname{[$-$0.013, $-$0.004]}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.all.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.all.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vat.diff\endcsname{$-$0.011}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vat.lo\endcsname{$-$0.018}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vat.hi\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vat.ci\endcsname{[$-$0.018, $-$0.004]}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.childplay.diff\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.childplay.lo\endcsname{$-$0.012}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.childplay.hi\endcsname{+0.004}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.childplay.ci\endcsname{[$-$0.012, +0.004]}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vacation.diff\endcsname{$-$0.009}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vacation.lo\endcsname{$-$0.018}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vacation.hi\endcsname{+0.001}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vacation.ci\endcsname{[$-$0.018, +0.001]}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.gt.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.all.diff\endcsname{$-$0.010}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.all.lo\endcsname{$-$0.015}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.all.hi\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.all.ci\endcsname{[$-$0.015, $-$0.005]}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.all.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.all.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vat.diff\endcsname{$-$0.016}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vat.lo\endcsname{$-$0.024}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vat.hi\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vat.ci\endcsname{[$-$0.024, $-$0.007]}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vat.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.childplay.diff\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.childplay.lo\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.childplay.hi\endcsname{0.000}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.childplay.ci\endcsname{[$-$0.013, +0.000]}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vacation.diff\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vacation.lo\endcsname{$-$0.020}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vacation.hi\endcsname{+0.005}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vacation.ci\endcsname{[$-$0.020, +0.005]}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.mtgs.vs.gt.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.all.diff\endcsname{+0.002}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.all.lo\endcsname{$-$0.003}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.all.hi\endcsname{+0.007}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.all.ci\endcsname{[$-$0.003, +0.007]}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vat.diff\endcsname{+0.005}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vat.lo\endcsname{$-$0.003}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vat.hi\endcsname{+0.012}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vat.ci\endcsname{[$-$0.003, +0.012]}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.childplay.diff\endcsname{+0.001}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.childplay.lo\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.childplay.hi\endcsname{+0.010}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.childplay.ci\endcsname{[$-$0.006, +0.010]}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vacation.diff\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vacation.lo\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vacation.hi\endcsname{+0.010}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vacation.ci\endcsname{[$-$0.013, +0.010]}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.gazelle.vs.mtgs.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.all.diff\endcsname{+0.001}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.all.lo\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.all.hi\endcsname{+0.009}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.all.ci\endcsname{[$-$0.007, +0.009]}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vat.diff\endcsname{+0.012}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vat.lo\endcsname{+0.006}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vat.hi\endcsname{+0.018}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vat.ci\endcsname{[+0.006, +0.018]}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.childplay.diff\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.childplay.lo\endcsname{$-$0.023}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.childplay.hi\endcsname{0.000}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.childplay.ci\endcsname{[$-$0.023, +0.000]}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vacation.diff\endcsname{+0.007}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vacation.lo\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vacation.hi\endcsname{+0.023}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vacation.ci\endcsname{[$-$0.007, +0.023]}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.ovdmixrand.vs.ovdgate55.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.all.diff\endcsname{+0.002}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.all.lo\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.all.hi\endcsname{+0.008}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.all.ci\endcsname{[$-$0.006, +0.008]}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vat.diff\endcsname{+0.007}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vat.lo\endcsname{$-$0.002}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vat.hi\endcsname{+0.017}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vat.ci\endcsname{[$-$0.002, +0.017]}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vat.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.childplay.diff\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.childplay.lo\endcsname{$-$0.025}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.childplay.hi\endcsname{+0.008}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.childplay.ci\endcsname{[$-$0.025, +0.008]}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vacation.diff\endcsname{+0.003}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vacation.lo\endcsname{$-$0.003}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vacation.hi\endcsname{+0.009}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vacation.ci\endcsname{[$-$0.003, +0.009]}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.teacher_internvl3_alone.vs.copyb.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.all.diff\endcsname{+0.135}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.all.lo\endcsname{+0.110}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.all.hi\endcsname{+0.160}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.all.ci\endcsname{[+0.110, +0.160]}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.all.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.all.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vat.diff\endcsname{+0.123}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vat.lo\endcsname{+0.099}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vat.hi\endcsname{+0.146}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vat.ci\endcsname{[+0.099, +0.146]}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vat.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.childplay.diff\endcsname{+0.146}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.childplay.lo\endcsname{+0.088}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.childplay.hi\endcsname{+0.189}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.childplay.ci\endcsname{[+0.088, +0.189]}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.childplay.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.childplay.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vacation.diff\endcsname{+0.136}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vacation.lo\endcsname{+0.102}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vacation.hi\endcsname{+0.178}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vacation.ci\endcsname{[+0.102, +0.178]}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vacation.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.vlmnoleak.vs.gt.vacation.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.all.diff\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.all.lo\endcsname{$-$0.010}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.all.hi\endcsname{$-$0.002}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.all.ci\endcsname{[$-$0.010, $-$0.002]}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.all.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vat.diff\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vat.lo\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vat.hi\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vat.ci\endcsname{[$-$0.013, $-$0.001]}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.childplay.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.childplay.lo\endcsname{$-$0.010}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.childplay.hi\endcsname{+0.005}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.childplay.ci\endcsname{[$-$0.010, +0.005]}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vacation.diff\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vacation.lo\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vacation.hi\endcsname{$-$0.002}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vacation.ci\endcsname{[$-$0.013, $-$0.002]}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vacation.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.ovdmix40.vs.ovdgate40.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.all.diff\endcsname{$-$0.001}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.all.lo\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.all.hi\endcsname{+0.004}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.all.ci\endcsname{[$-$0.005, +0.004]}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vat.diff\endcsname{0.000}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vat.lo\endcsname{$-$0.006}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vat.hi\endcsname{+0.006}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vat.ci\endcsname{[$-$0.006, +0.006]}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.childplay.diff\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.childplay.lo\endcsname{$-$0.012}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.childplay.hi\endcsname{$-$0.002}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.childplay.ci\endcsname{[$-$0.012, $-$0.002]}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.childplay.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vacation.diff\endcsname{+0.009}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vacation.lo\endcsname{+0.001}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vacation.hi\endcsname{+0.018}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vacation.ci\endcsname{[+0.001, +0.018]}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vacation.sig\endcsname{significant}
\expandafter\def\csname pn@sig.small.ovdmix48.vs.ovdgate48.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.all.diff\endcsname{$-$0.005}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.all.lo\endcsname{$-$0.011}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.all.hi\endcsname{+0.001}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.all.ci\endcsname{[$-$0.011, +0.001]}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vat.diff\endcsname{$-$0.009}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vat.lo\endcsname{$-$0.017}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vat.hi\endcsname{$-$0.003}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vat.ci\endcsname{[$-$0.017, $-$0.003]}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vat.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.childplay.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.childplay.lo\endcsname{$-$0.014}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.childplay.hi\endcsname{+0.011}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.childplay.ci\endcsname{[$-$0.014, +0.011]}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vacation.diff\endcsname{$-$0.002}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vacation.lo\endcsname{$-$0.012}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vacation.hi\endcsname{+0.009}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vacation.ci\endcsname{[$-$0.012, +0.009]}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headpos_tiny.gazelle.vs.gt.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.all.diff\endcsname{+0.134}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.all.lo\endcsname{+0.106}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.all.hi\endcsname{+0.162}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.all.ci\endcsname{[+0.106, +0.162]}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.all.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.all.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vat.diff\endcsname{+0.129}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vat.lo\endcsname{+0.101}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vat.hi\endcsname{+0.158}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vat.ci\endcsname{[+0.101, +0.158]}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vat.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vat.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.childplay.diff\endcsname{+0.137}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.childplay.lo\endcsname{+0.073}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.childplay.hi\endcsname{+0.187}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.childplay.ci\endcsname{[+0.073, +0.187]}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.childplay.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.childplay.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vacation.diff\endcsname{+0.137}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vacation.lo\endcsname{+0.099}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vacation.hi\endcsname{+0.183}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vacation.ci\endcsname{[+0.099, +0.183]}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vacation.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headpos_tiny.vlmnoleak.vs.gt.vacation.seedpairs.same\endcsname{all nine}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.all.diff\endcsname{$-$0.003}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.all.clips\endcsname{172}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.all.lo\endcsname{$-$0.008}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.all.hi\endcsname{+0.001}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.all.ci\endcsname{[$-$0.008, +0.001]}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.all.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.all.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vat.diff\endcsname{$-$0.007}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vat.clips\endcsname{91}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vat.lo\endcsname{$-$0.014}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vat.hi\endcsname{0.000}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vat.ci\endcsname{[$-$0.014, +0.000]}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vat.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vat.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.childplay.diff\endcsname{+0.001}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.childplay.clips\endcsname{43}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.childplay.lo\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.childplay.hi\endcsname{+0.006}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.childplay.ci\endcsname{[$-$0.004, +0.006]}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.childplay.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.childplay.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vacation.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vacation.clips\endcsname{38}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vacation.lo\endcsname{$-$0.013}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vacation.hi\endcsname{+0.006}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vacation.ci\endcsname{[$-$0.013, +0.006]}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vacation.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headpos_small.gazelle.vs.gt.vacation.seedpairs.same\endcsname{not all}
\expandafter\def\csname pn@sig.headposgain.tiny.gt.diff\endcsname{$-$0.009}
\expandafter\def\csname pn@sig.headposgain.tiny.gt.ci\endcsname{[$-$0.016, $-$0.002]}
\expandafter\def\csname pn@sig.headposgain.tiny.gt.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headposgain.tiny.gazelle.diff\endcsname{$-$0.010}
\expandafter\def\csname pn@sig.headposgain.tiny.gazelle.ci\endcsname{[$-$0.015, $-$0.005]}
\expandafter\def\csname pn@sig.headposgain.tiny.gazelle.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headposgain.tiny.vlmnoleak.diff\endcsname{0.000}
\expandafter\def\csname pn@sig.headposgain.tiny.vlmnoleak.ci\endcsname{[$-$0.007, +0.008]}
\expandafter\def\csname pn@sig.headposgain.tiny.vlmnoleak.sig\endcsname{not significant}
\expandafter\def\csname pn@sig.headposgain.small.gt.diff\endcsname{$-$0.010}
\expandafter\def\csname pn@sig.headposgain.small.gt.ci\endcsname{[$-$0.014, $-$0.004]}
\expandafter\def\csname pn@sig.headposgain.small.gt.sig\endcsname{significant}
\expandafter\def\csname pn@sig.headposgain.small.gazelle.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@sig.headposgain.small.gazelle.ci\endcsname{[$-$0.008, $-$0.001]}
\expandafter\def\csname pn@sig.headposgain.small.gazelle.sig\endcsname{significant}
\expandafter\def\csname pn@cost.student_tiny.params\endcsname{5.7}
\expandafter\def\csname pn@cost.student_tiny.gflops\endcsname{5.0}
\expandafter\def\csname pn@cost.student_tiny.gpu_ms\endcsname{12.1}
\expandafter\def\csname pn@cost.student_tiny.cpu4_ms\endcsname{34}
\expandafter\def\csname pn@cost.student_tiny.cpu1_ms\endcsname{68}
\expandafter\def\csname pn@cost.student_tiny.cpu4_fps\endcsname{29.4}
\expandafter\def\csname pn@cost.student_tiny.gpu_fps\endcsname{83}
\expandafter\def\csname pn@cost.student_tiny.gpu_mem\endcsname{31}
\expandafter\def\csname pn@cost.student_small.params\endcsname{21.9}
\expandafter\def\csname pn@cost.student_small.gflops\endcsname{18.4}
\expandafter\def\csname pn@cost.student_small.gpu_ms\endcsname{12.4}
\expandafter\def\csname pn@cost.student_small.cpu4_ms\endcsname{98}
\expandafter\def\csname pn@cost.student_small.cpu1_ms\endcsname{219}
\expandafter\def\csname pn@cost.student_small.cpu4_fps\endcsname{10.2}
\expandafter\def\csname pn@cost.student_small.gpu_fps\endcsname{81}
\expandafter\def\csname pn@cost.student_small.gpu_mem\endcsname{93}
\expandafter\def\csname pn@cost.gazelle_vitb14.params\endcsname{89.4}
\expandafter\def\csname pn@cost.gazelle_vitb14.gflops\endcsname{222.8}
\expandafter\def\csname pn@cost.gazelle_vitb14.gpu_ms\endcsname{62.7}
\expandafter\def\csname pn@cost.gazelle_vitb14.cpu4_ms\endcsname{1{,}077}
\expandafter\def\csname pn@cost.gazelle_vitb14.cpu1_ms\endcsname{2{,}552}
\expandafter\def\csname pn@cost.gazelle_vitb14.cpu4_fps\endcsname{0.9}
\expandafter\def\csname pn@cost.gazelle_vitb14.gpu_fps\endcsname{16}
\expandafter\def\csname pn@cost.gazelle_vitb14.gpu_mem\endcsname{1{,}993}
\expandafter\def\csname pn@cost.gazelle_vitb14.decoder_params\endcsname{2.8}
\expandafter\def\csname pn@cost.gazelle_vitl14.params\endcsname{307.3}
\expandafter\def\csname pn@cost.gazelle_vitl14.gflops\endcsname{732.7}
\expandafter\def\csname pn@cost.gazelle_vitl14.gpu_ms\endcsname{190.9}
\expandafter\def\csname pn@cost.gazelle_vitl14.cpu4_ms\endcsname{4{,}299}
\expandafter\def\csname pn@cost.gazelle_vitl14.cpu1_ms\endcsname{9{,}160}
\expandafter\def\csname pn@cost.gazelle_vitl14.cpu4_fps\endcsname{0.2}
\expandafter\def\csname pn@cost.gazelle_vitl14.gpu_fps\endcsname{5}
\expandafter\def\csname pn@cost.gazelle_vitl14.gpu_mem\endcsname{3{,}371}
\expandafter\def\csname pn@cost.gazelle_vitl14.decoder_params\endcsname{2.9}
\expandafter\def\csname pn@cost.student_small.flops_x_tiny\endcsname{4}
\expandafter\def\csname pn@cost.student_small.cpu4_x_tiny\endcsname{3}
\expandafter\def\csname pn@cost.student_small.gpu_x_tiny\endcsname{1.0}
\expandafter\def\csname pn@cost.gazelle_vitb14.flops_x_tiny\endcsname{44}
\expandafter\def\csname pn@cost.gazelle_vitb14.cpu4_x_tiny\endcsname{32}
\expandafter\def\csname pn@cost.gazelle_vitb14.gpu_x_tiny\endcsname{5.2}
\expandafter\def\csname pn@cost.gazelle_vitl14.flops_x_tiny\endcsname{146}
\expandafter\def\csname pn@cost.gazelle_vitl14.cpu4_x_tiny\endcsname{127}
\expandafter\def\csname pn@cost.gazelle_vitl14.gpu_x_tiny\endcsname{15.8}
\expandafter\def\csname pn@cost.cpu\endcsname{Ryzen 5 5600H}
\expandafter\def\csname pn@cost.gpu\endcsname{RTX 3060 Laptop}
\expandafter\def\csname pn@svlm.rows\endcsname{19{,}563}
\expandafter\def\csname pn@svlm.internvl3_leaky.all\endcsname{0.276}
\expandafter\def\csname pn@svlm.internvl3_leaky.social\endcsname{0.202}
\expandafter\def\csname pn@svlm.internvl3_leaky.object\endcsname{0.390}
\expandafter\def\csname pn@svlm.internvl3_leaky.pck10\endcsname{0.350}
\expandafter\def\csname pn@svlm.internvl3_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.internvl3_leaky.gtshare\endcsname{6.0\%}
\expandafter\def\csname pn@svlm.internvl3_leaky.copy\endcsname{96.8\%}
\expandafter\def\csname pn@svlm.internvl3_leaky.copy.social\endcsname{96.4\%}
\expandafter\def\csname pn@svlm.internvl3_leaky.copy.object\endcsname{97.6\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.all\endcsname{0.268}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.social\endcsname{0.198}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.object\endcsname{0.375}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.pck10\endcsname{0.370}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.gtshare\endcsname{6.0\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.copy\endcsname{97.4\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.copy.social\endcsname{99.3\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_leaky.copy.object\endcsname{94.1\%}
\expandafter\def\csname pn@svlm.copyb.all\endcsname{0.273}
\expandafter\def\csname pn@svlm.copyb.social\endcsname{0.195}
\expandafter\def\csname pn@svlm.copyb.object\endcsname{0.391}
\expandafter\def\csname pn@svlm.copyb.pck10\endcsname{0.367}
\expandafter\def\csname pn@svlm.copyb.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.copyb.gtshare\endcsname{6.0\%}
\expandafter\def\csname pn@svlm.internvl3_noleak.all\endcsname{0.335}
\expandafter\def\csname pn@svlm.internvl3_noleak.social\endcsname{0.332}
\expandafter\def\csname pn@svlm.internvl3_noleak.object\endcsname{0.340}
\expandafter\def\csname pn@svlm.internvl3_noleak.pck10\endcsname{0.051}
\expandafter\def\csname pn@svlm.internvl3_noleak.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.internvl3_noleak.gtshare\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.internvl3_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.internvl3_noleak.copy.social\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.internvl3_noleak.copy.object\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.all\endcsname{0.266}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.social\endcsname{0.239}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.object\endcsname{0.307}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.pck10\endcsname{0.203}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.offclaims\endcsname{106}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.gtshare\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.copy.social\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.qwen3vl8b_noleak.copy.object\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.boot.leaky.diff\endcsname{$-$0.009}
\expandafter\def\csname pn@svlm.boot.leaky.ci\endcsname{[$-$0.017, $-$0.002]}
\expandafter\def\csname pn@svlm.boot.leaky.sig\endcsname{significant}
\expandafter\def\csname pn@svlm.boot.noleak.diff\endcsname{$-$0.068}
\expandafter\def\csname pn@svlm.boot.noleak.ci\endcsname{[$-$0.093, $-$0.046]}
\expandafter\def\csname pn@svlm.boot.noleak.sig\endcsname{significant}
\expandafter\def\csname pn@svlm.childplay.rows\endcsname{20{,}100}
\expandafter\def\csname pn@svlm.childplay.internvl3_leaky.all\endcsname{0.325}
\expandafter\def\csname pn@svlm.childplay.internvl3_leaky.social\endcsname{0.135}
\expandafter\def\csname pn@svlm.childplay.internvl3_leaky.object\endcsname{0.391}
\expandafter\def\csname pn@svlm.childplay.internvl3_leaky.pck10\endcsname{0.208}
\expandafter\def\csname pn@svlm.childplay.internvl3_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.childplay.internvl3_leaky.copy\endcsname{89.8\%}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_leaky.all\endcsname{0.244}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_leaky.social\endcsname{0.135}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_leaky.object\endcsname{0.282}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_leaky.pck10\endcsname{0.294}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_leaky.copy\endcsname{60.5\%}
\expandafter\def\csname pn@svlm.childplay.copyb.all\endcsname{0.319}
\expandafter\def\csname pn@svlm.childplay.copyb.social\endcsname{0.114}
\expandafter\def\csname pn@svlm.childplay.copyb.object\endcsname{0.391}
\expandafter\def\csname pn@svlm.childplay.copyb.pck10\endcsname{0.222}
\expandafter\def\csname pn@svlm.childplay.copyb.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.childplay.internvl3_noleak.all\endcsname{0.323}
\expandafter\def\csname pn@svlm.childplay.internvl3_noleak.social\endcsname{0.293}
\expandafter\def\csname pn@svlm.childplay.internvl3_noleak.object\endcsname{0.334}
\expandafter\def\csname pn@svlm.childplay.internvl3_noleak.pck10\endcsname{0.060}
\expandafter\def\csname pn@svlm.childplay.internvl3_noleak.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.childplay.internvl3_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_noleak.all\endcsname{0.205}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_noleak.social\endcsname{0.154}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_noleak.object\endcsname{0.223}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_noleak.pck10\endcsname{0.297}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_noleak.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.childplay.qwen3vl8b_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.childplay.boot.leaky.diff\endcsname{$-$0.081}
\expandafter\def\csname pn@svlm.childplay.boot.leaky.ci\endcsname{[$-$0.136, $-$0.044]}
\expandafter\def\csname pn@svlm.childplay.boot.leaky.sig\endcsname{significant}
\expandafter\def\csname pn@svlm.childplay.boot.noleak.diff\endcsname{$-$0.118}
\expandafter\def\csname pn@svlm.childplay.boot.noleak.ci\endcsname{[$-$0.141, $-$0.081]}
\expandafter\def\csname pn@svlm.childplay.boot.noleak.sig\endcsname{significant}
\expandafter\def\csname pn@svlm.vacation.rows\endcsname{11{,}928}
\expandafter\def\csname pn@svlm.vacation.internvl3_leaky.all\endcsname{0.237}
\expandafter\def\csname pn@svlm.vacation.internvl3_leaky.social\endcsname{0.069}
\expandafter\def\csname pn@svlm.vacation.internvl3_leaky.object\endcsname{0.458}
\expandafter\def\csname pn@svlm.vacation.internvl3_leaky.pck10\endcsname{0.499}
\expandafter\def\csname pn@svlm.vacation.internvl3_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.vacation.internvl3_leaky.copy\endcsname{94.3\%}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_leaky.all\endcsname{0.226}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_leaky.social\endcsname{0.069}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_leaky.object\endcsname{0.434}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_leaky.pck10\endcsname{0.533}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_leaky.copy\endcsname{90.7\%}
\expandafter\def\csname pn@svlm.vacation.copyb.all\endcsname{0.244}
\expandafter\def\csname pn@svlm.vacation.copyb.social\endcsname{0.058}
\expandafter\def\csname pn@svlm.vacation.copyb.object\endcsname{0.491}
\expandafter\def\csname pn@svlm.vacation.copyb.pck10\endcsname{0.484}
\expandafter\def\csname pn@svlm.vacation.copyb.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.vacation.internvl3_noleak.all\endcsname{0.351}
\expandafter\def\csname pn@svlm.vacation.internvl3_noleak.social\endcsname{0.338}
\expandafter\def\csname pn@svlm.vacation.internvl3_noleak.object\endcsname{0.369}
\expandafter\def\csname pn@svlm.vacation.internvl3_noleak.pck10\endcsname{0.063}
\expandafter\def\csname pn@svlm.vacation.internvl3_noleak.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.vacation.internvl3_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_noleak.all\endcsname{0.285}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_noleak.social\endcsname{0.259}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_noleak.object\endcsname{0.320}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_noleak.pck10\endcsname{0.198}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_noleak.offclaims\endcsname{2}
\expandafter\def\csname pn@svlm.vacation.qwen3vl8b_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.vacation.boot.leaky.diff\endcsname{$-$0.010}
\expandafter\def\csname pn@svlm.vacation.boot.leaky.ci\endcsname{[$-$0.025, +0.005]}
\expandafter\def\csname pn@svlm.vacation.boot.leaky.sig\endcsname{not significant}
\expandafter\def\csname pn@svlm.vacation.boot.noleak.diff\endcsname{$-$0.066}
\expandafter\def\csname pn@svlm.vacation.boot.noleak.ci\endcsname{[$-$0.094, $-$0.039]}
\expandafter\def\csname pn@svlm.vacation.boot.noleak.sig\endcsname{significant}
\expandafter\def\csname pn@svlm.pooled.rows\endcsname{51{,}591}
\expandafter\def\csname pn@svlm.pooled.internvl3_leaky.all\endcsname{0.286}
\expandafter\def\csname pn@svlm.pooled.internvl3_leaky.social\endcsname{0.149}
\expandafter\def\csname pn@svlm.pooled.internvl3_leaky.object\endcsname{0.403}
\expandafter\def\csname pn@svlm.pooled.internvl3_leaky.pck10\endcsname{0.329}
\expandafter\def\csname pn@svlm.pooled.internvl3_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.pooled.internvl3_leaky.copy\endcsname{93.4\%}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_leaky.all\endcsname{0.249}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_leaky.social\endcsname{0.147}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_leaky.object\endcsname{0.336}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_leaky.pck10\endcsname{0.378}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_leaky.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_leaky.copy\endcsname{81.1\%}
\expandafter\def\csname pn@svlm.pooled.copyb.all\endcsname{0.284}
\expandafter\def\csname pn@svlm.pooled.copyb.social\endcsname{0.138}
\expandafter\def\csname pn@svlm.pooled.copyb.object\endcsname{0.409}
\expandafter\def\csname pn@svlm.pooled.copyb.pck10\endcsname{0.337}
\expandafter\def\csname pn@svlm.pooled.copyb.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.pooled.internvl3_noleak.all\endcsname{0.334}
\expandafter\def\csname pn@svlm.pooled.internvl3_noleak.social\endcsname{0.325}
\expandafter\def\csname pn@svlm.pooled.internvl3_noleak.object\endcsname{0.342}
\expandafter\def\csname pn@svlm.pooled.internvl3_noleak.pck10\endcsname{0.057}
\expandafter\def\csname pn@svlm.pooled.internvl3_noleak.offclaims\endcsname{0}
\expandafter\def\csname pn@svlm.pooled.internvl3_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_noleak.all\endcsname{0.247}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_noleak.social\endcsname{0.226}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_noleak.object\endcsname{0.264}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_noleak.pck10\endcsname{0.238}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_noleak.offclaims\endcsname{108}
\expandafter\def\csname pn@svlm.pooled.qwen3vl8b_noleak.copy\endcsname{0.0\%}
\expandafter\def\csname pn@svlm.pooled.boot.leaky.diff\endcsname{$-$0.037}
\expandafter\def\csname pn@svlm.pooled.boot.leaky.ci\endcsname{[$-$0.060, $-$0.020]}
\expandafter\def\csname pn@svlm.pooled.boot.leaky.sig\endcsname{significant}
\expandafter\def\csname pn@svlm.pooled.boot.noleak.diff\endcsname{$-$0.087}
\expandafter\def\csname pn@svlm.pooled.boot.noleak.ci\endcsname{[$-$0.107, $-$0.067]}
\expandafter\def\csname pn@svlm.pooled.boot.noleak.sig\endcsname{significant}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.n\endcsname{882}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.share\endcsname{8\%}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.head\endcsname{0.264}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vscopy.diff\endcsname{$-$0.008}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vscopy.ci\endcsname{[$-$0.012, $-$0.004]}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vscopy.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vsshrink.diff\endcsname{$-$0.003}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vsshrink.ci\endcsname{[$-$0.007, +0.000]}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vsshrink.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vsctx1.diff\endcsname{0.000}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vsctx1.ci\endcsname{[$-$0.001, +0.002]}
\expandafter\def\csname pn@shift.tiny.gt.h300.shift.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.n\endcsname{10{,}345}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.share\endcsname{90\%}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.head\endcsname{0.205}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vscopy.diff\endcsname{+0.003}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vscopy.ci\endcsname{[$-$0.001, +0.006]}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vscopy.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vsshrink.diff\endcsname{+0.003}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vsshrink.ci\endcsname{[+0.000, +0.006]}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vsshrink.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vsctx1.diff\endcsname{0.000}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vsctx1.ci\endcsname{[$-$0.001, +0.001]}
\expandafter\def\csname pn@shift.tiny.gt.h300.stay.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.n\endcsname{1{,}276}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.share\endcsname{12\%}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.head\endcsname{0.266}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vscopy.diff\endcsname{$-$0.010}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vscopy.ci\endcsname{[$-$0.014, $-$0.005]}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vscopy.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vsshrink.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vsshrink.ci\endcsname{[$-$0.008, $-$0.000]}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vsshrink.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vsctx1.diff\endcsname{+0.001}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vsctx1.ci\endcsname{[$-$0.001, +0.002]}
\expandafter\def\csname pn@shift.tiny.gt.h500.shift.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.n\endcsname{9{,}113}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.share\endcsname{85\%}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.head\endcsname{0.205}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vscopy.diff\endcsname{+0.003}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vscopy.ci\endcsname{[$-$0.001, +0.007]}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vscopy.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vsshrink.diff\endcsname{+0.003}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vsshrink.ci\endcsname{[+0.000, +0.007]}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vsshrink.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vsctx1.diff\endcsname{0.000}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vsctx1.ci\endcsname{[$-$0.001, +0.001]}
\expandafter\def\csname pn@shift.tiny.gt.h500.stay.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.n\endcsname{882}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.share\endcsname{8\%}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.head\endcsname{0.261}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vscopy.diff\endcsname{$-$0.009}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vscopy.ci\endcsname{[$-$0.013, $-$0.005]}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vscopy.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vsshrink.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vsshrink.ci\endcsname{[$-$0.007, $-$0.000]}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vsshrink.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vsctx1.diff\endcsname{+0.002}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vsctx1.ci\endcsname{[+0.000, +0.003]}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.shift.vsctx1.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.n\endcsname{10{,}345}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.share\endcsname{90\%}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.head\endcsname{0.201}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vscopy.diff\endcsname{+0.002}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vscopy.ci\endcsname{[$-$0.002, +0.006]}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vscopy.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vsshrink.diff\endcsname{+0.002}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vsshrink.ci\endcsname{[$-$0.001, +0.006]}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vsshrink.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vsctx1.diff\endcsname{0.000}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vsctx1.ci\endcsname{[$-$0.001, +0.001]}
\expandafter\def\csname pn@shift.tiny.mtgs.h300.stay.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.n\endcsname{1{,}276}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.share\endcsname{12\%}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.head\endcsname{0.267}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vscopy.diff\endcsname{$-$0.011}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vscopy.ci\endcsname{[$-$0.014, $-$0.007]}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vscopy.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vsshrink.diff\endcsname{$-$0.004}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vsshrink.ci\endcsname{[$-$0.007, $-$0.002]}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vsshrink.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vsctx1.diff\endcsname{+0.001}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vsctx1.ci\endcsname{[$-$0.000, +0.002]}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.shift.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.n\endcsname{9{,}113}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.share\endcsname{85\%}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.head\endcsname{0.200}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vscopy.diff\endcsname{+0.002}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vscopy.ci\endcsname{[$-$0.002, +0.006]}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vscopy.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vsshrink.diff\endcsname{+0.002}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vsshrink.ci\endcsname{[$-$0.000, +0.006]}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vsshrink.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vsctx1.diff\endcsname{0.000}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vsctx1.ci\endcsname{[$-$0.002, +0.001]}
\expandafter\def\csname pn@shift.tiny.mtgs.h500.stay.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.n\endcsname{882}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.share\endcsname{8\%}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.head\endcsname{0.257}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vscopy.diff\endcsname{$-$0.007}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vscopy.ci\endcsname{[$-$0.010, $-$0.004]}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vscopy.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vsshrink.diff\endcsname{$-$0.005}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vsshrink.ci\endcsname{[$-$0.008, $-$0.002]}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vsshrink.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vsctx1.diff\endcsname{+0.001}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vsctx1.ci\endcsname{[$-$0.001, +0.003]}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.shift.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.n\endcsname{10{,}345}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.share\endcsname{90\%}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.head\endcsname{0.202}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vscopy.diff\endcsname{+0.004}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vscopy.ci\endcsname{[$-$0.001, +0.010]}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vscopy.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vsshrink.diff\endcsname{+0.004}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vsshrink.ci\endcsname{[$-$0.000, +0.008]}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vsshrink.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vsctx1.diff\endcsname{$-$0.001}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vsctx1.ci\endcsname{[$-$0.002, +0.001]}
\expandafter\def\csname pn@shift.tiny.gazelle.h300.stay.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.n\endcsname{1{,}276}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.share\endcsname{12\%}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.head\endcsname{0.262}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vscopy.diff\endcsname{$-$0.010}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vscopy.ci\endcsname{[$-$0.013, $-$0.006]}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vscopy.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vsshrink.diff\endcsname{$-$0.007}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vsshrink.ci\endcsname{[$-$0.010, $-$0.003]}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vsshrink.sig\endcsname{sig.}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vsctx1.diff\endcsname{+0.001}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vsctx1.ci\endcsname{[$-$0.001, +0.002]}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.shift.vsctx1.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.n\endcsname{9{,}113}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.share\endcsname{85\%}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.head\endcsname{0.201}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vscopy.diff\endcsname{+0.005}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vscopy.ci\endcsname{[$-$0.002, +0.012]}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vscopy.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vsshrink.diff\endcsname{+0.004}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vsshrink.ci\endcsname{[$-$0.001, +0.010]}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vsshrink.sig\endcsname{n.s.}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vsctx1.diff\endcsname{$-$0.001}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vsctx1.ci\endcsname{[$-$0.002, $-$0.000]}
\expandafter\def\csname pn@shift.tiny.gazelle.h500.stay.vsctx1.sig\endcsname{sig.}
\expandafter\def\csname pn@uco.rows\endcsname{18{,}726}
\expandafter\def\csname pn@uco.lab.vlmleak_old\endcsname{0.030}
\expandafter\def\csname pn@uco.lab.mtgs\endcsname{0.031}
\expandafter\def\csname pn@uco.lab.gazelle\endcsname{0.059}
\expandafter\def\csname pn@uco.lab.vlmnoleak\endcsname{0.322}
\expandafter\def\csname pn@uco.tiny.gt.ade\endcsname{0.192}
\expandafter\def\csname pn@uco.tiny.gt.sd\endcsname{0.004}
\expandafter\def\csname pn@uco.tiny.gt.pck10\endcsname{0.247}
\expandafter\def\csname pn@uco.tiny.mtgs.ade\endcsname{0.174}
\expandafter\def\csname pn@uco.tiny.mtgs.sd\endcsname{0.001}
\expandafter\def\csname pn@uco.tiny.mtgs.pck10\endcsname{0.294}
\expandafter\def\csname pn@uco.tiny.gazelle.ade\endcsname{0.176}
\expandafter\def\csname pn@uco.tiny.gazelle.sd\endcsname{0.004}
\expandafter\def\csname pn@uco.tiny.gazelle.pck10\endcsname{0.278}
\expandafter\def\csname pn@uco.tiny.teacher_hybrid.ade\endcsname{0.204}
\expandafter\def\csname pn@uco.tiny.teacher_hybrid.sd\endcsname{0.015}
\expandafter\def\csname pn@uco.tiny.teacher_hybrid.pck10\endcsname{0.190}
\expandafter\def\csname pn@uco.tiny.teacher_internvl3_alone.ade\endcsname{0.159}
\expandafter\def\csname pn@uco.tiny.teacher_internvl3_alone.sd\endcsname{0.001}
\expandafter\def\csname pn@uco.tiny.teacher_internvl3_alone.pck10\endcsname{0.343}
\expandafter\def\csname pn@uco.tiny.copyb.ade\endcsname{0.145}
\expandafter\def\csname pn@uco.tiny.copyb.sd\endcsname{0.008}
\expandafter\def\csname pn@uco.tiny.copyb.pck10\endcsname{0.415}
\expandafter\def\csname pn@uco.tiny.vlmnoleak.ade\endcsname{0.313}
\expandafter\def\csname pn@uco.tiny.vlmnoleak.sd\endcsname{0.024}
\expandafter\def\csname pn@uco.tiny.vlmnoleak.pck10\endcsname{0.042}
\expandafter\def\csname pn@uco.tiny.ovdalwaysdino.ade\endcsname{0.268}
\expandafter\def\csname pn@uco.tiny.ovdalwaysdino.sd\endcsname{0.004}
\expandafter\def\csname pn@uco.tiny.ovdalwaysdino.pck10\endcsname{0.052}
\expandafter\def\csname pn@uco.tiny.ovdgate55.ade\endcsname{0.263}
\expandafter\def\csname pn@uco.tiny.ovdgate55.sd\endcsname{0.001}
\expandafter\def\csname pn@uco.tiny.ovdgate55.pck10\endcsname{0.060}
\expandafter\def\csname pn@uco.tiny.ovdmixrand.ade\endcsname{0.262}
\expandafter\def\csname pn@uco.tiny.ovdmixrand.sd\endcsname{0.004}
\expandafter\def\csname pn@uco.tiny.ovdmixrand.pck10\endcsname{0.055}
\expandafter\def\csname pn@uco.tiny.centre.ade\endcsname{0.283}
\expandafter\def\csname pn@uco.tiny.centre.sd\endcsname{0.000}
\expandafter\def\csname pn@uco.tiny.centre.pck10\endcsname{0.028}
\expandafter\def\csname pn@uco.small.gt.ade\endcsname{0.165}
\expandafter\def\csname pn@uco.small.gt.sd\endcsname{0.005}
\expandafter\def\csname pn@uco.small.gt.pck10\endcsname{0.301}
\expandafter\def\csname pn@uco.small.mtgs.ade\endcsname{0.147}
\expandafter\def\csname pn@uco.small.mtgs.sd\endcsname{0.003}
\expandafter\def\csname pn@uco.small.mtgs.pck10\endcsname{0.399}
\expandafter\def\csname pn@uco.small.gazelle.ade\endcsname{0.152}
\expandafter\def\csname pn@uco.small.gazelle.sd\endcsname{0.007}
\expandafter\def\csname pn@uco.small.gazelle.pck10\endcsname{0.348}
\expandafter\def\csname pn@uco.small.teacher_hybrid.ade\endcsname{0.168}
\expandafter\def\csname pn@uco.small.teacher_hybrid.sd\endcsname{0.008}
\expandafter\def\csname pn@uco.small.teacher_hybrid.pck10\endcsname{0.302}
\expandafter\def\csname pn@uco.small.teacher_internvl3_alone.ade\endcsname{0.138}
\expandafter\def\csname pn@uco.small.teacher_internvl3_alone.sd\endcsname{0.010}
\expandafter\def\csname pn@uco.small.teacher_internvl3_alone.pck10\endcsname{0.423}
\expandafter\def\csname pn@uco.small.copyb.ade\endcsname{0.109}
\expandafter\def\csname pn@uco.small.copyb.sd\endcsname{0.006}
\expandafter\def\csname pn@uco.small.copyb.pck10\endcsname{0.618}
\expandafter\def\csname pn@uco.small.vlmnoleak.ade\endcsname{0.321}
\expandafter\def\csname pn@uco.small.vlmnoleak.sd\endcsname{0.007}
\expandafter\def\csname pn@uco.small.vlmnoleak.pck10\endcsname{0.042}
\expandafter\def\csname pn@uco.small.ovdalwaysdino.ade\endcsname{0.277}
\expandafter\def\csname pn@uco.small.ovdalwaysdino.sd\endcsname{0.032}
\expandafter\def\csname pn@uco.small.ovdalwaysdino.pck10\endcsname{0.047}
\expandafter\def\csname pn@uco.small.ovdgate55.ade\endcsname{0.290}
\expandafter\def\csname pn@uco.small.ovdgate55.sd\endcsname{0.035}
\expandafter\def\csname pn@uco.small.ovdgate55.pck10\endcsname{0.049}
\expandafter\def\csname pn@uco.small.ovdmixrand.ade\endcsname{0.312}
\expandafter\def\csname pn@uco.small.ovdmixrand.sd\endcsname{0.008}
\expandafter\def\csname pn@uco.small.ovdmixrand.pck10\endcsname{0.038}
\expandafter\def\csname pn@uco.small.centre.ade\endcsname{0.283}
\expandafter\def\csname pn@uco.small.centre.sd\endcsname{0.000}
\expandafter\def\csname pn@uco.small.centre.pck10\endcsname{0.028}
\expandafter\def\csname pn@e2e.tiny.gt.copygap\endcsname{0.0016}
\expandafter\def\csname pn@e2e.tiny.gt.runs\endcsname{4}
\expandafter\def\csname pn@e2e.tiny.gt.h300.e2e.ade\endcsname{0.208}
\expandafter\def\csname pn@e2e.tiny.gt.h300.e2e.obj\endcsname{0.231}
\expandafter\def\csname pn@e2e.tiny.gt.h300.e2e.soc\endcsname{0.183}
\expandafter\def\csname pn@e2e.tiny.gt.h300.copy.ade\endcsname{0.208}
\expandafter\def\csname pn@e2e.tiny.gt.h300.copy.obj\endcsname{0.235}
\expandafter\def\csname pn@e2e.tiny.gt.h300.copy.soc\endcsname{0.179}
\expandafter\def\csname pn@e2e.tiny.gt.h300.head.ade\endcsname{0.210}
\expandafter\def\csname pn@e2e.tiny.gt.h300.head.obj\endcsname{0.236}
\expandafter\def\csname pn@e2e.tiny.gt.h300.head.soc\endcsname{0.181}
\expandafter\def\csname pn@e2e.tiny.gt.h300.lkgt.ade\endcsname{0.035}
\expandafter\def\csname pn@e2e.tiny.gt.h300.lkgt.obj\endcsname{0.039}
\expandafter\def\csname pn@e2e.tiny.gt.h300.lkgt.soc\endcsname{0.031}
\expandafter\def\csname pn@e2e.tiny.gt.h300.delta\endcsname{0.000}
\expandafter\def\csname pn@e2e.tiny.gt.h300.deltahead\endcsname{$-$0.002}
\expandafter\def\csname pn@e2e.tiny.gt.h300.nseeds\endcsname{3}
\expandafter\def\csname pn@e2e.tiny.gt.h300.epochs\endcsname{5, 2, 1}
\expandafter\def\csname pn@e2e.tiny.gt.h300.ntrain\endcsname{79{,}470}
\expandafter\def\csname pn@e2e.tiny.gt.h300.nval\endcsname{10{,}011}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.pooled.ns\endcsname{3}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.object.REALp\endcsname{1}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.object.ns\endcsname{2}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.social.ns\endcsname{2}
\expandafter\def\csname pn@e2e.tiny.gt.h300.v.social.REALm\endcsname{1}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s42.e2e\endcsname{0.207}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s42.copy\endcsname{0.209}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s42.ci\endcsname{[-0.0108, +0.0063]}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s42.lossratio\endcsname{5.3}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s88.e2e\endcsname{0.208}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s88.copy\endcsname{0.211}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s88.ci\endcsname{[-0.0119, +0.0062]}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s88.lossratio\endcsname{2.3}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s137.e2e\endcsname{0.209}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s137.copy\endcsname{0.205}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s137.ci\endcsname{[-0.0030, +0.0121]}
\expandafter\def\csname pn@e2e.tiny.gt.h300.s137.lossratio\endcsname{2.0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.e2e.ade\endcsname{0.212}
\expandafter\def\csname pn@e2e.tiny.gt.h500.e2e.obj\endcsname{0.239}
\expandafter\def\csname pn@e2e.tiny.gt.h500.e2e.soc\endcsname{0.182}
\expandafter\def\csname pn@e2e.tiny.gt.h500.copy.ade\endcsname{0.212}
\expandafter\def\csname pn@e2e.tiny.gt.h500.copy.obj\endcsname{0.239}
\expandafter\def\csname pn@e2e.tiny.gt.h500.copy.soc\endcsname{0.182}
\expandafter\def\csname pn@e2e.tiny.gt.h500.head.ade\endcsname{0.215}
\expandafter\def\csname pn@e2e.tiny.gt.h500.head.obj\endcsname{0.240}
\expandafter\def\csname pn@e2e.tiny.gt.h500.head.soc\endcsname{0.188}
\expandafter\def\csname pn@e2e.tiny.gt.h500.lkgt.ade\endcsname{0.053}
\expandafter\def\csname pn@e2e.tiny.gt.h500.lkgt.obj\endcsname{0.057}
\expandafter\def\csname pn@e2e.tiny.gt.h500.lkgt.soc\endcsname{0.047}
\expandafter\def\csname pn@e2e.tiny.gt.h500.delta\endcsname{0.000}
\expandafter\def\csname pn@e2e.tiny.gt.h500.deltahead\endcsname{$-$0.003}
\expandafter\def\csname pn@e2e.tiny.gt.h500.nseeds\endcsname{1}
\expandafter\def\csname pn@e2e.tiny.gt.h500.epochs\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.ntrain\endcsname{75{,}125}
\expandafter\def\csname pn@e2e.tiny.gt.h500.nval\endcsname{9{,}561}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.pooled.REALp\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.pooled.ns\endcsname{1}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.pooled.REALm\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.object.REALp\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.object.ns\endcsname{1}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.object.REALm\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.social.REALp\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.social.ns\endcsname{1}
\expandafter\def\csname pn@e2e.tiny.gt.h500.v.social.REALm\endcsname{0}
\expandafter\def\csname pn@e2e.tiny.gt.h500.s42.e2e\endcsname{0.212}
\expandafter\def\csname pn@e2e.tiny.gt.h500.s42.copy\endcsname{0.212}
\expandafter\def\csname pn@e2e.tiny.gt.h500.s42.ci\endcsname{[+0.0000, +0.0000]}
\expandafter\def\csname pn@e2e.tiny.gt.h500.s42.lossratio\endcsname{1.7}
\expandafter\def\csname pn@lc.sources\endcsname{10}
\expandafter\def\csname pn@lc.draws\endcsname{2{,}000}
\expandafter\def\csname pn@lc.rho.tiny\endcsname{0.93}
\expandafter\def\csname pn@lc.rho.small\endcsname{0.95}
\expandafter\def\csname pn@lc.k3.clips\endcsname{3}
\expandafter\def\csname pn@lc.k3.frames\endcsname{700}
\expandafter\def\csname pn@lc.k3.top2\endcsname{76\%}
\expandafter\def\csname pn@lc.k3.rho.tiny\endcsname{0.77}
\expandafter\def\csname pn@lc.k5.clips\endcsname{5}
\expandafter\def\csname pn@lc.k5.frames\endcsname{1{,}300}
\expandafter\def\csname pn@lc.k5.top2\endcsname{90\%}
\expandafter\def\csname pn@lc.k5.rho.tiny\endcsname{0.82}
\expandafter\def\csname pn@lc.k10.clips\endcsname{10}
\expandafter\def\csname pn@lc.k10.frames\endcsname{2{,}700}
\expandafter\def\csname pn@lc.k10.top2\endcsname{99\%}
\expandafter\def\csname pn@lc.k10.rho.tiny\endcsname{0.87}
\expandafter\def\csname pn@lc.k20.clips\endcsname{20}
\expandafter\def\csname pn@lc.k20.frames\endcsname{5{,}600}
\expandafter\def\csname pn@lc.k20.top2\endcsname{100\%}
\expandafter\def\csname pn@lc.k20.rho.tiny\endcsname{0.89}
\expandafter\def\csname pn@lc.k40.clips\endcsname{40}
\expandafter\def\csname pn@lc.k40.frames\endcsname{11{,}500}
\expandafter\def\csname pn@lc.k40.top2\endcsname{100\%}
\expandafter\def\csname pn@lc.k40.rho.tiny\endcsname{0.91}
\expandafter\def\csname pn@lc.k10.trainshare\endcsname{0.8\%}
\expandafter\def\csname pn@lc.vat.k10.rho.tiny\endcsname{0.82}
\expandafter\def\csname pn@lc.childplay.k10.rho.tiny\endcsname{0.94}
\expandafter\def\csname pn@lc.vacation.k10.rho.tiny\endcsname{0.92}
\expandafter\def\csname pn@tp.tiny.proto.sel_clip.object.REALp.biased\endcsname{27}
\expandafter\def\csname cn@gt\endcsname{Annotation}
\expandafter\def\csname cn@mtgs\endcsname{MTGS}
\expandafter\def\csname cn@gazelle\endcsname{Gaze-LLE}
\expandafter\def\csname cn@teacher_hybrid\endcsname{VLM+OVD, leaky}
\expandafter\def\csname cn@teacher_internvl3_alone\endcsname{VLM, leaky}
\expandafter\def\csname cn@copyb\endcsname{Copy-B}
\expandafter\def\csname cn@vlmnoleak\endcsname{VLM, no leak}
\expandafter\def\csname cn@ovdalwaysdino\endcsname{VLM+OVD, no leak}
\expandafter\def\csname cn@ovdgate55\endcsname{\quad + conf.\ gate}
\expandafter\def\csname cn@ovdmixrand\endcsname{\quad + random swap}
\expandafter\def\csname cn@centre\endcsname{Image centre}
\expandafter\def\csname cn@ovdgate40\endcsname{\quad + conf.\ gate ($t{=}0.40$)}
\expandafter\def\csname cn@ovdmix40\endcsname{\quad + random swap (same rate)}
\expandafter\def\csname cn@ovdgate48\endcsname{\quad + conf.\ gate ($t{=}0.48$)}
\expandafter\def\csname cn@ovdmix48\endcsname{\quad + random swap (same rate)}
\expandafter\def\csname cn@ovdgate100\endcsname{\quad + every detection replaced ($t{=}1$)}
\expandafter\def\csname pn@lcv.draws\endcsname{2{,}000}
\expandafter\def\csname pn@lcv.clips\endcsname{82}
\expandafter\def\csname pn@lcv.rows\endcsname{42{,}170}
\expandafter\def\csname pn@lcv.rho.tiny\endcsname{0.91}
\expandafter\def\csname pn@lcv.rho.small\endcsname{0.90}
\expandafter\def\csname pn@lcv.k3.clips\endcsname{3}
\expandafter\def\csname pn@lcv.k3.frames\endcsname{1{,}300}
\expandafter\def\csname pn@lcv.k3.top2\endcsname{70\%}
\expandafter\def\csname pn@lcv.k3.rho.tiny\endcsname{0.79}
\expandafter\def\csname pn@lcv.k5.clips\endcsname{5}
\expandafter\def\csname pn@lcv.k5.frames\endcsname{2{,}200}
\expandafter\def\csname pn@lcv.k5.top2\endcsname{83\%}
\expandafter\def\csname pn@lcv.k5.rho.tiny\endcsname{0.84}
\expandafter\def\csname pn@lcv.k10.clips\endcsname{10}
\expandafter\def\csname pn@lcv.k10.frames\endcsname{4{,}800}
\expandafter\def\csname pn@lcv.k10.top2\endcsname{95\%}
\expandafter\def\csname pn@lcv.k10.rho.tiny\endcsname{0.87}
\expandafter\def\csname pn@lcv.k20.clips\endcsname{20}
\expandafter\def\csname pn@lcv.k20.frames\endcsname{10{,}300}
\expandafter\def\csname pn@lcv.k20.top2\endcsname{99\%}
\expandafter\def\csname pn@lcv.k20.rho.tiny\endcsname{0.90}
\expandafter\def\csname pn@lcv.k40.clips\endcsname{40}
\expandafter\def\csname pn@lcv.k40.frames\endcsname{20{,}500}
\expandafter\def\csname pn@lcv.k40.top2\endcsname{100\%}
\expandafter\def\csname pn@lcv.k40.rho.tiny\endcsname{0.91}
\expandafter\def\csname pn@lcv.k10.trainshare\endcsname{1.3\%}
\expandafter\def\csname pn@lcv.vat.k10.rho.tiny\endcsname{0.93}
\expandafter\def\csname pn@lcv.vat.k10.top2\endcsname{92\%}
\expandafter\def\csname pn@lcv.childplay.k10.rho.tiny\endcsname{0.93}
\expandafter\def\csname pn@lcv.childplay.k10.top2\endcsname{43\%}
\expandafter\def\csname pn@lcv.vacation.k10.rho.tiny\endcsname{0.76}
\expandafter\def\csname pn@lcv.vacation.k10.top2\endcsname{100\%}
\providecommand{\C}[1]{\ifcsname cn@#1\endcsname\csname cn@#1\endcsname\else\textbf{\color{red}??\detokenize{#1}}\fi}
\makeatother

